Invisible-to-Visible: Privacy-Aware Human Instance Segmentation using Airborne Ultrasound via Collaborative Learning Variational Autoencoder

In action understanding in indoor, we have to recognize human pose and action considering privacy. Although camera images can be used for highly accurate human action recognition, camera images do not preserve privacy. Therefore, we propose a new task for human instance segmentation from invisible information, especially airborne ultrasound, for action recognition. To perform instance segmentation from invisible information, we first convert sound waves to reflected sound directional images (sound images). Although the sound images can roughly identify the location of a person, the detailed shape is ambiguous. To address this problem, we propose a collaborative learning variational autoencoder (CL-VAE) that simultaneously uses sound and RGB images during training. In inference, it is possible to obtain instance segmentation results only from sound images. As a result of performance verification, CL-VAE could estimate human instance segmentations more accurately than conventional variational autoencoder and some other models. Since this method can obtain human segmentations individually, it could be applied to human action recognition tasks with privacy protection.

==> dvipdfm/ChangeLog <==
2000-07-25  Mark A. Wicks  <mwicks@betelgeuse.localdomain>

        * Changed version to 0.13
	* Cleaned up DVI and VF code so it all works on 16 bit chars
	* Added support for 16 bit virtual fonts (OTF file)
	
2000-07-23  Mark A. Wicks  <mwicks@betelgeuse.localdomain>

	* Cleanly separated encodings from fonts so that multiple
	  encodings can be used for the same font in the same document.
	  That way, all glyphs (>256) are available from a font:-).
	* Made Type 1 font parsing and font subsetting more robust
	* Changed version to 0.12.9beta
      	* Changed encoding method to help Acrobat Exchange 3.0
	  merge files created by dvipdfm.
	
2000-07-06  Mark A. Wicks  <mwicks@betelgeuse.localdomain>

	* Changed version to 0.12.8
	* Fixed a bug in the encoding code that could
	  cause characters to disappear in certain situations
	* Fixed figure inclusion bugs
	    - Specials generated by older psfig macros now work
	    - Clipping/cropping and bounding box overrides now
     	      work on included MetaPost images.  Clipping/cropping
	      and bounding box overrides don't (and may never)
	      work on bitmaps.
	
2000-05-24  Mark A. Wicks  <mwicks@betelgeuse.localdomain>
	* Fixed another unrelated bug that mostly affected color maps on
	  embedded bitmaps

2000-02-06  Mark A. Wicks  <mwicks@betelgeuse.localdomain>
	* Fixed a bug that mostly affected color maps on embedded bitmaps

1999-01 thru
2000-03 07-06  Mark A. Wicks  <mwicks@betelgeuse.localdomain>
	* Made PS parsing a bit more robust

1999-09-19  Mark A. Wicks  <mwicks@betelgeuse.wicks.net>
       	* Changed version to 0.12.4.
	* Added link breaking code (aka breaklinks) and additional
	  \special operators to support them.
	* Fixed a bug in slanted font code
	* Fixed a bug in TFM code that won't actually execute
	  unless you have a defective TFM file.

1999-09-06  Mark A. Wicks  <mwicks@betelgeuse.wicks.net>

	* Added native MetaPost and native support
  	  for simple PS operators
	* Added PS/EPS support with helper program
	* Added a configuration file
	* Added standard color specials
	* Added standard landscape and papersize specials
	* Added support for PSfile and plotfile specials

1999-08-22  Mark A. Wicks  <mwicks@betelgeuse.wicks.net>

	* Added slantfont and expand font support
	* Removed dependency on AFM files
	* Added support for font remapping to work around
	  some problems with Adobe Reader and certain character positions.
	* Reworked font code a lot.

1999-02-08  Mark A. Wicks  <mwicks@odo.kettering.edu>
	* Version 0.10.0 includes 
	    PK font support
	    Tpic special support
	    kpath searching for included pdf and jpeg files via 
	    the path defined by TEXPICTS

1998-11-30  Mark A. Wicks  <mwicks@odo.kettering.edu>

	* Cleaned up a lot of little things.
	* Tried to make code 8-bit clean in most places
	* Added check for timezone in autoconf script.

1998-11-29  Mark A. Wicks  <mwicks@betelgeuse.wicks.net>

	* Added font re-encoding support and created a map file for common
	  PostScript fonts.

	* Cleaned up some little things.

1998-11-27  Mark A. Wicks  <mwicks@odo.kettering.edu>

	* Changed source tree to fit with texk distribution.

	* Added cmyk color support.
	
1998-11-26  Mark A. Wicks  <mwicks@odo.kettering.edu>

	* Fixed a bug in the outline/bookmark tree structure.
	
	* Changed the \special parser so it would recognize numbers
          that don't start with a digit.

        * Added macro support for Graphics and hyperref.
   
        * Several minor changes.


==> dvipdfm/README <==
   This is dvipdfm, a DVI to PDF translator.  I wrote this mainly as
exercise to get at the features of PDF I wanted to experiment with. You're
probably wondering why I don't use PDFTeX.  I am a bit of a purist and I
would rather use TeX unmodified as Donald Knuth left it.
You can get it or the manual from

    http://odo.kettering.edu/dvipdfm

or if you prefer FTP:

    ftp://ftp.kettering.edu/pub/outgoing/mwicks/dvipdfm
    

   Features:
      - TeX \special's that approximate the functionality 
        of the PostScript pdfmarks used by Adobe's
	Acrobat Distiller.  Links, outlines, articles, and named
	destinations are supported, for example.

      - Ability to include PDF, JPEG, PNG, MetaPost, and self-contained
	(e.g., eps) PostScript (with help from an external program) files as
	embedded images.  For PDF files, only the first page is included.
	Resources will be embedded from the original file as necessary.
	File inclusion does not work for PDF files that store the page
	contents in several segments in an array.

      - Support for several \special standards for
        DVI file portability.

      - Support for thumbnails (with a little help from GhostScript).
	
      - Re-encoding support for PostScript fonts.  dvipdfm
        uses the same .enc files as dvips.  The mapfile is different.
	
      - Virtual font support.	
	
      - Support for arbitrary linear graphics transformations.
        Any material on the page can be scaled and rotated.

      - An internal color stack accessible via \special's.

      - Beginning of page (BOP) and end of page (EOP)
        \special's for placing arbitrary PDF stream
	graphics on every page.
	
      - Partial font embedding and Flate compression
        for reduced file size.
	
      - Balanced page tree and dest tree to improve reader
        speed on very large documents.

   Limitations (at present):

      - Contents streams consisting of multiple parts cannot be embedded.
      - All instances of the same Type1 font must have the same encoding.
     
   Additional Information:
   
   There is a dvipdfm e-mail list.  To join, send
e-mail to majordomo@gaspra.kettering.edu containing
the line:

   subscribe dvipdfm
    
   Mark A. Wicks
   Kettering University
   mwicks@kettering.edu


==> dvipdfm/configure <==
#! /bin/sh
# Guess values for system-dependent variables and create Makefiles.
# Generated by GNU Autoconf 2.60.
#
# Copyright (C) 1992, 1993, 1994, 1995, 1996, 1998, 1999, 2000, 2001,
# 2002, 2003, 2004, 2005, 2006 Free Software Foundation, Inc.
# This configure script is free software; the Free Software Foundation
# gives unlimited permission to copy, distribute and modify it.
## --------------------- ##
## M4sh Initialization.  ##
## --------------------- ##

# Be Bourne compatible
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in *posix*) set -o posix;; esac
fi
BIN_SH=xpg4; export BIN_SH # for Tru64
DUALCASE=1; export DUALCASE # for MKS sh


# PATH needs CR
# Avoid depending upon Character Ranges.
as_cr_letters='abcdefghijklmnopqrstuvwxyz'
as_cr_LETTERS='ABCDEFGHIJKLMNOPQRSTUVWXYZ'
as_cr_Letters=$as_cr_letters$as_cr_LETTERS
as_cr_digits='0123456789'
as_cr_alnum=$as_cr_Letters$as_cr_digits

# The user is always right.
if test "${PATH_SEPARATOR+set}" != set; then
  echo "#! /bin/sh" >conf$$.sh
  echo  "exit 0"   >>conf$$.sh
  chmod +x conf$$.sh
  if (PATH="/nonexistent;."; conf$$.sh) >/dev/null 2>&1; then
    PATH_SEPARATOR=';'
  else
    PATH_SEPARATOR=:
  fi
  rm -f conf$$.sh
fi

# Support unset when possible.
if ( (MAIL=60; unset MAIL) || exit) >/dev/null 2>&1; then
  as_unset=unset
else
  as_unset=false
fi


# IFS
# We need space, tab and new line, in precisely that order.  Quoting is
# there to prevent editors from complaining about space-tab.
# (If _AS_PATH_WALK were called with IFS unset, it would disable word
# splitting by setting IFS to empty value.)
as_nl='
'
IFS=" ""	$as_nl"

# Find who we are.  Look in the path if we contain no directory separator.
case $0 in
  *[\\/]* ) as_myself=$0 ;;
  *) as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  test -r "$as_dir/$0" && as_myself=$as_dir/$0 && break
done
IFS=$as_save_IFS

     ;;
esac
# We did not find ourselves, most probably we were run as `sh COMMAND'
# in which case we are not to be found in the path.
if test "x$as_myself" = x; then
  as_myself=$0
fi
if test ! -f "$as_myself"; then
  echo "$as_myself: error: cannot find myself; rerun with an absolute file name" >&2
  { (exit 1); exit 1; }
fi

# Work around bugs in pre-3.0 UWIN ksh.
for as_var in ENV MAIL MAILPATH
do ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
done
PS1='$ '
PS2='> '
PS4='+ '

# NLS nuisances.
for as_var in \
  LANG LANGUAGE LC_ADDRESS LC_ALL LC_COLLATE LC_CTYPE LC_IDENTIFICATION \
  LC_MEASUREMENT LC_MESSAGES LC_MONETARY LC_NAME LC_NUMERIC LC_PAPER \
  LC_TELEPHONE LC_TIME
do
  if (set +x; test -z "`(eval $as_var=C; export $as_var) 2>&1`"); then
    eval $as_var=C; export $as_var
  else
    ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
  fi
done

# Required to use basename.
if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

if (basename -- /) >/dev/null 2>&1 && test "X`basename -- / 2>&1`" = "X/"; then
  as_basename=basename
else
  as_basename=false
fi


# Name of the executable.
as_me=`$as_basename -- "$0" ||
$as_expr X/"$0" : '.*/\([^/][^/]*\)/*$' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
echo X/"$0" |
    sed '/^.*\/\([^/][^/]*\)\/*$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`

# CDPATH.
$as_unset CDPATH


if test "x$CONFIG_SHELL" = x; then
  if (eval ":") 2>/dev/null; then
  as_have_required=yes
else
  as_have_required=no
fi

  if test $as_have_required = yes && 	 (eval ":
(as_func_return () {
  (exit \$1)
}
as_func_success () {
  as_func_return 0
}
as_func_failure () {
  as_func_return 1
}
as_func_ret_success () {
  return 0
}
as_func_ret_failure () {
  return 1
}

exitcode=0
if as_func_success; then
  :
else
  exitcode=1
  echo as_func_success failed.
fi

if as_func_failure; then
  exitcode=1
  echo as_func_failure succeeded.
fi

if as_func_ret_success; then
  :
else
  exitcode=1
  echo as_func_ret_success failed.
fi

if as_func_ret_failure; then
  exitcode=1
  echo as_func_ret_failure succeeded.
fi

if ( set x; as_func_ret_success y && test x = \"\$1\" ); then
  :
else
  exitcode=1
  echo positional parameters were not saved.
fi

test \$exitcode = 0) || { (exit 1); exit 1; }

(
  as_lineno_1=\$LINENO
  as_lineno_2=\$LINENO
  test \"x\$as_lineno_1\" != \"x\$as_lineno_2\" &&
  test \"x\`expr \$as_lineno_1 + 1\`\" = \"x\$as_lineno_2\") || { (exit 1); exit 1; }
") 2> /dev/null; then
  :
else
  as_candidate_shells=
    as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in /usr/bin/posix$PATH_SEPARATOR/bin$PATH_SEPARATOR/usr/bin$PATH_SEPARATOR$PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  case $as_dir in
	 /*)
	   for as_base in sh bash ksh sh5; do
	     as_candidate_shells="$as_candidate_shells $as_dir/$as_base"
	   done;;
       esac
done
IFS=$as_save_IFS


      for as_shell in $as_candidate_shells $SHELL; do
	 # Try only shells that exist, to save several forks.
	 if { test -f "$as_shell" || test -f "$as_shell.exe"; } &&
		{ ("$as_shell") 2> /dev/null <<\_ASEOF
# Be Bourne compatible
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in *posix*) set -o posix;; esac
fi
BIN_SH=xpg4; export BIN_SH # for Tru64
DUALCASE=1; export DUALCASE # for MKS sh

:
_ASEOF
}; then
  CONFIG_SHELL=$as_shell
	       as_have_required=yes
	       if { "$as_shell" 2> /dev/null <<\_ASEOF
# Be Bourne compatible
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in *posix*) set -o posix;; esac
fi
BIN_SH=xpg4; export BIN_SH # for Tru64
DUALCASE=1; export DUALCASE # for MKS sh

:
(as_func_return () {
  (exit $1)
}
as_func_success () {
  as_func_return 0
}
as_func_failure () {
  as_func_return 1
}
as_func_ret_success () {
  return 0
}
as_func_ret_failure () {
  return 1
}

exitcode=0
if as_func_success; then
  :
else
  exitcode=1
  echo as_func_success failed.
fi

if as_func_failure; then
  exitcode=1
  echo as_func_failure succeeded.
fi

if as_func_ret_success; then
  :
else
  exitcode=1
  echo as_func_ret_success failed.
fi

if as_func_ret_failure; then
  exitcode=1
  echo as_func_ret_failure succeeded.
fi

if ( set x; as_func_ret_success y && test x = "$1" ); then
  :
else
  exitcode=1
  echo positional parameters were not saved.
fi

test $exitcode = 0) || { (exit 1); exit 1; }

(
  as_lineno_1=$LINENO
  as_lineno_2=$LINENO
  test "x$as_lineno_1" != "x$as_lineno_2" &&
  test "x`expr $as_lineno_1 + 1`" = "x$as_lineno_2") || { (exit 1); exit 1; }

_ASEOF
}; then
  break
fi

fi

      done

      if test "x$CONFIG_SHELL" != x; then
  for as_var in BASH_ENV ENV
        do ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
        done
        export CONFIG_SHELL
        exec "$CONFIG_SHELL" "$as_myself" ${1+"$@"}
fi


    if test $as_have_required = no; then
  echo This script requires a shell more modern than all the
      echo shells that I found on your system.  Please install a
      echo modern shell, or manually run the script under such a
      echo shell if you do have one.
      { (exit 1); exit 1; }
fi


fi

fi



(eval "as_func_return () {
  (exit \$1)
}
as_func_success () {
  as_func_return 0
}
as_func_failure () {
  as_func_return 1
}
as_func_ret_success () {
  return 0
}
as_func_ret_failure () {
  return 1
}

exitcode=0
if as_func_success; then
  :
else
  exitcode=1
  echo as_func_success failed.
fi

if as_func_failure; then
  exitcode=1
  echo as_func_failure succeeded.
fi

if as_func_ret_success; then
  :
else
  exitcode=1
  echo as_func_ret_success failed.
fi

if as_func_ret_failure; then
  exitcode=1
  echo as_func_ret_failure succeeded.
fi

if ( set x; as_func_ret_success y && test x = \"\$1\" ); then
  :
else
  exitcode=1
  echo positional parameters were not saved.
fi

test \$exitcode = 0") || {
  echo No shell found that supports shell functions.
  echo Please tell autoconf@gnu.org about your system,
  echo including any error possibly output before this
  echo message
}



  as_lineno_1=$LINENO
  as_lineno_2=$LINENO
  test "x$as_lineno_1" != "x$as_lineno_2" &&
  test "x`expr $as_lineno_1 + 1`" = "x$as_lineno_2" || {

  # Create $as_me.lineno as a copy of $as_myself, but with $LINENO
  # uniformly replaced by the line number.  The first 'sed' inserts a
  # line-number line after each line using $LINENO; the second 'sed'
  # does the real work.  The second script uses 'N' to pair each
  # line-number line with the line containing $LINENO, and appends
  # trailing '-' during substitution so that $LINENO is not a special
  # case at line end.
  # (Raja R Harinath suggested sed '=', and Paul Eggert wrote the
  # scripts with optimization help from Paolo Bonzini.  Blame Lee
  # E. McMahon (1931-1989) for sed's syntax.  :-)
  sed -n '
    p
    /[$]LINENO/=
  ' <$as_myself |
    sed '
      s/[$]LINENO.*/&-/
      t lineno
      b
      :lineno
      N
      :loop
      s/[$]LINENO\([^'$as_cr_alnum'_].*\n\)\(.*\)/\2\1\2/
      t loop
      s/-\n.*//
    ' >$as_me.lineno &&
  chmod +x "$as_me.lineno" ||
    { echo "$as_me: error: cannot create $as_me.lineno; rerun with a POSIX shell" >&2
   { (exit 1); exit 1; }; }

  # Don't try to exec as it changes $[0], causing all sort of problems
  # (the dirname of $[0] is not the place where we might find the
  # original and so on.  Autoconf is especially sensitive to this).
  . "./$as_me.lineno"
  # Exit status is that of the last command.
  exit
}


if (as_dir=`dirname -- /` && test "X$as_dir" = X/) >/dev/null 2>&1; then
  as_dirname=dirname
else
  as_dirname=false
fi

ECHO_C= ECHO_N= ECHO_T=
case `echo -n x` in
-n*)
  case `echo 'x\c'` in
  *c*) ECHO_T='	';;	# ECHO_T is single tab character.
  *)   ECHO_C='\c';;
  esac;;
*)
  ECHO_N='-n';;
esac

if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

rm -f conf$$ conf$$.exe conf$$.file
if test -d conf$$.dir; then
  rm -f conf$$.dir/conf$$.file
else
  rm -f conf$$.dir
  mkdir conf$$.dir
fi
echo >conf$$.file
if ln -s conf$$.file conf$$ 2>/dev/null; then
  as_ln_s='ln -s'
  # ... but there are two gotchas:
  # 1) On MSYS, both `ln -s file dir' and `ln file dir' fail.
  # 2) DJGPP < 2.04 has no symlinks; `ln -s' creates a wrapper executable.
  # In both cases, we have to default to `cp -p'.
  ln -s conf$$.file conf$$.dir 2>/dev/null && test ! -f conf$$.exe ||
    as_ln_s='cp -p'
elif ln conf$$.file conf$$ 2>/dev/null; then
  as_ln_s=ln
else
  as_ln_s='cp -p'
fi
rm -f conf$$ conf$$.exe conf$$.dir/conf$$.file conf$$.file
rmdir conf$$.dir 2>/dev/null

if mkdir -p . 2>/dev/null; then
  as_mkdir_p=:
else
  test -d ./-p && rmdir ./-p
  as_mkdir_p=false
fi

# Find out whether ``test -x'' works.  Don't use a zero-byte file, as
# systems may use methods other than mode bits to determine executability.
cat >conf$$.file <<_ASEOF
#! /bin/sh
exit 0
_ASEOF
chmod +x conf$$.file
if test -x conf$$.file >/dev/null 2>&1; then
  as_executable_p="test -x"
else
  as_executable_p=:
fi
rm -f conf$$.file

# Sed expression to map a string onto a valid CPP name.
as_tr_cpp="eval sed 'y%*$as_cr_letters%P$as_cr_LETTERS%;s%[^_$as_cr_alnum]%_%g'"

# Sed expression to map a string onto a valid variable name.
as_tr_sh="eval sed 'y%*+%pp%;s%[^_$as_cr_alnum]%_%g'"



exec 7<&0 </dev/null 6>&1

# Name of the host.
# hostname on some systems (SVR3.2, Linux) returns a bogus exit status,
# so uname gets run too.
ac_hostname=`(hostname || uname -n) 2>/dev/null | sed 1q`

#
# Initializations.
#
ac_default_prefix=/usr/local
ac_clean_files=
ac_config_libobj_dir=.
LIBOBJS=
cross_compiling=no
subdirs=
MFLAGS=
MAKEFLAGS=
SHELL=${CONFIG_SHELL-/bin/sh}

# Identity of this package.
PACKAGE_NAME=
PACKAGE_TARNAME=
PACKAGE_VERSION=
PACKAGE_STRING=
PACKAGE_BUGREPORT=

ac_unique_file="dvipdfm.c"
# Factoring default headers for most tests.
ac_includes_default="\
#include <stdio.h>
#if HAVE_SYS_TYPES_H
# include <sys/types.h>
#endif
#if HAVE_SYS_STAT_H
# include <sys/stat.h>
#endif
#if STDC_HEADERS
# include <stdlib.h>
# include <stddef.h>
#else
# if HAVE_STDLIB_H
#  include <stdlib.h>
# endif
#endif
#if HAVE_STRING_H
# if !STDC_HEADERS && HAVE_MEMORY_H
#  include <memory.h>
# endif
# include <string.h>
#endif
#if HAVE_STRINGS_H
# include <strings.h>
#endif
#if HAVE_INTTYPES_H
# include <inttypes.h>
#endif
#if HAVE_STDINT_H
# include <stdint.h>
#endif
#if HAVE_UNISTD_H
# include <unistd.h>
#endif"

ac_subst_vars='SHELL
PATH_SEPARATOR
PACKAGE_NAME
PACKAGE_TARNAME
PACKAGE_VERSION
PACKAGE_STRING
PACKAGE_BUGREPORT
exec_prefix
prefix
program_transform_name
bindir
sbindir
libexecdir
datarootdir
datadir
sysconfdir
sharedstatedir
localstatedir
includedir
oldincludedir
docdir
infodir
htmldir
dvidir
pdfdir
psdir
libdir
localedir
mandir
DEFS
ECHO_C
ECHO_N
ECHO_T
LIBS
build_alias
host_alias
target_alias
VERSION
MAINT
CC
CFLAGS
LDFLAGS
CPPFLAGS
ac_ct_CC
EXEEXT
OBJEXT
INSTALL_PROGRAM
INSTALL_SCRIPT
INSTALL_DATA
LN_S
SET_MAKE
TTF_OPT
TEXMF
CPP
GREP
EGREP
LIBOBJS
LTLIBOBJS'
ac_subst_files=''
      ac_precious_vars='build_alias
host_alias
target_alias
CC
CFLAGS
LDFLAGS
CPPFLAGS
CPP'


# Initialize some variables set by options.
ac_init_help=
ac_init_version=false
# The variables have the same names as the options, with
# dashes changed to underlines.
cache_file=/dev/null
exec_prefix=NONE
no_create=
no_recursion=
prefix=NONE
program_prefix=NONE
program_suffix=NONE
program_transform_name=s,x,x,
silent=
site=
srcdir=
verbose=
x_includes=NONE
x_libraries=NONE

# Installation directory options.
# These are left unexpanded so users can "make install exec_prefix=/foo"
# and all the variables that are supposed to be based on exec_prefix
# by default will actually change.
# Use braces instead of parens because sh, perl, etc. also accept them.
# (The list follows the same order as the GNU Coding Standards.)
bindir='${exec_prefix}/bin'
sbindir='${exec_prefix}/sbin'
libexecdir='${exec_prefix}/libexec'
datarootdir='${prefix}/share'
datadir='${datarootdir}'
sysconfdir='${prefix}/etc'
sharedstatedir='${prefix}/com'
localstatedir='${prefix}/var'
includedir='${prefix}/include'
oldincludedir='/usr/include'
docdir='${datarootdir}/doc/${PACKAGE}'
infodir='${datarootdir}/info'
htmldir='${docdir}'
dvidir='${docdir}'
pdfdir='${docdir}'
psdir='${docdir}'
libdir='${exec_prefix}/lib'
localedir='${datarootdir}/locale'
mandir='${datarootdir}/man'

ac_prev=
ac_dashdash=
for ac_option
do
  # If the previous option needs an argument, assign it.
  if test -n "$ac_prev"; then
    eval $ac_prev=\$ac_option
    ac_prev=
    continue
  fi

  case $ac_option in
  *=*)	ac_optarg=`expr "X$ac_option" : '[^=]*=\(.*\)'` ;;
  *)	ac_optarg=yes ;;
  esac

  # Accept the important Cygnus configure options, so we can diagnose typos.

  case $ac_dashdash$ac_option in
  --)
    ac_dashdash=yes ;;

  -bindir | --bindir | --bindi | --bind | --bin | --bi)
    ac_prev=bindir ;;
  -bindir=* | --bindir=* | --bindi=* | --bind=* | --bin=* | --bi=*)
    bindir=$ac_optarg ;;

  -build | --build | --buil | --bui | --bu)
    ac_prev=build_alias ;;
  -build=* | --build=* | --buil=* | --bui=* | --bu=*)
    build_alias=$ac_optarg ;;

  -cache-file | --cache-file | --cache-fil | --cache-fi \
  | --cache-f | --cache- | --cache | --cach | --cac | --ca | --c)
    ac_prev=cache_file ;;
  -cache-file=* | --cache-file=* | --cache-fil=* | --cache-fi=* \
  | --cache-f=* | --cache-=* | --cache=* | --cach=* | --cac=* | --ca=* | --c=*)
    cache_file=$ac_optarg ;;

  --config-cache | -C)
    cache_file=config.cache ;;

  -datadir | --datadir | --datadi | --datad)
    ac_prev=datadir ;;
  -datadir=* | --datadir=* | --datadi=* | --datad=*)
    datadir=$ac_optarg ;;

  -datarootdir | --datarootdir | --datarootdi | --datarootd | --dataroot \
  | --dataroo | --dataro | --datar)
    ac_prev=datarootdir ;;
  -datarootdir=* | --datarootdir=* | --datarootdi=* | --datarootd=* \
  | --dataroot=* | --dataroo=* | --dataro=* | --datar=*)
    datarootdir=$ac_optarg ;;

  -disable-* | --disable-*)
    ac_feature=`expr "x$ac_option" : 'x-*disable-\(.*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_feature" : ".*[^-_$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid feature name: $ac_feature" >&2
   { (exit 1); exit 1; }; }
    ac_feature=`echo $ac_feature | sed 's/-/_/g'`
    eval enable_$ac_feature=no ;;

  -docdir | --docdir | --docdi | --doc | --do)
    ac_prev=docdir ;;
  -docdir=* | --docdir=* | --docdi=* | --doc=* | --do=*)
    docdir=$ac_optarg ;;

  -dvidir | --dvidir | --dvidi | --dvid | --dvi | --dv)
    ac_prev=dvidir ;;
  -dvidir=* | --dvidir=* | --dvidi=* | --dvid=* | --dvi=* | --dv=*)
    dvidir=$ac_optarg ;;

  -enable-* | --enable-*)
    ac_feature=`expr "x$ac_option" : 'x-*enable-\([^=]*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_feature" : ".*[^-_$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid feature name: $ac_feature" >&2
   { (exit 1); exit 1; }; }
    ac_feature=`echo $ac_feature | sed 's/-/_/g'`
    eval enable_$ac_feature=\$ac_optarg ;;

  -exec-prefix | --exec_prefix | --exec-prefix | --exec-prefi \
  | --exec-pref | --exec-pre | --exec-pr | --exec-p | --exec- \
  | --exec | --exe | --ex)
    ac_prev=exec_prefix ;;
  -exec-prefix=* | --exec_prefix=* | --exec-prefix=* | --exec-prefi=* \
  | --exec-pref=* | --exec-pre=* | --exec-pr=* | --exec-p=* | --exec-=* \
  | --exec=* | --exe=* | --ex=*)
    exec_prefix=$ac_optarg ;;

  -gas | --gas | --ga | --g)
    # Obsolete; use --with-gas.
    with_gas=yes ;;

  -help | --help | --hel | --he | -h)
    ac_init_help=long ;;
  -help=r* | --help=r* | --hel=r* | --he=r* | -hr*)
    ac_init_help=recursive ;;
  -help=s* | --help=s* | --hel=s* | --he=s* | -hs*)
    ac_init_help=short ;;

  -host | --host | --hos | --ho)
    ac_prev=host_alias ;;
  -host=* | --host=* | --hos=* | --ho=*)
    host_alias=$ac_optarg ;;

  -htmldir | --htmldir | --htmldi | --htmld | --html | --htm | --ht)
    ac_prev=htmldir ;;
  -htmldir=* | --htmldir=* | --htmldi=* | --htmld=* | --html=* | --htm=* \
  | --ht=*)
    htmldir=$ac_optarg ;;

  -includedir | --includedir | --includedi | --included | --include \
  | --includ | --inclu | --incl | --inc)
    ac_prev=includedir ;;
  -includedir=* | --includedir=* | --includedi=* | --included=* | --include=* \
  | --includ=* | --inclu=* | --incl=* | --inc=*)
    includedir=$ac_optarg ;;

  -infodir | --infodir | --infodi | --infod | --info | --inf)
    ac_prev=infodir ;;
  -infodir=* | --infodir=* | --infodi=* | --infod=* | --info=* | --inf=*)
    infodir=$ac_optarg ;;

  -libdir | --libdir | --libdi | --libd)
    ac_prev=libdir ;;
  -libdir=* | --libdir=* | --libdi=* | --libd=*)
    libdir=$ac_optarg ;;

  -libexecdir | --libexecdir | --libexecdi | --libexecd | --libexec \
  | --libexe | --libex | --libe)
    ac_prev=libexecdir ;;
  -libexecdir=* | --libexecdir=* | --libexecdi=* | --libexecd=* | --libexec=* \
  | --libexe=* | --libex=* | --libe=*)
    libexecdir=$ac_optarg ;;

  -localedir | --localedir | --localedi | --localed | --locale)
    ac_prev=localedir ;;
  -localedir=* | --localedir=* | --localedi=* | --localed=* | --locale=*)
    localedir=$ac_optarg ;;

  -localstatedir | --localstatedir | --localstatedi | --localstated \
  | --localstate | --localstat | --localsta | --localst | --locals)
    ac_prev=localstatedir ;;
  -localstatedir=* | --localstatedir=* | --localstatedi=* | --localstated=* \
  | --localstate=* | --localstat=* | --localsta=* | --localst=* | --locals=*)
    localstatedir=$ac_optarg ;;

  -mandir | --mandir | --mandi | --mand | --man | --ma | --m)
    ac_prev=mandir ;;
  -mandir=* | --mandir=* | --mandi=* | --mand=* | --man=* | --ma=* | --m=*)
    mandir=$ac_optarg ;;

  -nfp | --nfp | --nf)
    # Obsolete; use --without-fp.
    with_fp=no ;;

  -no-create | --no-create | --no-creat | --no-crea | --no-cre \
  | --no-cr | --no-c | -n)
    no_create=yes ;;

  -no-recursion | --no-recursion | --no-recursio | --no-recursi \
  | --no-recurs | --no-recur | --no-recu | --no-rec | --no-re | --no-r)
    no_recursion=yes ;;

  -oldincludedir | --oldincludedir | --oldincludedi | --oldincluded \
  | --oldinclude | --oldinclud | --oldinclu | --oldincl | --oldinc \
  | --oldin | --oldi | --old | --ol | --o)
    ac_prev=oldincludedir ;;
  -oldincludedir=* | --oldincludedir=* | --oldincludedi=* | --oldincluded=* \
  | --oldinclude=* | --oldinclud=* | --oldinclu=* | --oldincl=* | --oldinc=* \
  | --oldin=* | --oldi=* | --old=* | --ol=* | --o=*)
    oldincludedir=$ac_optarg ;;

  -prefix | --prefix | --prefi | --pref | --pre | --pr | --p)
    ac_prev=prefix ;;
  -prefix=* | --prefix=* | --prefi=* | --pref=* | --pre=* | --pr=* | --p=*)
    prefix=$ac_optarg ;;

  -program-prefix | --program-prefix | --program-prefi | --program-pref \
  | --program-pre | --program-pr | --program-p)
    ac_prev=program_prefix ;;
  -program-prefix=* | --program-prefix=* | --program-prefi=* \
  | --program-pref=* | --program-pre=* | --program-pr=* | --program-p=*)
    program_prefix=$ac_optarg ;;

  -program-suffix | --program-suffix | --program-suffi | --program-suff \
  | --program-suf | --program-su | --program-s)
    ac_prev=program_suffix ;;
  -program-suffix=* | --program-suffix=* | --program-suffi=* \
  | --program-suff=* | --program-suf=* | --program-su=* | --program-s=*)
    program_suffix=$ac_optarg ;;

  -program-transform-name | --program-transform-name \
  | --program-transform-nam | --program-transform-na \
  | --program-transform-n | --program-transform- \
  | --program-transform | --program-transfor \
  | --program-transfo | --program-transf \
  | --program-trans | --program-tran \
  | --progr-tra | --program-tr | --program-t)
    ac_prev=program_transform_name ;;
  -program-transform-name=* | --program-transform-name=* \
  | --program-transform-nam=* | --program-transform-na=* \
  | --program-transform-n=* | --program-transform-=* \
  | --program-transform=* | --program-transfor=* \
  | --program-transfo=* | --program-transf=* \
  | --program-trans=* | --program-tran=* \
  | --progr-tra=* | --program-tr=* | --program-t=*)
    program_transform_name=$ac_optarg ;;

  -pdfdir | --pdfdir | --pdfdi | --pdfd | --pdf | --pd)
    ac_prev=pdfdir ;;
  -pdfdir=* | --pdfdir=* | --pdfdi=* | --pdfd=* | --pdf=* | --pd=*)
    pdfdir=$ac_optarg ;;

  -psdir | --psdir | --psdi | --psd | --ps)
    ac_prev=psdir ;;
  -psdir=* | --psdir=* | --psdi=* | --psd=* | --ps=*)
    psdir=$ac_optarg ;;

  -q | -quiet | --quiet | --quie | --qui | --qu | --q \
  | -silent | --silent | --silen | --sile | --sil)
    silent=yes ;;

  -sbindir | --sbindir | --sbindi | --sbind | --sbin | --sbi | --sb)
    ac_prev=sbindir ;;
  -sbindir=* | --sbindir=* | --sbindi=* | --sbind=* | --sbin=* \
  | --sbi=* | --sb=*)
    sbindir=$ac_optarg ;;

  -sharedstatedir | --sharedstatedir | --sharedstatedi \
  | --sharedstated | --sharedstate | --sharedstat | --sharedsta \
  | --sharedst | --shareds | --shared | --share | --shar \
  | --sha | --sh)
    ac_prev=sharedstatedir ;;
  -sharedstatedir=* | --sharedstatedir=* | --sharedstatedi=* \
  | --sharedstated=* | --sharedstate=* | --sharedstat=* | --sharedsta=* \
  | --sharedst=* | --shareds=* | --shared=* | --share=* | --shar=* \
  | --sha=* | --sh=*)
    sharedstatedir=$ac_optarg ;;

  -site | --site | --sit)
    ac_prev=site ;;
  -site=* | --site=* | --sit=*)
    site=$ac_optarg ;;

  -srcdir | --srcdir | --srcdi | --srcd | --src | --sr)
    ac_prev=srcdir ;;
  -srcdir=* | --srcdir=* | --srcdi=* | --srcd=* | --src=* | --sr=*)
    srcdir=$ac_optarg ;;

  -sysconfdir | --sysconfdir | --sysconfdi | --sysconfd | --sysconf \
  | --syscon | --sysco | --sysc | --sys | --sy)
    ac_prev=sysconfdir ;;
  -sysconfdir=* | --sysconfdir=* | --sysconfdi=* | --sysconfd=* | --sysconf=* \
  | --syscon=* | --sysco=* | --sysc=* | --sys=* | --sy=*)
    sysconfdir=$ac_optarg ;;

  -target | --target | --targe | --targ | --tar | --ta | --t)
    ac_prev=target_alias ;;
  -target=* | --target=* | --targe=* | --targ=* | --tar=* | --ta=* | --t=*)
    target_alias=$ac_optarg ;;

  -v | -verbose | --verbose | --verbos | --verbo | --verb)
    verbose=yes ;;

  -version | --version | --versio | --versi | --vers | -V)
    ac_init_version=: ;;

  -with-* | --with-*)
    ac_package=`expr "x$ac_option" : 'x-*with-\([^=]*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_package" : ".*[^-_$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid package name: $ac_package" >&2
   { (exit 1); exit 1; }; }
    ac_package=`echo $ac_package| sed 's/-/_/g'`
    eval with_$ac_package=\$ac_optarg ;;

  -without-* | --without-*)
    ac_package=`expr "x$ac_option" : 'x-*without-\(.*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_package" : ".*[^-_$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid package name: $ac_package" >&2
   { (exit 1); exit 1; }; }
    ac_package=`echo $ac_package | sed 's/-/_/g'`
    eval with_$ac_package=no ;;

  --x)
    # Obsolete; use --with-x.
    with_x=yes ;;

  -x-includes | --x-includes | --x-include | --x-includ | --x-inclu \
  | --x-incl | --x-inc | --x-in | --x-i)
    ac_prev=x_includes ;;
  -x-includes=* | --x-includes=* | --x-include=* | --x-includ=* | --x-inclu=* \
  | --x-incl=* | --x-inc=* | --x-in=* | --x-i=*)
    x_includes=$ac_optarg ;;

  -x-libraries | --x-libraries | --x-librarie | --x-librari \
  | --x-librar | --x-libra | --x-libr | --x-lib | --x-li | --x-l)
    ac_prev=x_libraries ;;
  -x-libraries=* | --x-libraries=* | --x-librarie=* | --x-librari=* \
  | --x-librar=* | --x-libra=* | --x-libr=* | --x-lib=* | --x-li=* | --x-l=*)
    x_libraries=$ac_optarg ;;

  -*) { echo "$as_me: error: unrecognized option: $ac_option
Try \`$0 --help' for more information." >&2
   { (exit 1); exit 1; }; }
    ;;

  *=*)
    ac_envvar=`expr "x$ac_option" : 'x\([^=]*\)='`
    # Reject names that are not valid shell variable names.
    expr "x$ac_envvar" : ".*[^_$as_cr_alnum]" >/dev/null &&
      { echo "$as_me: error: invalid variable name: $ac_envvar" >&2
   { (exit 1); exit 1; }; }
    eval $ac_envvar=\$ac_optarg
    export $ac_envvar ;;

  *)
    # FIXME: should be removed in autoconf 3.0.
    echo "$as_me: WARNING: you should use --build, --host, --target" >&2
    expr "x$ac_option" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      echo "$as_me: WARNING: invalid host type: $ac_option" >&2
    : ${build_alias=$ac_option} ${host_alias=$ac_option} ${target_alias=$ac_option}
    ;;

  esac
done

if test -n "$ac_prev"; then
  ac_option=--`echo $ac_prev | sed 's/_/-/g'`
  { echo "$as_me: error: missing argument to $ac_option" >&2
   { (exit 1); exit 1; }; }
fi

# Be sure to have absolute directory names.
for ac_var in	exec_prefix prefix bindir sbindir libexecdir datarootdir \
		datadir sysconfdir sharedstatedir localstatedir includedir \
		oldincludedir docdir infodir htmldir dvidir pdfdir psdir \
		libdir localedir mandir
do
  eval ac_val=\$$ac_var
  case $ac_val in
    [\\/$]* | ?:[\\/]* )  continue;;
    NONE | '' ) case $ac_var in *prefix ) continue;; esac;;
  esac
  { echo "$as_me: error: expected an absolute directory name for --$ac_var: $ac_val" >&2
   { (exit 1); exit 1; }; }
done

# There might be people who depend on the old broken behavior: `$host'
# used to hold the argument of --host etc.
# FIXME: To remove some day.
build=$build_alias
host=$host_alias
target=$target_alias

# FIXME: To remove some day.
if test "x$host_alias" != x; then
  if test "x$build_alias" = x; then
    cross_compiling=maybe
    echo "$as_me: WARNING: If you wanted to set the --build type, don't use --host.
    If a cross compiler is detected then cross compile mode will be used." >&2
  elif test "x$build_alias" != "x$host_alias"; then
    cross_compiling=yes
  fi
fi

ac_tool_prefix=
test -n "$host_alias" && ac_tool_prefix=$host_alias-

test "$silent" = yes && exec 6>/dev/null


ac_pwd=`pwd` && test -n "$ac_pwd" &&
ac_ls_di=`ls -di .` &&
ac_pwd_ls_di=`cd "$ac_pwd" && ls -di .` ||
  { echo "$as_me: error: Working directory cannot be determined" >&2
   { (exit 1); exit 1; }; }
test "X$ac_ls_di" = "X$ac_pwd_ls_di" ||
  { echo "$as_me: error: pwd does not report name of working directory" >&2
   { (exit 1); exit 1; }; }


# Find the source files, if location was not specified.
if test -z "$srcdir"; then
  ac_srcdir_defaulted=yes
  # Try the directory containing this script, then the parent directory.
  ac_confdir=`$as_dirname -- "$0" ||
$as_expr X"$0" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$0" : 'X\(//\)[^/]' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$0" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  srcdir=$ac_confdir
  if test ! -r "$srcdir/$ac_unique_file"; then
    srcdir=..
  fi
else
  ac_srcdir_defaulted=no
fi
if test ! -r "$srcdir/$ac_unique_file"; then
  test "$ac_srcdir_defaulted" = yes && srcdir="$ac_confdir or .."
  { echo "$as_me: error: cannot find sources ($ac_unique_file) in $srcdir" >&2
   { (exit 1); exit 1; }; }
fi
ac_msg="sources are in $srcdir, but \`cd $srcdir' does not work"
ac_abs_confdir=`(
	cd "$srcdir" && test -r "./$ac_unique_file" || { echo "$as_me: error: $ac_msg" >&2
   { (exit 1); exit 1; }; }
	pwd)`
# When building in place, set srcdir=.
if test "$ac_abs_confdir" = "$ac_pwd"; then
  srcdir=.
fi
# Remove unnecessary trailing slashes from srcdir.
# Double slashes in file names in object file debugging info
# mess up M-x gdb in Emacs.
case $srcdir in
*/) srcdir=`expr "X$srcdir" : 'X\(.*[^/]\)' \| "X$srcdir" : 'X\(.*\)'`;;
esac
for ac_var in $ac_precious_vars; do
  eval ac_env_${ac_var}_set=\${${ac_var}+set}
  eval ac_env_${ac_var}_value=\$${ac_var}
  eval ac_cv_env_${ac_var}_set=\${${ac_var}+set}
  eval ac_cv_env_${ac_var}_value=\$${ac_var}
done

#
# Report the --help message.
#
if test "$ac_init_help" = "long"; then
  # Omit some internal or obsolete options to make the list less imposing.
  # This message is too long to be a string in the A/UX 3.1 sh.
  cat <<_ACEOF
\`configure' configures this package to adapt to many kinds of systems.

Usage: $0 [OPTION]... [VAR=VALUE]...

To assign environment variables (e.g., CC, CFLAGS...), specify them as
VAR=VALUE.  See below for descriptions of some of the useful variables.

Defaults for the options are specified in brackets.

Configuration:
  -h, --help              display this help and exit
      --help=short        display options specific to this package
      --help=recursive    display the short help of all the included packages
  -V, --version           display version information and exit
  -q, --quiet, --silent   do not print \`checking...' messages
      --cache-file=FILE   cache test results in FILE [disabled]
  -C, --config-cache      alias for \`--cache-file=config.cache'
  -n, --no-create         do not create output files
      --srcdir=DIR        find the sources in DIR [configure dir or \`..']

Installation directories:
  --prefix=PREFIX         install architecture-independent files in PREFIX
			  [$ac_default_prefix]
  --exec-prefix=EPREFIX   install architecture-dependent files in EPREFIX
			  [PREFIX]

By default, \`make install' will install all the files in
\`$ac_default_prefix/bin', \`$ac_default_prefix/lib' etc.  You can specify
an installation prefix other than \`$ac_default_prefix' using \`--prefix',
for instance \`--prefix=\$HOME'.

For better control, use the options below.

Fine tuning of the installation directories:
  --bindir=DIR           user executables [EPREFIX/bin]
  --sbindir=DIR          system admin executables [EPREFIX/sbin]
  --libexecdir=DIR       program executables [EPREFIX/libexec]
  --sysconfdir=DIR       read-only single-machine data [PREFIX/etc]
  --sharedstatedir=DIR   modifiable architecture-independent data [PREFIX/com]
  --localstatedir=DIR    modifiable single-machine data [PREFIX/var]
  --libdir=DIR           object code libraries [EPREFIX/lib]
  --includedir=DIR       C header files [PREFIX/include]
  --oldincludedir=DIR    C header files for non-gcc [/usr/include]
  --datarootdir=DIR      read-only arch.-independent data root [PREFIX/share]
  --datadir=DIR          read-only architecture-independent data [DATAROOTDIR]
  --infodir=DIR          info documentation [DATAROOTDIR/info]
  --localedir=DIR        locale-dependent data [DATAROOTDIR/locale]
  --mandir=DIR           man documentation [DATAROOTDIR/man]
  --docdir=DIR           documentation root [DATAROOTDIR/doc/PACKAGE]
  --htmldir=DIR          html documentation [DOCDIR]
  --dvidir=DIR           dvi documentation [DOCDIR]
  --pdfdir=DIR           pdf documentation [DOCDIR]
  --psdir=DIR            ps documentation [DOCDIR]
_ACEOF

  cat <<\_ACEOF
_ACEOF
fi

if test -n "$ac_init_help"; then

  cat <<\_ACEOF

Optional Features:
  --disable-FEATURE       do not include FEATURE (same as --enable-FEATURE=no)
  --enable-FEATURE[=ARG]  include FEATURE [ARG=yes]
  --enable-maint          enable autoconf portions of Makefile

Optional Packages:
  --with-PACKAGE[=ARG]    use PACKAGE [ARG=yes]
  --without-PACKAGE       do not use PACKAGE (same as --with-PACKAGE=no)
  --with-kpathsea=DIR     use kpathsea include/library files from DIR
  --with-png=DIR          use png include/library files from DIR
  --with-zlib=DIR         use zlib include/library files from DIR

Some influential environment variables:
  CC          C compiler command
  CFLAGS      C compiler flags
  LDFLAGS     linker flags, e.g. -L<lib dir> if you have libraries in a
              nonstandard directory <lib dir>
  CPPFLAGS    C/C++/Objective C preprocessor flags, e.g. -I<include dir> if
              you have headers in a nonstandard directory <include dir>
  CPP         C preprocessor

Use these variables to override the choices made by `configure' or to help
it to find libraries and programs with nonstandard names/locations.

_ACEOF
ac_status=$?
fi

if test "$ac_init_help" = "recursive"; then
  # If there are subdirs, report their specific --help.
  for ac_dir in : $ac_subdirs_all; do test "x$ac_dir" = x: && continue
    test -d "$ac_dir" || continue
    ac_builddir=.

case "$ac_dir" in
.) ac_dir_suffix= ac_top_builddir_sub=. ac_top_build_prefix= ;;
*)
  ac_dir_suffix=/`echo "$ac_dir" | sed 's,^\.[\\/],,'`
  # A ".." for each directory in $ac_dir_suffix.
  ac_top_builddir_sub=`echo "$ac_dir_suffix" | sed 's,/[^\\/]*,/..,g;s,/,,'`
  case $ac_top_builddir_sub in
  "") ac_top_builddir_sub=. ac_top_build_prefix= ;;
  *)  ac_top_build_prefix=$ac_top_builddir_sub/ ;;
  esac ;;
esac
ac_abs_top_builddir=$ac_pwd
ac_abs_builddir=$ac_pwd$ac_dir_suffix
# for backward compatibility:
ac_top_builddir=$ac_top_build_prefix

case $srcdir in
  .)  # We are building in place.
    ac_srcdir=.
    ac_top_srcdir=$ac_top_builddir_sub
    ac_abs_top_srcdir=$ac_pwd ;;
  [\\/]* | ?:[\\/]* )  # Absolute name.
    ac_srcdir=$srcdir$ac_dir_suffix;
    ac_top_srcdir=$srcdir
    ac_abs_top_srcdir=$srcdir ;;
  *) # Relative name.
    ac_srcdir=$ac_top_build_prefix$srcdir$ac_dir_suffix
    ac_top_srcdir=$ac_top_build_prefix$srcdir
    ac_abs_top_srcdir=$ac_pwd/$srcdir ;;
esac
ac_abs_srcdir=$ac_abs_top_srcdir$ac_dir_suffix

    cd "$ac_dir" || { ac_status=$?; continue; }
    # Check for guested configure.
    if test -f "$ac_srcdir/configure.gnu"; then
      echo &&
      $SHELL "$ac_srcdir/configure.gnu" --help=recursive
    elif test -f "$ac_srcdir/configure"; then
      echo &&
      $SHELL "$ac_srcdir/configure" --help=recursive
    else
      echo "$as_me: WARNING: no configuration information is in $ac_dir" >&2
    fi || ac_status=$?
    cd "$ac_pwd" || { ac_status=$?; break; }
  done
fi

test -n "$ac_init_help" && exit $ac_status
if $ac_init_version; then
  cat <<\_ACEOF
configure
generated by GNU Autoconf 2.60

Copyright (C) 1992, 1993, 1994, 1995, 1996, 1998, 1999, 2000, 2001,
2002, 2003, 2004, 2005, 2006 Free Software Foundation, Inc.
This configure script is free software; the Free Software Foundation
gives unlimited permission to copy, distribute and modify it.
_ACEOF
  exit
fi
cat >config.log <<_ACEOF
This file contains any messages produced by compilers while
running configure, to aid debugging if configure makes a mistake.

It was created by $as_me, which was
generated by GNU Autoconf 2.60.  Invocation command line was

  $ $0 $@

_ACEOF
exec 5>>config.log
{
cat <<_ASUNAME
## --------- ##
## Platform. ##
## --------- ##

hostname = `(hostname || uname -n) 2>/dev/null | sed 1q`
uname -m = `(uname -m) 2>/dev/null || echo unknown`
uname -r = `(uname -r) 2>/dev/null || echo unknown`
uname -s = `(uname -s) 2>/dev/null || echo unknown`
uname -v = `(uname -v) 2>/dev/null || echo unknown`

/usr/bin/uname -p = `(/usr/bin/uname -p) 2>/dev/null || echo unknown`
/bin/uname -X     = `(/bin/uname -X) 2>/dev/null     || echo unknown`

/bin/arch              = `(/bin/arch) 2>/dev/null              || echo unknown`
/usr/bin/arch -k       = `(/usr/bin/arch -k) 2>/dev/null       || echo unknown`
/usr/convex/getsysinfo = `(/usr/convex/getsysinfo) 2>/dev/null || echo unknown`
/usr/bin/hostinfo      = `(/usr/bin/hostinfo) 2>/dev/null      || echo unknown`
/bin/machine           = `(/bin/machine) 2>/dev/null           || echo unknown`
/usr/bin/oslevel       = `(/usr/bin/oslevel) 2>/dev/null       || echo unknown`
/bin/universe          = `(/bin/universe) 2>/dev/null          || echo unknown`

_ASUNAME

as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  echo "PATH: $as_dir"
done
IFS=$as_save_IFS

} >&5

cat >&5 <<_ACEOF


## ----------- ##
## Core tests. ##
## ----------- ##

_ACEOF


# Keep a trace of the command line.
# Strip out --no-create and --no-recursion so they do not pile up.
# Strip out --silent because we don't want to record it for future runs.
# Also quote any args containing shell meta-characters.
# Make two passes to allow for proper duplicate-argument suppression.
ac_configure_args=
ac_configure_args0=
ac_configure_args1=
ac_must_keep_next=false
for ac_pass in 1 2
do
  for ac_arg
  do
    case $ac_arg in
    -no-create | --no-c* | -n | -no-recursion | --no-r*) continue ;;
    -q | -quiet | --quiet | --quie | --qui | --qu | --q \
    | -silent | --silent | --silen | --sile | --sil)
      continue ;;
    *\'*)
      ac_arg=`echo "$ac_arg" | sed "s/'/'\\\\\\\\''/g"` ;;
    esac
    case $ac_pass in
    1) ac_configure_args0="$ac_configure_args0 '$ac_arg'" ;;
    2)
      ac_configure_args1="$ac_configure_args1 '$ac_arg'"
      if test $ac_must_keep_next = true; then
	ac_must_keep_next=false # Got value, back to normal.
      else
	case $ac_arg in
	  *=* | --config-cache | -C | -disable-* | --disable-* \
	  | -enable-* | --enable-* | -gas | --g* | -nfp | --nf* \
	  | -q | -quiet | --q* | -silent | --sil* | -v | -verb* \
	  | -with-* | --with-* | -without-* | --without-* | --x)
	    case "$ac_configure_args0 " in
	      "$ac_configure_args1"*" '$ac_arg' "* ) continue ;;
	    esac
	    ;;
	  -* ) ac_must_keep_next=true ;;
	esac
      fi
      ac_configure_args="$ac_configure_args '$ac_arg'"
      ;;
    esac
  done
done
$as_unset ac_configure_args0 || test "${ac_configure_args0+set}" != set || { ac_configure_args0=; export ac_configure_args0; }
$as_unset ac_configure_args1 || test "${ac_configure_args1+set}" != set || { ac_configure_args1=; export ac_configure_args1; }

# When interrupted or exit'd, cleanup temporary files, and complete
# config.log.  We remove comments because anyway the quotes in there
# would cause problems or look ugly.
# WARNING: Use '\'' to represent an apostrophe within the trap.
# WARNING: Do not start the trap code with a newline, due to a FreeBSD 4.0 bug.
trap 'exit_status=$?
  # Save into config.log some information that might help in debugging.
  {
    echo

    cat <<\_ASBOX
## ---------------- ##
## Cache variables. ##
## ---------------- ##
_ASBOX
    echo
    # The following way of writing the cache mishandles newlines in values,
(
  for ac_var in `(set) 2>&1 | sed -n '\''s/^\([a-zA-Z_][a-zA-Z0-9_]*\)=.*/\1/p'\''`; do
    eval ac_val=\$$ac_var
    case $ac_val in #(
    *${as_nl}*)
      case $ac_var in #(
      *_cv_*) { echo "$as_me:$LINENO: WARNING: Cache variable $ac_var contains a newline." >&5
echo "$as_me: WARNING: Cache variable $ac_var contains a newline." >&2;} ;;
      esac
      case $ac_var in #(
      _ | IFS | as_nl) ;; #(
      *) $as_unset $ac_var ;;
      esac ;;
    esac
  done
  (set) 2>&1 |
    case $as_nl`(ac_space='\'' '\''; set) 2>&1` in #(
    *${as_nl}ac_space=\ *)
      sed -n \
	"s/'\''/'\''\\\\'\'''\''/g;
	  s/^\\([_$as_cr_alnum]*_cv_[_$as_cr_alnum]*\\)=\\(.*\\)/\\1='\''\\2'\''/p"
      ;; #(
    *)
      sed -n "/^[_$as_cr_alnum]*_cv_[_$as_cr_alnum]*=/p"
      ;;
    esac |
    sort
)
    echo

    cat <<\_ASBOX
## ----------------- ##
## Output variables. ##
## ----------------- ##
_ASBOX
    echo
    for ac_var in $ac_subst_vars
    do
      eval ac_val=\$$ac_var
      case $ac_val in
      *\'\''*) ac_val=`echo "$ac_val" | sed "s/'\''/'\''\\\\\\\\'\'''\''/g"`;;
      esac
      echo "$ac_var='\''$ac_val'\''"
    done | sort
    echo

    if test -n "$ac_subst_files"; then
      cat <<\_ASBOX
## ------------------- ##
## File substitutions. ##
## ------------------- ##
_ASBOX
      echo
      for ac_var in $ac_subst_files
      do
	eval ac_val=\$$ac_var
	case $ac_val in
	*\'\''*) ac_val=`echo "$ac_val" | sed "s/'\''/'\''\\\\\\\\'\'''\''/g"`;;
	esac
	echo "$ac_var='\''$ac_val'\''"
      done | sort
      echo
    fi

    if test -s confdefs.h; then
      cat <<\_ASBOX
## ----------- ##
## confdefs.h. ##
## ----------- ##
_ASBOX
      echo
      cat confdefs.h
      echo
    fi
    test "$ac_signal" != 0 &&
      echo "$as_me: caught signal $ac_signal"
    echo "$as_me: exit $exit_status"
  } >&5
  rm -f core *.core core.conftest.* &&
    rm -f -r conftest* confdefs* conf$$* $ac_clean_files &&
    exit $exit_status
' 0
for ac_signal in 1 2 13 15; do
  trap 'ac_signal='$ac_signal'; { (exit 1); exit 1; }' $ac_signal
done
ac_signal=0

# confdefs.h avoids OS command line length limits that DEFS can exceed.
rm -f -r conftest* confdefs.h

# Predefined preprocessor variables.

cat >>confdefs.h <<_ACEOF
#define PACKAGE_NAME "$PACKAGE_NAME"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_TARNAME "$PACKAGE_TARNAME"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_VERSION "$PACKAGE_VERSION"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_STRING "$PACKAGE_STRING"
_ACEOF


cat >>confdefs.h <<_ACEOF
#define PACKAGE_BUGREPORT "$PACKAGE_BUGREPORT"
_ACEOF


# Let the site file select an alternate cache file if it wants to.
# Prefer explicitly selected file to automatically selected ones.
if test -n "$CONFIG_SITE"; then
  set x "$CONFIG_SITE"
elif test "x$prefix" != xNONE; then
  set x "$prefix/share/config.site" "$prefix/etc/config.site"
else
  set x "$ac_default_prefix/share/config.site" \
	"$ac_default_prefix/etc/config.site"
fi
shift
for ac_site_file
do
  if test -r "$ac_site_file"; then
    { echo "$as_me:$LINENO: loading site script $ac_site_file" >&5
echo "$as_me: loading site script $ac_site_file" >&6;}
    sed 's/^/| /' "$ac_site_file" >&5
    . "$ac_site_file"
  fi
done

if test -r "$cache_file"; then
  # Some versions of bash will fail to source /dev/null (special
  # files actually), so we avoid doing that.
  if test -f "$cache_file"; then
    { echo "$as_me:$LINENO: loading cache $cache_file" >&5
echo "$as_me: loading cache $cache_file" >&6;}
    case $cache_file in
      [\\/]* | ?:[\\/]* ) . "$cache_file";;
      *)                      . "./$cache_file";;
    esac
  fi
else
  { echo "$as_me:$LINENO: creating cache $cache_file" >&5
echo "$as_me: creating cache $cache_file" >&6;}
  >$cache_file
fi

# Check that the precious variables saved in the cache have kept the same
# value.
ac_cache_corrupted=false
for ac_var in $ac_precious_vars; do
  eval ac_old_set=\$ac_cv_env_${ac_var}_set
  eval ac_new_set=\$ac_env_${ac_var}_set
  eval ac_old_val=\$ac_cv_env_${ac_var}_value
  eval ac_new_val=\$ac_env_${ac_var}_value
  case $ac_old_set,$ac_new_set in
    set,)
      { echo "$as_me:$LINENO: error: \`$ac_var' was set to \`$ac_old_val' in the previous run" >&5
echo "$as_me: error: \`$ac_var' was set to \`$ac_old_val' in the previous run" >&2;}
      ac_cache_corrupted=: ;;
    ,set)
      { echo "$as_me:$LINENO: error: \`$ac_var' was not set in the previous run" >&5
echo "$as_me: error: \`$ac_var' was not set in the previous run" >&2;}
      ac_cache_corrupted=: ;;
    ,);;
    *)
      if test "x$ac_old_val" != "x$ac_new_val"; then
	{ echo "$as_me:$LINENO: error: \`$ac_var' has changed since the previous run:" >&5
echo "$as_me: error: \`$ac_var' has changed since the previous run:" >&2;}
	{ echo "$as_me:$LINENO:   former value:  $ac_old_val" >&5
echo "$as_me:   former value:  $ac_old_val" >&2;}
	{ echo "$as_me:$LINENO:   current value: $ac_new_val" >&5
echo "$as_me:   current value: $ac_new_val" >&2;}
	ac_cache_corrupted=:
      fi;;
  esac
  # Pass precious variables to config.status.
  if test "$ac_new_set" = set; then
    case $ac_new_val in
    *\'*) ac_arg=$ac_var=`echo "$ac_new_val" | sed "s/'/'\\\\\\\\''/g"` ;;
    *) ac_arg=$ac_var=$ac_new_val ;;
    esac
    case " $ac_configure_args " in
      *" '$ac_arg' "*) ;; # Avoid dups.  Use of quotes ensures accuracy.
      *) ac_configure_args="$ac_configure_args '$ac_arg'" ;;
    esac
  fi
done
if $ac_cache_corrupted; then
  { echo "$as_me:$LINENO: error: changes in the environment can compromise the build" >&5
echo "$as_me: error: changes in the environment can compromise the build" >&2;}
  { { echo "$as_me:$LINENO: error: run \`make distclean' and/or \`rm $cache_file' and start over" >&5
echo "$as_me: error: run \`make distclean' and/or \`rm $cache_file' and start over" >&2;}
   { (exit 1); exit 1; }; }
fi

















ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu





VERSION="0.13.2d"

cat >>confdefs.h <<\_ACEOF
#define VERSION "0.13.2d"
_ACEOF

cat >>confdefs.h <<\_ACEOF
#define PACKAGE "dvipdfm"
_ACEOF


ac_config_headers="$ac_config_headers config.h"


# Check whether --enable-maint was given.
if test "${enable_maint+set}" = set; then
  enableval=$enable_maint; MAINT=''
else
  MAINT='#'
fi



ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu
if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}gcc", so it can be a program name with args.
set dummy ${ac_tool_prefix}gcc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_executable_p "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CC="${ac_tool_prefix}gcc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$ac_cv_prog_CC"; then
  ac_ct_CC=$CC
  # Extract the first word of "gcc", so it can be a program name with args.
set dummy gcc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_executable_p "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_CC="gcc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { echo "$as_me:$LINENO: result: $ac_ct_CC" >&5
echo "${ECHO_T}$ac_ct_CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
else
  CC="$ac_cv_prog_CC"
fi

if test -z "$CC"; then
          if test -n "$ac_tool_prefix"; then
    # Extract the first word of "${ac_tool_prefix}cc", so it can be a program name with args.
set dummy ${ac_tool_prefix}cc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_executable_p "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CC="${ac_tool_prefix}cc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  fi
fi
if test -z "$CC"; then
  # Extract the first word of "cc", so it can be a program name with args.
set dummy cc; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
  ac_prog_rejected=no
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_executable_p "$as_dir/$ac_word$ac_exec_ext"; }; then
    if test "$as_dir/$ac_word$ac_exec_ext" = "/usr/ucb/cc"; then
       ac_prog_rejected=yes
       continue
     fi
    ac_cv_prog_CC="cc"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

if test $ac_prog_rejected = yes; then
  # We found a bogon in the path, so make sure we never use it.
  set dummy $ac_cv_prog_CC
  shift
  if test $# != 0; then
    # We chose a different compiler from the bogus one.
    # However, it has the same basename, so the bogon will be chosen
    # first if we set CC to just the basename; use the full file name.
    shift
    ac_cv_prog_CC="$as_dir/$ac_word${1+' '}$@"
  fi
fi
fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


fi
if test -z "$CC"; then
  if test -n "$ac_tool_prefix"; then
  for ac_prog in cl.exe
  do
    # Extract the first word of "$ac_tool_prefix$ac_prog", so it can be a program name with args.
set dummy $ac_tool_prefix$ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_executable_p "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_CC="$ac_tool_prefix$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { echo "$as_me:$LINENO: result: $CC" >&5
echo "${ECHO_T}$CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


    test -n "$CC" && break
  done
fi
if test -z "$CC"; then
  ac_ct_CC=$CC
  for ac_prog in cl.exe
do
  # Extract the first word of "$ac_prog", so it can be a program name with args.
set dummy $ac_prog; ac_word=$2
{ echo "$as_me:$LINENO: checking for $ac_word" >&5
echo $ECHO_N "checking for $ac_word... $ECHO_C" >&6; }
if test "${ac_cv_prog_ac_ct_CC+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_exec_ext in '' $ac_executable_extensions; do
  if { test -f "$as_dir/$ac_word$ac_exec_ext" && $as_executable_p "$as_dir/$ac_word$ac_exec_ext"; }; then
    ac_cv_prog_ac_ct_CC="$ac_prog"
    echo "$as_me:$LINENO: found $as_dir/$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { echo "$as_me:$LINENO: result: $ac_ct_CC" >&5
echo "${ECHO_T}$ac_ct_CC" >&6; }
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi


  test -n "$ac_ct_CC" && break
done

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ echo "$as_me:$LINENO: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&5
echo "$as_me: WARNING: In the future, Autoconf will not detect cross-tools
whose name does not start with the host triplet.  If you think this
configuration is useful to you, please write to autoconf@gnu.org." >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
fi

fi


test -z "$CC" && { { echo "$as_me:$LINENO: error: no acceptable C compiler found in \$PATH
See \`config.log' for more details." >&5
echo "$as_me: error: no acceptable C compiler found in \$PATH
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }

# Provide some information about the compiler.
echo "$as_me:$LINENO: checking for C compiler version" >&5
ac_compiler=`set X $ac_compile; echo $2`
{ (ac_try="$ac_compiler --version >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler --version >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -v >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -v >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }
{ (ac_try="$ac_compiler -V >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compiler -V >&5") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }

cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
ac_clean_files_save=$ac_clean_files
ac_clean_files="$ac_clean_files a.out a.exe b.out"
# Try to create an executable without -o first, disregard a.out.
# It will help us diagnose broken compilers, and finding out an intuition
# of exeext.
{ echo "$as_me:$LINENO: checking for C compiler default output file name" >&5
echo $ECHO_N "checking for C compiler default output file name... $ECHO_C" >&6; }
ac_link_default=`echo "$ac_link" | sed 's/ -o *conftest[^ ]*//'`
#
# List of possible output files, starting from the most likely.
# The algorithm is not robust to junk in `.', hence go to wildcards (a.*)
# only as a last resort.  b.out is created by i960 compilers.
ac_files='a_out.exe a.exe conftest.exe a.out conftest a.* conftest.* b.out'
#
# The IRIX 6 linker writes into existing files which may not be
# executable, retaining their permissions.  Remove them first so a
# subsequent execution test works.
ac_rmfiles=
for ac_file in $ac_files
do
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.o | *.obj ) ;;
    * ) ac_rmfiles="$ac_rmfiles $ac_file";;
  esac
done
rm -f $ac_rmfiles

if { (ac_try="$ac_link_default"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link_default") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  # Autoconf-2.13 could set the ac_cv_exeext variable to `no'.
# So ignore a value of `no', otherwise this would lead to `EXEEXT = no'
# in a Makefile.  We should not override ac_cv_exeext if it was cached,
# so that the user can short-circuit this test for compilers unknown to
# Autoconf.
for ac_file in $ac_files
do
  test -f "$ac_file" || continue
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.o | *.obj )
	;;
    [ab].out )
	# We found the default executable, but exeext='' is most
	# certainly right.
	break;;
    *.* )
        if test "${ac_cv_exeext+set}" = set && test "$ac_cv_exeext" != no;
	then :; else
	   ac_cv_exeext=`expr "$ac_file" : '[^.]*\(\..*\)'`
	fi
	# We set ac_cv_exeext here because the later test for it is not
	# safe: cross compilers may not add the suffix if given an `-o'
	# argument, so we may need to know it at that point already.
	# Even if this section looks crufty: it has the advantage of
	# actually working.
	break;;
    * )
	break;;
  esac
done
test "$ac_cv_exeext" = no && ac_cv_exeext=

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

{ { echo "$as_me:$LINENO: error: C compiler cannot create executables
See \`config.log' for more details." >&5
echo "$as_me: error: C compiler cannot create executables
See \`config.log' for more details." >&2;}
   { (exit 77); exit 77; }; }
fi

ac_exeext=$ac_cv_exeext
{ echo "$as_me:$LINENO: result: $ac_file" >&5
echo "${ECHO_T}$ac_file" >&6; }

# Check that the compiler produces executables we can run.  If not, either
# the compiler is broken, or we cross compile.
{ echo "$as_me:$LINENO: checking whether the C compiler works" >&5
echo $ECHO_N "checking whether the C compiler works... $ECHO_C" >&6; }
# FIXME: These cross compiler hacks should be removed for Autoconf 3.0
# If not cross compiling, check that we can run a simple program.
if test "$cross_compiling" != yes; then
  if { ac_try='./$ac_file'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
    cross_compiling=no
  else
    if test "$cross_compiling" = maybe; then
	cross_compiling=yes
    else
	{ { echo "$as_me:$LINENO: error: cannot run C compiled programs.
If you meant to cross compile, use \`--host'.
See \`config.log' for more details." >&5
echo "$as_me: error: cannot run C compiled programs.
If you meant to cross compile, use \`--host'.
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
    fi
  fi
fi
{ echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }

rm -f a.out a.exe conftest$ac_cv_exeext b.out
ac_clean_files=$ac_clean_files_save
# Check that the compiler produces executables we can run.  If not, either
# the compiler is broken, or we cross compile.
{ echo "$as_me:$LINENO: checking whether we are cross compiling" >&5
echo $ECHO_N "checking whether we are cross compiling... $ECHO_C" >&6; }
{ echo "$as_me:$LINENO: result: $cross_compiling" >&5
echo "${ECHO_T}$cross_compiling" >&6; }

{ echo "$as_me:$LINENO: checking for suffix of executables" >&5
echo $ECHO_N "checking for suffix of executables... $ECHO_C" >&6; }
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  # If both `conftest.exe' and `conftest' are `present' (well, observable)
# catch `conftest.exe'.  For instance with Cygwin, `ls conftest' will
# work properly (i.e., refer to `conftest.exe'), while it won't with
# `rm'.
for ac_file in conftest.exe conftest conftest.*; do
  test -f "$ac_file" || continue
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.o | *.obj ) ;;
    *.* ) ac_cv_exeext=`expr "$ac_file" : '[^.]*\(\..*\)'`
	  break;;
    * ) break;;
  esac
done
else
  { { echo "$as_me:$LINENO: error: cannot compute suffix of executables: cannot compile and link
See \`config.log' for more details." >&5
echo "$as_me: error: cannot compute suffix of executables: cannot compile and link
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

rm -f conftest$ac_cv_exeext
{ echo "$as_me:$LINENO: result: $ac_cv_exeext" >&5
echo "${ECHO_T}$ac_cv_exeext" >&6; }

rm -f conftest.$ac_ext
EXEEXT=$ac_cv_exeext
ac_exeext=$EXEEXT
{ echo "$as_me:$LINENO: checking for suffix of object files" >&5
echo $ECHO_N "checking for suffix of object files... $ECHO_C" >&6; }
if test "${ac_cv_objext+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.o conftest.obj
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; then
  for ac_file in conftest.o conftest.obj conftest.*; do
  test -f "$ac_file" || continue;
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf ) ;;
    *) ac_cv_objext=`expr "$ac_file" : '.*\.\(.*\)'`
       break;;
  esac
done
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

{ { echo "$as_me:$LINENO: error: cannot compute suffix of object files: cannot compile
See \`config.log' for more details." >&5
echo "$as_me: error: cannot compute suffix of object files: cannot compile
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

rm -f conftest.$ac_cv_objext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_objext" >&5
echo "${ECHO_T}$ac_cv_objext" >&6; }
OBJEXT=$ac_cv_objext
ac_objext=$OBJEXT
{ echo "$as_me:$LINENO: checking whether we are using the GNU C compiler" >&5
echo $ECHO_N "checking whether we are using the GNU C compiler... $ECHO_C" >&6; }
if test "${ac_cv_c_compiler_gnu+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{
#ifndef __GNUC__
       choke me
#endif

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_compiler_gnu=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_compiler_gnu=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
ac_cv_c_compiler_gnu=$ac_compiler_gnu

fi
{ echo "$as_me:$LINENO: result: $ac_cv_c_compiler_gnu" >&5
echo "${ECHO_T}$ac_cv_c_compiler_gnu" >&6; }
GCC=`test $ac_compiler_gnu = yes && echo yes`
ac_test_CFLAGS=${CFLAGS+set}
ac_save_CFLAGS=$CFLAGS
{ echo "$as_me:$LINENO: checking whether $CC accepts -g" >&5
echo $ECHO_N "checking whether $CC accepts -g... $ECHO_C" >&6; }
if test "${ac_cv_prog_cc_g+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_save_c_werror_flag=$ac_c_werror_flag
   ac_c_werror_flag=yes
   ac_cv_prog_cc_g=no
   CFLAGS="-g"
   cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_prog_cc_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	CFLAGS=""
      cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_c_werror_flag=$ac_save_c_werror_flag
	 CFLAGS="-g"
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_prog_cc_g=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
   ac_c_werror_flag=$ac_save_c_werror_flag
fi
{ echo "$as_me:$LINENO: result: $ac_cv_prog_cc_g" >&5
echo "${ECHO_T}$ac_cv_prog_cc_g" >&6; }
if test "$ac_test_CFLAGS" = set; then
  CFLAGS=$ac_save_CFLAGS
elif test $ac_cv_prog_cc_g = yes; then
  if test "$GCC" = yes; then
    CFLAGS="-g -O2"
  else
    CFLAGS="-g"
  fi
else
  if test "$GCC" = yes; then
    CFLAGS="-O2"
  else
    CFLAGS=
  fi
fi
{ echo "$as_me:$LINENO: checking for $CC option to accept ISO C89" >&5
echo $ECHO_N "checking for $CC option to accept ISO C89... $ECHO_C" >&6; }
if test "${ac_cv_prog_cc_c89+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_cv_prog_cc_c89=no
ac_save_CC=$CC
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdarg.h>
#include <stdio.h>
#include <sys/types.h>
#include <sys/stat.h>
/* Most of the following tests are stolen from RCS 5.7's src/conf.sh.  */
struct buf { int x; };
FILE * (*rcsopen) (struct buf *, struct stat *, int);
static char *e (p, i)
     char **p;
     int i;
{
  return p[i];
}
static char *f (char * (*g) (char **, int), char **p, ...)
{
  char *s;
  va_list v;
  va_start (v,p);
  s = g (p, va_arg (v,int));
  va_end (v);
  return s;
}

/* OSF 4.0 Compaq cc is some sort of almost-ANSI by default.  It has
   function prototypes and stuff, but not '\xHH' hex character constants.
   These don't provoke an error unfortunately, instead are silently treated
   as 'x'.  The following induces an error, until -std is added to get
   proper ANSI mode.  Curiously '\x00'!='x' always comes out true, for an
   array size at least.  It's necessary to write '\x00'==0 to get something
   that's true only with -std.  */
int osf4_cc_array ['\x00' == 0 ? 1 : -1];

/* IBM C 6 for AIX is almost-ANSI by default, but it replaces macro parameters
   inside strings and character constants.  */
#define FOO(x) 'x'
int xlc6_cc_array[FOO(a) == 'x' ? 1 : -1];

int test (int i, double x);
struct s1 {int (*f) (int a);};
struct s2 {int (*f) (double a);};
int pairnames (int, char **, FILE *(*)(struct buf *, struct stat *, int), int, int);
int argc;
char **argv;
int
main ()
{
return f (e, argv, 0) != argv[0]  ||  f (e, argv, 1) != argv[1];
  ;
  return 0;
}
_ACEOF
for ac_arg in '' -qlanglvl=extc89 -qlanglvl=ansi -std \
	-Ae "-Aa -D_HPUX_SOURCE" "-Xc -D__EXTENSIONS__"
do
  CC="$ac_save_CC $ac_arg"
  rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_prog_cc_c89=$ac_arg
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


fi

rm -f core conftest.err conftest.$ac_objext
  test "x$ac_cv_prog_cc_c89" != "xno" && break
done
rm -f conftest.$ac_ext
CC=$ac_save_CC

fi
# AC_CACHE_VAL
case "x$ac_cv_prog_cc_c89" in
  x)
    { echo "$as_me:$LINENO: result: none needed" >&5
echo "${ECHO_T}none needed" >&6; } ;;
  xno)
    { echo "$as_me:$LINENO: result: unsupported" >&5
echo "${ECHO_T}unsupported" >&6; } ;;
  *)
    CC="$CC $ac_cv_prog_cc_c89"
    { echo "$as_me:$LINENO: result: $ac_cv_prog_cc_c89" >&5
echo "${ECHO_T}$ac_cv_prog_cc_c89" >&6; } ;;
esac


ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu

ac_aux_dir=
for ac_dir in "$srcdir" "$srcdir/.." "$srcdir/../.."; do
  if test -f "$ac_dir/install-sh"; then
    ac_aux_dir=$ac_dir
    ac_install_sh="$ac_aux_dir/install-sh -c"
    break
  elif test -f "$ac_dir/install.sh"; then
    ac_aux_dir=$ac_dir
    ac_install_sh="$ac_aux_dir/install.sh -c"
    break
  elif test -f "$ac_dir/shtool"; then
    ac_aux_dir=$ac_dir
    ac_install_sh="$ac_aux_dir/shtool install -c"
    break
  fi
done
if test -z "$ac_aux_dir"; then
  { { echo "$as_me:$LINENO: error: cannot find install-sh or install.sh in \"$srcdir\" \"$srcdir/..\" \"$srcdir/../..\"" >&5
echo "$as_me: error: cannot find install-sh or install.sh in \"$srcdir\" \"$srcdir/..\" \"$srcdir/../..\"" >&2;}
   { (exit 1); exit 1; }; }
fi

# These three variables are undocumented and unsupported,
# and are intended to be withdrawn in a future Autoconf release.
# They can cause serious problems if a builder's source tree is in a directory
# whose full name contains unusual characters.
ac_config_guess="$SHELL $ac_aux_dir/config.guess"  # Please don't use this var.
ac_config_sub="$SHELL $ac_aux_dir/config.sub"  # Please don't use this var.
ac_configure="$SHELL $ac_aux_dir/configure"  # Please don't use this var.


# Find a good install program.  We prefer a C program (faster),
# so one script is as good as another.  But avoid the broken or
# incompatible versions:
# SysV /etc/install, /usr/sbin/install
# SunOS /usr/etc/install
# IRIX /sbin/install
# AIX /bin/install
# AmigaOS /C/install, which installs bootblocks on floppy discs
# AIX 4 /usr/bin/installbsd, which doesn't work without a -g flag
# AFS /usr/afsws/bin/install, which mishandles nonexistent args
# SVR4 /usr/ucb/install, which tries to use the nonexistent group "staff"
# OS/2's system install, which has a completely different semantic
# ./install, which can be erroneously created by make from ./install.sh.
{ echo "$as_me:$LINENO: checking for a BSD-compatible install" >&5
echo $ECHO_N "checking for a BSD-compatible install... $ECHO_C" >&6; }
if test -z "$INSTALL"; then
if test "${ac_cv_path_install+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  # Account for people who put trailing slashes in PATH elements.
case $as_dir/ in
  ./ | .// | /cC/* | \
  /etc/* | /usr/sbin/* | /usr/etc/* | /sbin/* | /usr/afsws/bin/* | \
  ?:\\/os2\\/install\\/* | ?:\\/OS2\\/INSTALL\\/* | \
  /usr/ucb/* ) ;;
  *)
    # OSF1 and SCO ODT 3.0 have their own names for install.
    # Don't use installbsd from OSF since it installs stuff as root
    # by default.
    for ac_prog in ginstall scoinst install; do
      for ac_exec_ext in '' $ac_executable_extensions; do
	if { test -f "$as_dir/$ac_prog$ac_exec_ext" && $as_executable_p "$as_dir/$ac_prog$ac_exec_ext"; }; then
	  if test $ac_prog = install &&
	    grep dspmsg "$as_dir/$ac_prog$ac_exec_ext" >/dev/null 2>&1; then
	    # AIX install.  It has an incompatible calling convention.
	    :
	  elif test $ac_prog = install &&
	    grep pwplus "$as_dir/$ac_prog$ac_exec_ext" >/dev/null 2>&1; then
	    # program-specific install script used by HP pwplus--don't use.
	    :
	  else
	    ac_cv_path_install="$as_dir/$ac_prog$ac_exec_ext -c"
	    break 3
	  fi
	fi
      done
    done
    ;;
esac
done
IFS=$as_save_IFS


fi
  if test "${ac_cv_path_install+set}" = set; then
    INSTALL=$ac_cv_path_install
  else
    # As a last resort, use the slow shell script.  Don't cache a
    # value for INSTALL within a source directory, because that will
    # break other packages using the cache if that directory is
    # removed, or if the value is a relative name.
    INSTALL=$ac_install_sh
  fi
fi
{ echo "$as_me:$LINENO: result: $INSTALL" >&5
echo "${ECHO_T}$INSTALL" >&6; }

# Use test -z because SunOS4 sh mishandles braces in ${var-val}.
# It thinks the first close brace ends the variable substitution.
test -z "$INSTALL_PROGRAM" && INSTALL_PROGRAM='${INSTALL}'

test -z "$INSTALL_SCRIPT" && INSTALL_SCRIPT='${INSTALL}'

test -z "$INSTALL_DATA" && INSTALL_DATA='${INSTALL} -m 644'

{ echo "$as_me:$LINENO: checking whether ln -s works" >&5
echo $ECHO_N "checking whether ln -s works... $ECHO_C" >&6; }
LN_S=$as_ln_s
if test "$LN_S" = "ln -s"; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
else
  { echo "$as_me:$LINENO: result: no, using $LN_S" >&5
echo "${ECHO_T}no, using $LN_S" >&6; }
fi

{ echo "$as_me:$LINENO: checking whether ${MAKE-make} sets \$(MAKE)" >&5
echo $ECHO_N "checking whether ${MAKE-make} sets \$(MAKE)... $ECHO_C" >&6; }
set x ${MAKE-make}; ac_make=`echo "$2" | sed 's/+/p/g; s/[^a-zA-Z0-9_]/_/g'`
if { as_var=ac_cv_prog_make_${ac_make}_set; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.make <<\_ACEOF
SHELL = /bin/sh
all:
	@echo '@@@%%%=$(MAKE)=@@@%%%'
_ACEOF
# GNU make sometimes prints "make[1]: Entering...", which would confuse us.
case `${MAKE-make} -f conftest.make 2>/dev/null` in
  *@@@%%%=?*=@@@%%%*)
    eval ac_cv_prog_make_${ac_make}_set=yes;;
  *)
    eval ac_cv_prog_make_${ac_make}_set=no;;
esac
rm -f conftest.make
fi
if eval test \$ac_cv_prog_make_${ac_make}_set = yes; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
  SET_MAKE=
else
  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
  SET_MAKE="MAKE=${MAKE-make}"
fi



# Check whether --with-kpathsea was given.
if test "${with_kpathsea+set}" = set; then
  withval=$with_kpathsea;
  if test -d "$withval"; then
    CPPFLAGS="$CPPFLAGS -I$withval/include"
    LDFLAGS="$LDFLAGS -L$withval/lib"
 fi

fi



{ echo "$as_me:$LINENO: checking whether you have kpathsea headers and they whether they know about the required file formats" >&5
echo $ECHO_N "checking whether you have kpathsea headers and they whether they know about the required file formats... $ECHO_C" >&6; }
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdio.h>
#include <kpathsea/kpathsea.h>
int
main ()
{
kpse_tex_ps_header_format;
			 kpse_type1_format;kpse_vf_format
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }; cat >>confdefs.h <<\_ACEOF
#define HAVE_KPSE_FORMATS 1
_ACEOF

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	{ echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; };
{ { echo "$as_me:$LINENO: error: PS_HEADER and/or VF formats not found in Kpathsea header files.

This version of dvipdfm requires that kpathsea and its headers be installed.
If you are sure they are installed and in a standard place, maybe you need a
newer version of kpathsea?  You also might try setting the environment
variable CPPFLAGS (or CFLAGS) with -I pointing to the directory containing
the file \"kpathsea.h\"

" >&5
echo "$as_me: error: PS_HEADER and/or VF formats not found in Kpathsea header files.

This version of dvipdfm requires that kpathsea and its headers be installed.
If you are sure they are installed and in a standard place, maybe you need a
newer version of kpathsea?  You also might try setting the environment
variable CPPFLAGS (or CFLAGS) with -I pointing to the directory containing
the file \"kpathsea.h\"

" >&2;}
   { (exit 1); exit 1; }; }
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
{ echo "$as_me:$LINENO: checking whether your kpathsea supports Omega OFM file formats" >&5
echo $ECHO_N "checking whether your kpathsea supports Omega OFM file formats... $ECHO_C" >&6; }
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdio.h>
#include <kpathsea/kpathsea.h>
int
main ()
{
kpse_ofm_format
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }; cat >>confdefs.h <<\_ACEOF
#define HAVE_OMEGA_FORMATS 1
_ACEOF

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	{ echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
TTF_OPT='#'
{ echo "$as_me:$LINENO: checking whether your kpathsea supports Truetype (TTF) file formats" >&5
echo $ECHO_N "checking whether your kpathsea supports Truetype (TTF) file formats... $ECHO_C" >&6; }
	 cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdio.h>
#include <kpathsea/kpathsea.h>
int
main ()
{
kpse_truetype_format
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
			 cat >>confdefs.h <<\_ACEOF
#define HAVE_TTF_FORMATS 1
_ACEOF

			 TTF_OPT=''
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	{ echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext


{ echo "$as_me:$LINENO: checking for kpse_find_file in -lkpathsea" >&5
echo $ECHO_N "checking for kpse_find_file in -lkpathsea... $ECHO_C" >&6; }
if test "${ac_cv_lib_kpathsea_kpse_find_file+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lkpathsea  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char kpse_find_file ();
int
main ()
{
return kpse_find_file ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_lib_kpathsea_kpse_find_file=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_kpathsea_kpse_find_file=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_kpathsea_kpse_find_file" >&5
echo "${ECHO_T}$ac_cv_lib_kpathsea_kpse_find_file" >&6; }
if test $ac_cv_lib_kpathsea_kpse_find_file = yes; then
  cat >>confdefs.h <<\_ACEOF
#define HAVE_KPATHSEA 1
_ACEOF
 LIBS="-lkpathsea $LIBS"
else
  { { echo "$as_me:$LINENO: error: kpathsea library not found
This version of dvipdfm requires the kpathsea library and its headers.  If
you know where it is you might try setting the LDFLAGS environment variable
with -L pointing to the directory containing libkpathsea.a
" >&5
echo "$as_me: error: kpathsea library not found
This version of dvipdfm requires the kpathsea library and its headers.  If
you know where it is you might try setting the LDFLAGS environment variable
with -L pointing to the directory containing libkpathsea.a
" >&2;}
   { (exit 1); exit 1; }; }
fi



{ echo "$as_me:$LINENO: checking for xbasename in -lkpathsea" >&5
echo $ECHO_N "checking for xbasename in -lkpathsea... $ECHO_C" >&6; }
if test "${ac_cv_lib_kpathsea_xbasename+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lkpathsea  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char xbasename ();
int
main ()
{
return xbasename ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_lib_kpathsea_xbasename=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_kpathsea_xbasename=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_kpathsea_xbasename" >&5
echo "${ECHO_T}$ac_cv_lib_kpathsea_xbasename" >&6; }
if test $ac_cv_lib_kpathsea_xbasename = yes; then
  cat >>confdefs.h <<\_ACEOF
#define HAVE_XBASENAME 1
_ACEOF

fi


TEXMF='${datadir}/texmf'


_cppflags=$CPPFLAGS
_ldflags=$LDFLAGS

# Check whether --with-png was given.
if test "${with_png+set}" = set; then
  withval=$with_png;
  if test -d "$withval"; then
    CPPFLAGS="$CPPFLAGS -I$withval/include"
    LDFLAGS="$LDFLAGS -L$withval/lib"
  fi

fi

{ echo "$as_me:$LINENO: checking for pow" >&5
echo $ECHO_N "checking for pow... $ECHO_C" >&6; }
if test "${ac_cv_func_pow+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
/* Define pow to an innocuous variant, in case <limits.h> declares pow.
   For example, HP-UX 11i <limits.h> declares gettimeofday.  */
#define pow innocuous_pow

/* System header to define __stub macros and hopefully few prototypes,
    which can conflict with char pow (); below.
    Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
    <limits.h> exists even on freestanding compilers.  */

#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif

#undef pow

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char pow ();
/* The GNU C library defines this for functions which it implements
    to always fail with ENOSYS.  Some functions are actually named
    something starting with __ and the normal name is an alias.  */
#if defined __stub_pow || defined __stub___pow
choke me
#endif

int
main ()
{
return pow ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_func_pow=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_func_pow=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_func_pow" >&5
echo "${ECHO_T}$ac_cv_func_pow" >&6; }
if test $ac_cv_func_pow = yes; then
  :
else
  { echo "$as_me:$LINENO: checking for pow in -lm" >&5
echo $ECHO_N "checking for pow in -lm... $ECHO_C" >&6; }
if test "${ac_cv_lib_m_pow+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lm  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char pow ();
int
main ()
{
return pow ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_lib_m_pow=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_m_pow=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_m_pow" >&5
echo "${ECHO_T}$ac_cv_lib_m_pow" >&6; }
if test $ac_cv_lib_m_pow = yes; then
  LIBS="$LIBS -lm"
fi

fi

{ echo "$as_me:$LINENO: checking for png header files" >&5
echo $ECHO_N "checking for png header files... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <png.h>
int
main ()
{
png_infop p;
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then

  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
  { echo "$as_me:$LINENO: checking for png_get_image_width in -lpng" >&5
echo $ECHO_N "checking for png_get_image_width in -lpng... $ECHO_C" >&6; }
if test "${ac_cv_lib_png_png_get_image_width+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lpng -lz $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char png_get_image_width ();
int
main ()
{
return png_get_image_width ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_lib_png_png_get_image_width=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_png_png_get_image_width=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_png_png_get_image_width" >&5
echo "${ECHO_T}$ac_cv_lib_png_png_get_image_width" >&6; }
if test $ac_cv_lib_png_png_get_image_width = yes; then

    cat >>confdefs.h <<\_ACEOF
#define HAVE_LIBPNG 1
_ACEOF

    LIBS="$LIBS -lpng"
fi

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5


  { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
_cppflags=$CPPFLAGS
 _ldflags=$LDFLAGS

# Check whether --with-zlib was given.
if test "${with_zlib+set}" = set; then
  withval=$with_zlib;
  if test -d "$withval"; then
    CPPFLAGS="$CPPFLAGS -I$withval/include"
    LDFLAGS="$LDFLAGS -L$withval/lib"
  fi

fi

{ echo "$as_me:$LINENO: checking for zlib header files" >&5
echo $ECHO_N "checking for zlib header files... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <zlib.h>
int
main ()
{
z_stream p;
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }
 { echo "$as_me:$LINENO: checking for compress in -lz" >&5
echo $ECHO_N "checking for compress in -lz... $ECHO_C" >&6; }
if test "${ac_cv_lib_z_compress+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lz  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char compress ();
int
main ()
{
return compress ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_lib_z_compress=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_z_compress=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_z_compress" >&5
echo "${ECHO_T}$ac_cv_lib_z_compress" >&6; }
if test $ac_cv_lib_z_compress = yes; then
  cat >>confdefs.h <<\_ACEOF
#define HAVE_ZLIB 1
_ACEOF

 LIBS="$LIBS -lz"
 { echo "$as_me:$LINENO: checking for compress2 in -lz" >&5
echo $ECHO_N "checking for compress2 in -lz... $ECHO_C" >&6; }
if test "${ac_cv_lib_z_compress2+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lz  $LIBS"
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char compress2 ();
int
main ()
{
return compress2 ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_lib_z_compress2=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_lib_z_compress2=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ echo "$as_me:$LINENO: result: $ac_cv_lib_z_compress2" >&5
echo "${ECHO_T}$ac_cv_lib_z_compress2" >&6; }
if test $ac_cv_lib_z_compress2 = yes; then
  cat >>confdefs.h <<\_ACEOF
#define HAVE_ZLIB_COMPRESS2 1
_ACEOF

fi

fi

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	CPPFLAGS=$_cppflags
 LDDFLAGS=$_ldflags
 { echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext

{ echo "$as_me:$LINENO: checking for system" >&5
echo $ECHO_N "checking for system... $ECHO_C" >&6; }
if test "${ac_cv_func_system+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
/* Define system to an innocuous variant, in case <limits.h> declares system.
   For example, HP-UX 11i <limits.h> declares gettimeofday.  */
#define system innocuous_system

/* System header to define __stub macros and hopefully few prototypes,
    which can conflict with char system (); below.
    Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
    <limits.h> exists even on freestanding compilers.  */

#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif

#undef system

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char system ();
/* The GNU C library defines this for functions which it implements
    to always fail with ENOSYS.  Some functions are actually named
    something starting with __ and the normal name is an alias.  */
#if defined __stub_system || defined __stub___system
choke me
#endif

int
main ()
{
return system ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_func_system=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_func_system=no
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_func_system" >&5
echo "${ECHO_T}$ac_cv_func_system" >&6; }
if test $ac_cv_func_system = yes; then
  cat >>confdefs.h <<\_ACEOF
#define HAVE_SYSTEM 1
_ACEOF

fi



ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu
{ echo "$as_me:$LINENO: checking how to run the C preprocessor" >&5
echo $ECHO_N "checking how to run the C preprocessor... $ECHO_C" >&6; }
# On Suns, sometimes $CPP names a directory.
if test -n "$CPP" && test -d "$CPP"; then
  CPP=
fi
if test -z "$CPP"; then
  if test "${ac_cv_prog_CPP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
      # Double quotes because CPP needs to be expanded
    for CPP in "$CC -E" "$CC -E -traditional-cpp" "/lib/cpp"
    do
      ac_preproc_ok=false
for ac_c_preproc_warn_flag in '' yes
do
  # Use a header file that comes with gcc, so configuring glibc
  # with a fresh cross-compiler works.
  # Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
  # <limits.h> exists even on freestanding compilers.
  # On the NeXT, cc -E runs the code through the compiler's parser,
  # not just through cpp. "Syntax error" is here to catch this case.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif
		     Syntax error
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null; then
  if test -s conftest.err; then
    ac_cpp_err=$ac_c_preproc_warn_flag
    ac_cpp_err=$ac_cpp_err$ac_c_werror_flag
  else
    ac_cpp_err=
  fi
else
  ac_cpp_err=yes
fi
if test -z "$ac_cpp_err"; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Broken: fails on valid input.
continue
fi

rm -f conftest.err conftest.$ac_ext

  # OK, works on sane cases.  Now check whether nonexistent headers
  # can be detected and how.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ac_nonexistent.h>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null; then
  if test -s conftest.err; then
    ac_cpp_err=$ac_c_preproc_warn_flag
    ac_cpp_err=$ac_cpp_err$ac_c_werror_flag
  else
    ac_cpp_err=
  fi
else
  ac_cpp_err=yes
fi
if test -z "$ac_cpp_err"; then
  # Broken: success on invalid input.
continue
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Passes both tests.
ac_preproc_ok=:
break
fi

rm -f conftest.err conftest.$ac_ext

done
# Because of `break', _AC_PREPROC_IFELSE's cleaning code was skipped.
rm -f conftest.err conftest.$ac_ext
if $ac_preproc_ok; then
  break
fi

    done
    ac_cv_prog_CPP=$CPP

fi
  CPP=$ac_cv_prog_CPP
else
  ac_cv_prog_CPP=$CPP
fi
{ echo "$as_me:$LINENO: result: $CPP" >&5
echo "${ECHO_T}$CPP" >&6; }
ac_preproc_ok=false
for ac_c_preproc_warn_flag in '' yes
do
  # Use a header file that comes with gcc, so configuring glibc
  # with a fresh cross-compiler works.
  # Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
  # <limits.h> exists even on freestanding compilers.
  # On the NeXT, cc -E runs the code through the compiler's parser,
  # not just through cpp. "Syntax error" is here to catch this case.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif
		     Syntax error
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null; then
  if test -s conftest.err; then
    ac_cpp_err=$ac_c_preproc_warn_flag
    ac_cpp_err=$ac_cpp_err$ac_c_werror_flag
  else
    ac_cpp_err=
  fi
else
  ac_cpp_err=yes
fi
if test -z "$ac_cpp_err"; then
  :
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Broken: fails on valid input.
continue
fi

rm -f conftest.err conftest.$ac_ext

  # OK, works on sane cases.  Now check whether nonexistent headers
  # can be detected and how.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ac_nonexistent.h>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null; then
  if test -s conftest.err; then
    ac_cpp_err=$ac_c_preproc_warn_flag
    ac_cpp_err=$ac_cpp_err$ac_c_werror_flag
  else
    ac_cpp_err=
  fi
else
  ac_cpp_err=yes
fi
if test -z "$ac_cpp_err"; then
  # Broken: success on invalid input.
continue
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  # Passes both tests.
ac_preproc_ok=:
break
fi

rm -f conftest.err conftest.$ac_ext

done
# Because of `break', _AC_PREPROC_IFELSE's cleaning code was skipped.
rm -f conftest.err conftest.$ac_ext
if $ac_preproc_ok; then
  :
else
  { { echo "$as_me:$LINENO: error: C preprocessor \"$CPP\" fails sanity check
See \`config.log' for more details." >&5
echo "$as_me: error: C preprocessor \"$CPP\" fails sanity check
See \`config.log' for more details." >&2;}
   { (exit 1); exit 1; }; }
fi

ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu


{ echo "$as_me:$LINENO: checking for grep that handles long lines and -e" >&5
echo $ECHO_N "checking for grep that handles long lines and -e... $ECHO_C" >&6; }
if test "${ac_cv_path_GREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  # Extract the first word of "grep ggrep" to use in msg output
if test -z "$GREP"; then
set dummy grep ggrep; ac_prog_name=$2
if test "${ac_cv_path_GREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_path_GREP_found=false
# Loop through the user's path and test for each of PROGNAME-LIST
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH$PATH_SEPARATOR/usr/xpg4/bin
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_prog in grep ggrep; do
  for ac_exec_ext in '' $ac_executable_extensions; do
    ac_path_GREP="$as_dir/$ac_prog$ac_exec_ext"
    { test -f "$ac_path_GREP" && $as_executable_p "$ac_path_GREP"; } || continue
    # Check for GNU ac_path_GREP and select it if it is found.
  # Check for GNU $ac_path_GREP
case `"$ac_path_GREP" --version 2>&1` in
*GNU*)
  ac_cv_path_GREP="$ac_path_GREP" ac_path_GREP_found=:;;
*)
  ac_count=0
  echo $ECHO_N "0123456789$ECHO_C" >"conftest.in"
  while :
  do
    cat "conftest.in" "conftest.in" >"conftest.tmp"
    mv "conftest.tmp" "conftest.in"
    cp "conftest.in" "conftest.nl"
    echo 'GREP' >> "conftest.nl"
    "$ac_path_GREP" -e 'GREP$' -e '-(cannot match)-' < "conftest.nl" >"conftest.out" 2>/dev/null || break
    diff "conftest.out" "conftest.nl" >/dev/null 2>&1 || break
    ac_count=`expr $ac_count + 1`
    if test $ac_count -gt ${ac_path_GREP_max-0}; then
      # Best one so far, save it but keep looking for a better one
      ac_cv_path_GREP="$ac_path_GREP"
      ac_path_GREP_max=$ac_count
    fi
    # 10*(2^10) chars as input seems more than enough
    test $ac_count -gt 10 && break
  done
  rm -f conftest.in conftest.tmp conftest.nl conftest.out;;
esac


    $ac_path_GREP_found && break 3
  done
done

done
IFS=$as_save_IFS


fi

GREP="$ac_cv_path_GREP"
if test -z "$GREP"; then
  { { echo "$as_me:$LINENO: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&5
echo "$as_me: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&2;}
   { (exit 1); exit 1; }; }
fi

else
  ac_cv_path_GREP=$GREP
fi


fi
{ echo "$as_me:$LINENO: result: $ac_cv_path_GREP" >&5
echo "${ECHO_T}$ac_cv_path_GREP" >&6; }
 GREP="$ac_cv_path_GREP"


{ echo "$as_me:$LINENO: checking for egrep" >&5
echo $ECHO_N "checking for egrep... $ECHO_C" >&6; }
if test "${ac_cv_path_EGREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if echo a | $GREP -E '(a|b)' >/dev/null 2>&1
   then ac_cv_path_EGREP="$GREP -E"
   else
     # Extract the first word of "egrep" to use in msg output
if test -z "$EGREP"; then
set dummy egrep; ac_prog_name=$2
if test "${ac_cv_path_EGREP+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  ac_path_EGREP_found=false
# Loop through the user's path and test for each of PROGNAME-LIST
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH$PATH_SEPARATOR/usr/xpg4/bin
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  for ac_prog in egrep; do
  for ac_exec_ext in '' $ac_executable_extensions; do
    ac_path_EGREP="$as_dir/$ac_prog$ac_exec_ext"
    { test -f "$ac_path_EGREP" && $as_executable_p "$ac_path_EGREP"; } || continue
    # Check for GNU ac_path_EGREP and select it if it is found.
  # Check for GNU $ac_path_EGREP
case `"$ac_path_EGREP" --version 2>&1` in
*GNU*)
  ac_cv_path_EGREP="$ac_path_EGREP" ac_path_EGREP_found=:;;
*)
  ac_count=0
  echo $ECHO_N "0123456789$ECHO_C" >"conftest.in"
  while :
  do
    cat "conftest.in" "conftest.in" >"conftest.tmp"
    mv "conftest.tmp" "conftest.in"
    cp "conftest.in" "conftest.nl"
    echo 'EGREP' >> "conftest.nl"
    "$ac_path_EGREP" 'EGREP$' < "conftest.nl" >"conftest.out" 2>/dev/null || break
    diff "conftest.out" "conftest.nl" >/dev/null 2>&1 || break
    ac_count=`expr $ac_count + 1`
    if test $ac_count -gt ${ac_path_EGREP_max-0}; then
      # Best one so far, save it but keep looking for a better one
      ac_cv_path_EGREP="$ac_path_EGREP"
      ac_path_EGREP_max=$ac_count
    fi
    # 10*(2^10) chars as input seems more than enough
    test $ac_count -gt 10 && break
  done
  rm -f conftest.in conftest.tmp conftest.nl conftest.out;;
esac


    $ac_path_EGREP_found && break 3
  done
done

done
IFS=$as_save_IFS


fi

EGREP="$ac_cv_path_EGREP"
if test -z "$EGREP"; then
  { { echo "$as_me:$LINENO: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&5
echo "$as_me: error: no acceptable $ac_prog_name could be found in $PATH$PATH_SEPARATOR/usr/xpg4/bin" >&2;}
   { (exit 1); exit 1; }; }
fi

else
  ac_cv_path_EGREP=$EGREP
fi


   fi
fi
{ echo "$as_me:$LINENO: result: $ac_cv_path_EGREP" >&5
echo "${ECHO_T}$ac_cv_path_EGREP" >&6; }
 EGREP="$ac_cv_path_EGREP"


{ echo "$as_me:$LINENO: checking for ANSI C header files" >&5
echo $ECHO_N "checking for ANSI C header files... $ECHO_C" >&6; }
if test "${ac_cv_header_stdc+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdlib.h>
#include <stdarg.h>
#include <string.h>
#include <float.h>

int
main ()
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_header_stdc=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_header_stdc=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext

if test $ac_cv_header_stdc = yes; then
  # SunOS 4.x string.h does not declare mem*, contrary to ANSI.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <string.h>

_ACEOF
if (eval "$ac_cpp conftest.$ac_ext") 2>&5 |
  $EGREP "memchr" >/dev/null 2>&1; then
  :
else
  ac_cv_header_stdc=no
fi
rm -f conftest*

fi

if test $ac_cv_header_stdc = yes; then
  # ISC 2.0.2 stdlib.h does not declare free, contrary to ANSI.
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <stdlib.h>

_ACEOF
if (eval "$ac_cpp conftest.$ac_ext") 2>&5 |
  $EGREP "free" >/dev/null 2>&1; then
  :
else
  ac_cv_header_stdc=no
fi
rm -f conftest*

fi

if test $ac_cv_header_stdc = yes; then
  # /bin/cc in Irix-4.0.5 gets non-ANSI ctype macros unless using -ansi.
  if test "$cross_compiling" = yes; then
  :
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <ctype.h>
#include <stdlib.h>
#if ((' ' & 0x0FF) == 0x020)
# define ISLOWER(c) ('a' <= (c) && (c) <= 'z')
# define TOUPPER(c) (ISLOWER(c) ? 'A' + ((c) - 'a') : (c))
#else
# define ISLOWER(c) \
		   (('a' <= (c) && (c) <= 'i') \
		     || ('j' <= (c) && (c) <= 'r') \
		     || ('s' <= (c) && (c) <= 'z'))
# define TOUPPER(c) (ISLOWER(c) ? ((c) | 0x40) : (c))
#endif

#define XOR(e, f) (((e) && !(f)) || (!(e) && (f)))
int
main ()
{
  int i;
  for (i = 0; i < 256; i++)
    if (XOR (islower (i), ISLOWER (i))
	|| toupper (i) != TOUPPER (i))
      return 2;
  return 0;
}
_ACEOF
rm -f conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && { ac_try='./conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  :
else
  echo "$as_me: program exited with status $ac_status" >&5
echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

( exit $ac_status )
ac_cv_header_stdc=no
fi
rm -f core *.core core.conftest.* gmon.out bb.out conftest$ac_exeext conftest.$ac_objext conftest.$ac_ext
fi


fi
fi
{ echo "$as_me:$LINENO: result: $ac_cv_header_stdc" >&5
echo "${ECHO_T}$ac_cv_header_stdc" >&6; }
if test $ac_cv_header_stdc = yes; then

cat >>confdefs.h <<\_ACEOF
#define STDC_HEADERS 1
_ACEOF

fi

# On IRIX 5.3, sys/types and inttypes.h are conflicting.









for ac_header in sys/types.h sys/stat.h stdlib.h string.h memory.h strings.h \
		  inttypes.h stdint.h unistd.h
do
as_ac_Header=`echo "ac_cv_header_$ac_header" | $as_tr_sh`
{ echo "$as_me:$LINENO: checking for $ac_header" >&5
echo $ECHO_N "checking for $ac_header... $ECHO_C" >&6; }
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
$ac_includes_default

#include <$ac_header>
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  eval "$as_ac_Header=yes"
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	eval "$as_ac_Header=no"
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi
ac_res=`eval echo '${'$as_ac_Header'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }
if test `eval echo '${'$as_ac_Header'}'` = yes; then
  cat >>confdefs.h <<_ACEOF
#define `echo "HAVE_$ac_header" | $as_tr_cpp` 1
_ACEOF

fi

done



for ac_header in unistd.h
do
as_ac_Header=`echo "ac_cv_header_$ac_header" | $as_tr_sh`
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  { echo "$as_me:$LINENO: checking for $ac_header" >&5
echo $ECHO_N "checking for $ac_header... $ECHO_C" >&6; }
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
fi
ac_res=`eval echo '${'$as_ac_Header'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }
else
  # Is the header compilable?
{ echo "$as_me:$LINENO: checking $ac_header usability" >&5
echo $ECHO_N "checking $ac_header usability... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
$ac_includes_default
#include <$ac_header>
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_header_compiler=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_header_compiler=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
{ echo "$as_me:$LINENO: result: $ac_header_compiler" >&5
echo "${ECHO_T}$ac_header_compiler" >&6; }

# Is the header present?
{ echo "$as_me:$LINENO: checking $ac_header presence" >&5
echo $ECHO_N "checking $ac_header presence... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <$ac_header>
_ACEOF
if { (ac_try="$ac_cpp conftest.$ac_ext"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_cpp conftest.$ac_ext") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } >/dev/null; then
  if test -s conftest.err; then
    ac_cpp_err=$ac_c_preproc_warn_flag
    ac_cpp_err=$ac_cpp_err$ac_c_werror_flag
  else
    ac_cpp_err=
  fi
else
  ac_cpp_err=yes
fi
if test -z "$ac_cpp_err"; then
  ac_header_preproc=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

  ac_header_preproc=no
fi

rm -f conftest.err conftest.$ac_ext
{ echo "$as_me:$LINENO: result: $ac_header_preproc" >&5
echo "${ECHO_T}$ac_header_preproc" >&6; }

# So?  What about this header?
case $ac_header_compiler:$ac_header_preproc:$ac_c_preproc_warn_flag in
  yes:no: )
    { echo "$as_me:$LINENO: WARNING: $ac_header: accepted by the compiler, rejected by the preprocessor!" >&5
echo "$as_me: WARNING: $ac_header: accepted by the compiler, rejected by the preprocessor!" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: proceeding with the compiler's result" >&5
echo "$as_me: WARNING: $ac_header: proceeding with the compiler's result" >&2;}
    ac_header_preproc=yes
    ;;
  no:yes:* )
    { echo "$as_me:$LINENO: WARNING: $ac_header: present but cannot be compiled" >&5
echo "$as_me: WARNING: $ac_header: present but cannot be compiled" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header:     check for missing prerequisite headers?" >&5
echo "$as_me: WARNING: $ac_header:     check for missing prerequisite headers?" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: see the Autoconf documentation" >&5
echo "$as_me: WARNING: $ac_header: see the Autoconf documentation" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header:     section \"Present But Cannot Be Compiled\"" >&5
echo "$as_me: WARNING: $ac_header:     section \"Present But Cannot Be Compiled\"" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: proceeding with the preprocessor's result" >&5
echo "$as_me: WARNING: $ac_header: proceeding with the preprocessor's result" >&2;}
    { echo "$as_me:$LINENO: WARNING: $ac_header: in the future, the compiler will take precedence" >&5
echo "$as_me: WARNING: $ac_header: in the future, the compiler will take precedence" >&2;}

    ;;
esac
{ echo "$as_me:$LINENO: checking for $ac_header" >&5
echo $ECHO_N "checking for $ac_header... $ECHO_C" >&6; }
if { as_var=$as_ac_Header; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  eval "$as_ac_Header=\$ac_header_preproc"
fi
ac_res=`eval echo '${'$as_ac_Header'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }

fi
if test `eval echo '${'$as_ac_Header'}'` = yes; then
  cat >>confdefs.h <<_ACEOF
#define `echo "HAVE_$ac_header" | $as_tr_cpp` 1
_ACEOF

fi

done


{ echo "$as_me:$LINENO: checking whether time.h defines timezone as an external variable" >&5
echo $ECHO_N "checking whether time.h defines timezone as an external variable... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <time.h>
int
main ()
{
 -timezone;
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }; cat >>confdefs.h <<\_ACEOF
#define HAVE_TIMEZONE 1
_ACEOF

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	{ echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
{ echo "$as_me:$LINENO: checking whether struct tz has tm_gmtoff as a member" >&5
echo $ECHO_N "checking whether struct tz has tm_gmtoff as a member... $ECHO_C" >&6; }
cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <time.h>
int
main ()
{
struct tm *tp; tp->tm_gmtoff
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  { echo "$as_me:$LINENO: result: yes" >&5
echo "${ECHO_T}yes" >&6; }; cat >>confdefs.h <<\_ACEOF
#define HAVE_TM_GMTOFF 1
_ACEOF

else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	{ echo "$as_me:$LINENO: result: no" >&5
echo "${ECHO_T}no" >&6; }
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext

{ echo "$as_me:$LINENO: checking for an ANSI C-conforming const" >&5
echo $ECHO_N "checking for an ANSI C-conforming const... $ECHO_C" >&6; }
if test "${ac_cv_c_const+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */

int
main ()
{
/* FIXME: Include the comments suggested by Paul. */
#ifndef __cplusplus
  /* Ultrix mips cc rejects this.  */
  typedef int charset[2];
  const charset x;
  /* SunOS 4.1.1 cc rejects this.  */
  char const *const *ccp;
  char **p;
  /* NEC SVR4.0.2 mips cc rejects this.  */
  struct point {int x, y;};
  static struct point const zero = {0,0};
  /* AIX XL C 1.02.0.0 rejects this.
     It does not let you subtract one const X* pointer from another in
     an arm of an if-expression whose if-part is not a constant
     expression */
  const char *g = "string";
  ccp = &g + (g ? g-g : 0);
  /* HPUX 7.0 cc rejects these. */
  ++ccp;
  p = (char**) ccp;
  ccp = (char const *const *) p;
  { /* SCO 3.2v4 cc rejects this.  */
    char *t;
    char const *s = 0 ? (char *) 0 : (char const *) 0;

    *t++ = 0;
    if (s) return 0;
  }
  { /* Someone thinks the Sun supposedly-ANSI compiler will reject this.  */
    int x[] = {25, 17};
    const int *foo = &x[0];
    ++foo;
  }
  { /* Sun SC1.0 ANSI compiler rejects this -- but not the above. */
    typedef const int *iptr;
    iptr p = 0;
    ++p;
  }
  { /* AIX XL C 1.02.0.0 rejects this saying
       "k.c", line 2.27: 1506-025 (S) Operand must be a modifiable lvalue. */
    struct s { int j; const int *ap[3]; };
    struct s *b; b->j = 5;
  }
  { /* ULTRIX-32 V3.1 (Rev 9) vcc rejects this */
    const int foo = 10;
    if (!foo) return 0;
  }
  return !x[0] && !zero.x;
#endif

  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_c_const=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_c_const=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_c_const" >&5
echo "${ECHO_T}$ac_cv_c_const" >&6; }
if test $ac_cv_c_const = no; then

cat >>confdefs.h <<\_ACEOF
#define const
_ACEOF

fi

{ echo "$as_me:$LINENO: checking for size_t" >&5
echo $ECHO_N "checking for size_t... $ECHO_C" >&6; }
if test "${ac_cv_type_size_t+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
$ac_includes_default
typedef size_t ac__type_new_;
int
main ()
{
if ((ac__type_new_ *) 0)
  return 0;
if (sizeof (ac__type_new_))
  return 0;
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_type_size_t=yes
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_type_size_t=no
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_type_size_t" >&5
echo "${ECHO_T}$ac_cv_type_size_t" >&6; }
if test $ac_cv_type_size_t = yes; then
  :
else

cat >>confdefs.h <<_ACEOF
#define size_t unsigned int
_ACEOF

fi

{ echo "$as_me:$LINENO: checking whether struct tm is in sys/time.h or time.h" >&5
echo $ECHO_N "checking whether struct tm is in sys/time.h or time.h... $ECHO_C" >&6; }
if test "${ac_cv_struct_tm+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
#include <sys/types.h>
#include <time.h>

int
main ()
{
struct tm *tp; tp->tm_sec;
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext
if { (ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_compile") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest.$ac_objext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_struct_tm=time.h
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_cv_struct_tm=sys/time.h
fi

rm -f core conftest.err conftest.$ac_objext conftest.$ac_ext
fi
{ echo "$as_me:$LINENO: result: $ac_cv_struct_tm" >&5
echo "${ECHO_T}$ac_cv_struct_tm" >&6; }
if test $ac_cv_struct_tm = sys/time.h; then

cat >>confdefs.h <<\_ACEOF
#define TM_IN_SYS_TIME 1
_ACEOF

fi


{ echo "$as_me:$LINENO: checking for working memcmp" >&5
echo $ECHO_N "checking for working memcmp... $ECHO_C" >&6; }
if test "${ac_cv_func_memcmp_working+set}" = set; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  if test "$cross_compiling" = yes; then
  ac_cv_func_memcmp_working=no
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
$ac_includes_default
int
main ()
{

  /* Some versions of memcmp are not 8-bit clean.  */
  char c0 = '\100', c1 = '\200', c2 = '\201';
  if (memcmp(&c0, &c2, 1) >= 0 || memcmp(&c1, &c2, 1) >= 0)
    return 1;

  /* The Next x86 OpenStep bug shows up only when comparing 16 bytes
     or more and with at least one buffer not starting on a 4-byte boundary.
     William Lewis provided this test program.   */
  {
    char foo[21];
    char bar[21];
    int i;
    for (i = 0; i < 4; i++)
      {
	char *a = foo + i;
	char *b = bar + i;
	strcpy (a, "--------01111111");
	strcpy (b, "--------10000000");
	if (memcmp (a, b, 16) >= 0)
	  return 1;
      }
    return 0;
  }

  ;
  return 0;
}
_ACEOF
rm -f conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } && { ac_try='./conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  ac_cv_func_memcmp_working=yes
else
  echo "$as_me: program exited with status $ac_status" >&5
echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

( exit $ac_status )
ac_cv_func_memcmp_working=no
fi
rm -f core *.core core.conftest.* gmon.out bb.out conftest$ac_exeext conftest.$ac_objext conftest.$ac_ext
fi


fi
{ echo "$as_me:$LINENO: result: $ac_cv_func_memcmp_working" >&5
echo "${ECHO_T}$ac_cv_func_memcmp_working" >&6; }
test $ac_cv_func_memcmp_working = no && case " $LIBOBJS " in
  *" memcmp.$ac_objext "* ) ;;
  *) LIBOBJS="$LIBOBJS memcmp.$ac_objext"
 ;;
esac



for ac_func in strspn
do
as_ac_var=`echo "ac_cv_func_$ac_func" | $as_tr_sh`
{ echo "$as_me:$LINENO: checking for $ac_func" >&5
echo $ECHO_N "checking for $ac_func... $ECHO_C" >&6; }
if { as_var=$as_ac_var; eval "test \"\${$as_var+set}\" = set"; }; then
  echo $ECHO_N "(cached) $ECHO_C" >&6
else
  cat >conftest.$ac_ext <<_ACEOF
/* confdefs.h.  */
_ACEOF
cat confdefs.h >>conftest.$ac_ext
cat >>conftest.$ac_ext <<_ACEOF
/* end confdefs.h.  */
/* Define $ac_func to an innocuous variant, in case <limits.h> declares $ac_func.
   For example, HP-UX 11i <limits.h> declares gettimeofday.  */
#define $ac_func innocuous_$ac_func

/* System header to define __stub macros and hopefully few prototypes,
    which can conflict with char $ac_func (); below.
    Prefer <limits.h> to <assert.h> if __STDC__ is defined, since
    <limits.h> exists even on freestanding compilers.  */

#ifdef __STDC__
# include <limits.h>
#else
# include <assert.h>
#endif

#undef $ac_func

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char $ac_func ();
/* The GNU C library defines this for functions which it implements
    to always fail with ENOSYS.  Some functions are actually named
    something starting with __ and the normal name is an alias.  */
#if defined __stub_$ac_func || defined __stub___$ac_func
choke me
#endif

int
main ()
{
return $ac_func ();
  ;
  return 0;
}
_ACEOF
rm -f conftest.$ac_objext conftest$ac_exeext
if { (ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_link") 2>conftest.er1
  ac_status=$?
  grep -v '^ *+' conftest.er1 >conftest.err
  rm -f conftest.er1
  cat conftest.err >&5
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); } &&
	 { ac_try='test -z "$ac_c_werror_flag" || test ! -s conftest.err'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; } &&
	 { ac_try='test -s conftest$ac_exeext'
  { (case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval "echo \"\$as_me:$LINENO: $ac_try_echo\"") >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  echo "$as_me:$LINENO: \$? = $ac_status" >&5
  (exit $ac_status); }; }; then
  eval "$as_ac_var=yes"
else
  echo "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	eval "$as_ac_var=no"
fi

rm -f core conftest.err conftest.$ac_objext \
      conftest$ac_exeext conftest.$ac_ext
fi
ac_res=`eval echo '${'$as_ac_var'}'`
	       { echo "$as_me:$LINENO: result: $ac_res" >&5
echo "${ECHO_T}$ac_res" >&6; }
if test `eval echo '${'$as_ac_var'}'` = yes; then
  cat >>confdefs.h <<_ACEOF
#define `echo "HAVE_$ac_func" | $as_tr_cpp` 1
_ACEOF

fi
done



ac_config_files="$ac_config_files Makefile"

cat >confcache <<\_ACEOF
# This file is a shell script that caches the results of configure
# tests run on this system so they can be shared between configure
# scripts and configure runs, see configure's option --config-cache.
# It is not useful on other systems.  If it contains results you don't
# want to keep, you may remove or edit it.
#
# config.status only pays attention to the cache file if you give it
# the --recheck option to rerun configure.
#
# `ac_cv_env_foo' variables (set or unset) will be overridden when
# loading this file, other *unset* `ac_cv_foo' will be assigned the
# following values.

_ACEOF

# The following way of writing the cache mishandles newlines in values,
# but we know of no workaround that is simple, portable, and efficient.
# So, we kill variables containing newlines.
# Ultrix sh set writes to stderr and can't be redirected directly,
# and sets the high bit in the cache file unless we assign to the vars.
(
  for ac_var in `(set) 2>&1 | sed -n 's/^\([a-zA-Z_][a-zA-Z0-9_]*\)=.*/\1/p'`; do
    eval ac_val=\$$ac_var
    case $ac_val in #(
    *${as_nl}*)
      case $ac_var in #(
      *_cv_*) { echo "$as_me:$LINENO: WARNING: Cache variable $ac_var contains a newline." >&5
echo "$as_me: WARNING: Cache variable $ac_var contains a newline." >&2;} ;;
      esac
      case $ac_var in #(
      _ | IFS | as_nl) ;; #(
      *) $as_unset $ac_var ;;
      esac ;;
    esac
  done

  (set) 2>&1 |
    case $as_nl`(ac_space=' '; set) 2>&1` in #(
    *${as_nl}ac_space=\ *)
      # `set' does not quote correctly, so add quotes (double-quote
      # substitution turns \\\\ into \\, and sed turns \\ into \).
      sed -n \
	"s/'/'\\\\''/g;
	  s/^\\([_$as_cr_alnum]*_cv_[_$as_cr_alnum]*\\)=\\(.*\\)/\\1='\\2'/p"
      ;; #(
    *)
      # `set' quotes correctly as required by POSIX, so do not add quotes.
      sed -n "/^[_$as_cr_alnum]*_cv_[_$as_cr_alnum]*=/p"
      ;;
    esac |
    sort
) |
  sed '
     /^ac_cv_env_/b end
     t clear
     :clear
     s/^\([^=]*\)=\(.*[{}].*\)$/test "${\1+set}" = set || &/
     t end
     s/^\([^=]*\)=\(.*\)$/\1=${\1=\2}/
     :end' >>confcache
if diff "$cache_file" confcache >/dev/null 2>&1; then :; else
  if test -w "$cache_file"; then
    test "x$cache_file" != "x/dev/null" &&
      { echo "$as_me:$LINENO: updating cache $cache_file" >&5
echo "$as_me: updating cache $cache_file" >&6;}
    cat confcache >$cache_file
  else
    { echo "$as_me:$LINENO: not updating unwritable cache $cache_file" >&5
echo "$as_me: not updating unwritable cache $cache_file" >&6;}
  fi
fi
rm -f confcache

test "x$prefix" = xNONE && prefix=$ac_default_prefix
# Let make expand exec_prefix.
test "x$exec_prefix" = xNONE && exec_prefix='${prefix}'

DEFS=-DHAVE_CONFIG_H

ac_libobjs=
ac_ltlibobjs=
for ac_i in : $LIBOBJS; do test "x$ac_i" = x: && continue
  # 1. Remove the extension, and $U if already installed.
  ac_script='s/\$U\././;s/\.o$//;s/\.obj$//'
  ac_i=`echo "$ac_i" | sed "$ac_script"`
  # 2. Prepend LIBOBJDIR.  When used with automake>=1.10 LIBOBJDIR
  #    will be set to the directory where LIBOBJS objects are built.
  ac_libobjs="$ac_libobjs \${LIBOBJDIR}$ac_i\$U.$ac_objext"
  ac_ltlibobjs="$ac_ltlibobjs \${LIBOBJDIR}$ac_i"'$U.lo'
done
LIBOBJS=$ac_libobjs

LTLIBOBJS=$ac_ltlibobjs



: ${CONFIG_STATUS=./config.status}
ac_clean_files_save=$ac_clean_files
ac_clean_files="$ac_clean_files $CONFIG_STATUS"
{ echo "$as_me:$LINENO: creating $CONFIG_STATUS" >&5
echo "$as_me: creating $CONFIG_STATUS" >&6;}
cat >$CONFIG_STATUS <<_ACEOF
#! $SHELL
# Generated by $as_me.
# Run this file to recreate the current configuration.
# Compiler output produced by configure, useful for debugging
# configure, is in config.log if it exists.

debug=false
ac_cs_recheck=false
ac_cs_silent=false
SHELL=\${CONFIG_SHELL-$SHELL}
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
## --------------------- ##
## M4sh Initialization.  ##
## --------------------- ##

# Be Bourne compatible
if test -n "${ZSH_VERSION+set}" && (emulate sh) >/dev/null 2>&1; then
  emulate sh
  NULLCMD=:
  # Zsh 3.x and 4.x performs word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else
  case `(set -o) 2>/dev/null` in *posix*) set -o posix;; esac
fi
BIN_SH=xpg4; export BIN_SH # for Tru64
DUALCASE=1; export DUALCASE # for MKS sh


# PATH needs CR
# Avoid depending upon Character Ranges.
as_cr_letters='abcdefghijklmnopqrstuvwxyz'
as_cr_LETTERS='ABCDEFGHIJKLMNOPQRSTUVWXYZ'
as_cr_Letters=$as_cr_letters$as_cr_LETTERS
as_cr_digits='0123456789'
as_cr_alnum=$as_cr_Letters$as_cr_digits

# The user is always right.
if test "${PATH_SEPARATOR+set}" != set; then
  echo "#! /bin/sh" >conf$$.sh
  echo  "exit 0"   >>conf$$.sh
  chmod +x conf$$.sh
  if (PATH="/nonexistent;."; conf$$.sh) >/dev/null 2>&1; then
    PATH_SEPARATOR=';'
  else
    PATH_SEPARATOR=:
  fi
  rm -f conf$$.sh
fi

# Support unset when possible.
if ( (MAIL=60; unset MAIL) || exit) >/dev/null 2>&1; then
  as_unset=unset
else
  as_unset=false
fi


# IFS
# We need space, tab and new line, in precisely that order.  Quoting is
# there to prevent editors from complaining about space-tab.
# (If _AS_PATH_WALK were called with IFS unset, it would disable word
# splitting by setting IFS to empty value.)
as_nl='
'
IFS=" ""	$as_nl"

# Find who we are.  Look in the path if we contain no directory separator.
case $0 in
  *[\\/]* ) as_myself=$0 ;;
  *) as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  test -z "$as_dir" && as_dir=.
  test -r "$as_dir/$0" && as_myself=$as_dir/$0 && break
done
IFS=$as_save_IFS

     ;;
esac
# We did not find ourselves, most probably we were run as `sh COMMAND'
# in which case we are not to be found in the path.
if test "x$as_myself" = x; then
  as_myself=$0
fi
if test ! -f "$as_myself"; then
  echo "$as_myself: error: cannot find myself; rerun with an absolute file name" >&2
  { (exit 1); exit 1; }
fi

# Work around bugs in pre-3.0 UWIN ksh.
for as_var in ENV MAIL MAILPATH
do ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
done
PS1='$ '
PS2='> '
PS4='+ '

# NLS nuisances.
for as_var in \
  LANG LANGUAGE LC_ADDRESS LC_ALL LC_COLLATE LC_CTYPE LC_IDENTIFICATION \
  LC_MEASUREMENT LC_MESSAGES LC_MONETARY LC_NAME LC_NUMERIC LC_PAPER \
  LC_TELEPHONE LC_TIME
do
  if (set +x; test -z "`(eval $as_var=C; export $as_var) 2>&1`"); then
    eval $as_var=C; export $as_var
  else
    ($as_unset $as_var) >/dev/null 2>&1 && $as_unset $as_var
  fi
done

# Required to use basename.
if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

if (basename -- /) >/dev/null 2>&1 && test "X`basename -- / 2>&1`" = "X/"; then
  as_basename=basename
else
  as_basename=false
fi


# Name of the executable.
as_me=`$as_basename -- "$0" ||
$as_expr X/"$0" : '.*/\([^/][^/]*\)/*$' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
echo X/"$0" |
    sed '/^.*\/\([^/][^/]*\)\/*$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`

# CDPATH.
$as_unset CDPATH



  as_lineno_1=$LINENO
  as_lineno_2=$LINENO
  test "x$as_lineno_1" != "x$as_lineno_2" &&
  test "x`expr $as_lineno_1 + 1`" = "x$as_lineno_2" || {

  # Create $as_me.lineno as a copy of $as_myself, but with $LINENO
  # uniformly replaced by the line number.  The first 'sed' inserts a
  # line-number line after each line using $LINENO; the second 'sed'
  # does the real work.  The second script uses 'N' to pair each
  # line-number line with the line containing $LINENO, and appends
  # trailing '-' during substitution so that $LINENO is not a special
  # case at line end.
  # (Raja R Harinath suggested sed '=', and Paul Eggert wrote the
  # scripts with optimization help from Paolo Bonzini.  Blame Lee
  # E. McMahon (1931-1989) for sed's syntax.  :-)
  sed -n '
    p
    /[$]LINENO/=
  ' <$as_myself |
    sed '
      s/[$]LINENO.*/&-/
      t lineno
      b
      :lineno
      N
      :loop
      s/[$]LINENO\([^'$as_cr_alnum'_].*\n\)\(.*\)/\2\1\2/
      t loop
      s/-\n.*//
    ' >$as_me.lineno &&
  chmod +x "$as_me.lineno" ||
    { echo "$as_me: error: cannot create $as_me.lineno; rerun with a POSIX shell" >&2
   { (exit 1); exit 1; }; }

  # Don't try to exec as it changes $[0], causing all sort of problems
  # (the dirname of $[0] is not the place where we might find the
  # original and so on.  Autoconf is especially sensitive to this).
  . "./$as_me.lineno"
  # Exit status is that of the last command.
  exit
}


if (as_dir=`dirname -- /` && test "X$as_dir" = X/) >/dev/null 2>&1; then
  as_dirname=dirname
else
  as_dirname=false
fi

ECHO_C= ECHO_N= ECHO_T=
case `echo -n x` in
-n*)
  case `echo 'x\c'` in
  *c*) ECHO_T='	';;	# ECHO_T is single tab character.
  *)   ECHO_C='\c';;
  esac;;
*)
  ECHO_N='-n';;
esac

if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

rm -f conf$$ conf$$.exe conf$$.file
if test -d conf$$.dir; then
  rm -f conf$$.dir/conf$$.file
else
  rm -f conf$$.dir
  mkdir conf$$.dir
fi
echo >conf$$.file
if ln -s conf$$.file conf$$ 2>/dev/null; then
  as_ln_s='ln -s'
  # ... but there are two gotchas:
  # 1) On MSYS, both `ln -s file dir' and `ln file dir' fail.
  # 2) DJGPP < 2.04 has no symlinks; `ln -s' creates a wrapper executable.
  # In both cases, we have to default to `cp -p'.
  ln -s conf$$.file conf$$.dir 2>/dev/null && test ! -f conf$$.exe ||
    as_ln_s='cp -p'
elif ln conf$$.file conf$$ 2>/dev/null; then
  as_ln_s=ln
else
  as_ln_s='cp -p'
fi
rm -f conf$$ conf$$.exe conf$$.dir/conf$$.file conf$$.file
rmdir conf$$.dir 2>/dev/null

if mkdir -p . 2>/dev/null; then
  as_mkdir_p=:
else
  test -d ./-p && rmdir ./-p
  as_mkdir_p=false
fi

# Find out whether ``test -x'' works.  Don't use a zero-byte file, as
# systems may use methods other than mode bits to determine executability.
cat >conf$$.file <<_ASEOF
#! /bin/sh
exit 0
_ASEOF
chmod +x conf$$.file
if test -x conf$$.file >/dev/null 2>&1; then
  as_executable_p="test -x"
else
  as_executable_p=:
fi
rm -f conf$$.file

# Sed expression to map a string onto a valid CPP name.
as_tr_cpp="eval sed 'y%*$as_cr_letters%P$as_cr_LETTERS%;s%[^_$as_cr_alnum]%_%g'"

# Sed expression to map a string onto a valid variable name.
as_tr_sh="eval sed 'y%*+%pp%;s%[^_$as_cr_alnum]%_%g'"


exec 6>&1

# Save the log message, to keep $[0] and so on meaningful, and to
# report actual input values of CONFIG_FILES etc. instead of their
# values after options handling.
ac_log="
This file was extended by $as_me, which was
generated by GNU Autoconf 2.60.  Invocation command line was

  CONFIG_FILES    = $CONFIG_FILES
  CONFIG_HEADERS  = $CONFIG_HEADERS
  CONFIG_LINKS    = $CONFIG_LINKS
  CONFIG_COMMANDS = $CONFIG_COMMANDS
  $ $0 $@

on `(hostname || uname -n) 2>/dev/null | sed 1q`
"

_ACEOF

cat >>$CONFIG_STATUS <<_ACEOF
# Files that config.status was made for.
config_files="$ac_config_files"
config_headers="$ac_config_headers"

_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
ac_cs_usage="\
\`$as_me' instantiates files from templates according to the
current configuration.

Usage: $0 [OPTIONS] [FILE]...

  -h, --help       print this help, then exit
  -V, --version    print version number, then exit
  -q, --quiet      do not print progress messages
  -d, --debug      don't remove temporary files
      --recheck    update $as_me by reconfiguring in the same conditions
  --file=FILE[:TEMPLATE]
		   instantiate the configuration file FILE
  --header=FILE[:TEMPLATE]
		   instantiate the configuration header FILE

Configuration files:
$config_files

Configuration headers:
$config_headers

Report bugs to <bug-autoconf@gnu.org>."

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
ac_cs_version="\\
config.status
configured by $0, generated by GNU Autoconf 2.60,
  with options \\"`echo "$ac_configure_args" | sed 's/^ //; s/[\\""\`\$]/\\\\&/g'`\\"

Copyright (C) 2006 Free Software Foundation, Inc.
This config.status script is free software; the Free Software Foundation
gives unlimited permission to copy, distribute and modify it."

ac_pwd='$ac_pwd'
srcdir='$srcdir'
INSTALL='$INSTALL'
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
# If no file are specified by the user, then we need to provide default
# value.  By we need to know if files were specified by the user.
ac_need_defaults=:
while test $# != 0
do
  case $1 in
  --*=*)
    ac_option=`expr "X$1" : 'X\([^=]*\)='`
    ac_optarg=`expr "X$1" : 'X[^=]*=\(.*\)'`
    ac_shift=:
    ;;
  *)
    ac_option=$1
    ac_optarg=$2
    ac_shift=shift
    ;;
  esac

  case $ac_option in
  # Handling of the options.
  -recheck | --recheck | --rechec | --reche | --rech | --rec | --re | --r)
    ac_cs_recheck=: ;;
  --version | --versio | --versi | --vers | --ver | --ve | --v | -V )
    echo "$ac_cs_version"; exit ;;
  --debug | --debu | --deb | --de | --d | -d )
    debug=: ;;
  --file | --fil | --fi | --f )
    $ac_shift
    CONFIG_FILES="$CONFIG_FILES $ac_optarg"
    ac_need_defaults=false;;
  --header | --heade | --head | --hea )
    $ac_shift
    CONFIG_HEADERS="$CONFIG_HEADERS $ac_optarg"
    ac_need_defaults=false;;
  --he | --h)
    # Conflict between --help and --header
    { echo "$as_me: error: ambiguous option: $1
Try \`$0 --help' for more information." >&2
   { (exit 1); exit 1; }; };;
  --help | --hel | -h )
    echo "$ac_cs_usage"; exit ;;
  -q | -quiet | --quiet | --quie | --qui | --qu | --q \
  | -silent | --silent | --silen | --sile | --sil | --si | --s)
    ac_cs_silent=: ;;

  # This is an error.
  -*) { echo "$as_me: error: unrecognized option: $1
Try \`$0 --help' for more information." >&2
   { (exit 1); exit 1; }; } ;;

  *) ac_config_targets="$ac_config_targets $1"
     ac_need_defaults=false ;;

  esac
  shift
done

ac_configure_extra_args=

if $ac_cs_silent; then
  exec 6>/dev/null
  ac_configure_extra_args="$ac_configure_extra_args --silent"
fi

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
if \$ac_cs_recheck; then
  echo "running CONFIG_SHELL=$SHELL $SHELL $0 "$ac_configure_args \$ac_configure_extra_args " --no-create --no-recursion" >&6
  CONFIG_SHELL=$SHELL
  export CONFIG_SHELL
  exec $SHELL "$0"$ac_configure_args \$ac_configure_extra_args --no-create --no-recursion
fi

_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF
exec 5>>config.log
{
  echo
  sed 'h;s/./-/g;s/^.../## /;s/...$/ ##/;p;x;p;x' <<_ASBOX
## Running $as_me. ##
_ASBOX
  echo "$ac_log"
} >&5

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF

# Handling of arguments.
for ac_config_target in $ac_config_targets
do
  case $ac_config_target in
    "config.h") CONFIG_HEADERS="$CONFIG_HEADERS config.h" ;;
    "Makefile") CONFIG_FILES="$CONFIG_FILES Makefile" ;;

  *) { { echo "$as_me:$LINENO: error: invalid argument: $ac_config_target" >&5
echo "$as_me: error: invalid argument: $ac_config_target" >&2;}
   { (exit 1); exit 1; }; };;
  esac
done


# If the user did not use the arguments to specify the items to instantiate,
# then the envvar interface is used.  Set only those that are not.
# We use the long form for the default assignment because of an extremely
# bizarre bug on SunOS 4.1.3.
if $ac_need_defaults; then
  test "${CONFIG_FILES+set}" = set || CONFIG_FILES=$config_files
  test "${CONFIG_HEADERS+set}" = set || CONFIG_HEADERS=$config_headers
fi

# Have a temporary directory for convenience.  Make it in the build tree
# simply because there is no reason against having it here, and in addition,
# creating and moving files from /tmp can sometimes cause problems.
# Hook for its removal unless debugging.
# Note that there is a small window in which the directory will not be cleaned:
# after its creation but before its name has been assigned to `$tmp'.
$debug ||
{
  tmp=
  trap 'exit_status=$?
  { test -z "$tmp" || test ! -d "$tmp" || rm -fr "$tmp"; } && exit $exit_status
' 0
  trap '{ (exit 1); exit 1; }' 1 2 13 15
}
# Create a (secure) tmp directory for tmp files.

{
  tmp=`(umask 077 && mktemp -d "./confXXXXXX") 2>/dev/null` &&
  test -n "$tmp" && test -d "$tmp"
}  ||
{
  tmp=./conf$$-$RANDOM
  (umask 077 && mkdir "$tmp")
} ||
{
   echo "$me: cannot create a temporary directory in ." >&2
   { (exit 1); exit 1; }
}

#
# Set up the sed scripts for CONFIG_FILES section.
#

# No need to generate the scripts if there are no CONFIG_FILES.
# This happens for instance when ./config.status config.h
if test -n "$CONFIG_FILES"; then

_ACEOF



ac_delim='%!_!# '
for ac_last_try in false false false false false :; do
  cat >conf$$subs.sed <<_ACEOF
SHELL!$SHELL$ac_delim
PATH_SEPARATOR!$PATH_SEPARATOR$ac_delim
PACKAGE_NAME!$PACKAGE_NAME$ac_delim
PACKAGE_TARNAME!$PACKAGE_TARNAME$ac_delim
PACKAGE_VERSION!$PACKAGE_VERSION$ac_delim
PACKAGE_STRING!$PACKAGE_STRING$ac_delim
PACKAGE_BUGREPORT!$PACKAGE_BUGREPORT$ac_delim
exec_prefix!$exec_prefix$ac_delim
prefix!$prefix$ac_delim
program_transform_name!$program_transform_name$ac_delim
bindir!$bindir$ac_delim
sbindir!$sbindir$ac_delim
libexecdir!$libexecdir$ac_delim
datarootdir!$datarootdir$ac_delim
datadir!$datadir$ac_delim
sysconfdir!$sysconfdir$ac_delim
sharedstatedir!$sharedstatedir$ac_delim
localstatedir!$localstatedir$ac_delim
includedir!$includedir$ac_delim
oldincludedir!$oldincludedir$ac_delim
docdir!$docdir$ac_delim
infodir!$infodir$ac_delim
htmldir!$htmldir$ac_delim
dvidir!$dvidir$ac_delim
pdfdir!$pdfdir$ac_delim
psdir!$psdir$ac_delim
libdir!$libdir$ac_delim
localedir!$localedir$ac_delim
mandir!$mandir$ac_delim
DEFS!$DEFS$ac_delim
ECHO_C!$ECHO_C$ac_delim
ECHO_N!$ECHO_N$ac_delim
ECHO_T!$ECHO_T$ac_delim
LIBS!$LIBS$ac_delim
build_alias!$build_alias$ac_delim
host_alias!$host_alias$ac_delim
target_alias!$target_alias$ac_delim
VERSION!$VERSION$ac_delim
MAINT!$MAINT$ac_delim
CC!$CC$ac_delim
CFLAGS!$CFLAGS$ac_delim
LDFLAGS!$LDFLAGS$ac_delim
CPPFLAGS!$CPPFLAGS$ac_delim
ac_ct_CC!$ac_ct_CC$ac_delim
EXEEXT!$EXEEXT$ac_delim
OBJEXT!$OBJEXT$ac_delim
INSTALL_PROGRAM!$INSTALL_PROGRAM$ac_delim
INSTALL_SCRIPT!$INSTALL_SCRIPT$ac_delim
INSTALL_DATA!$INSTALL_DATA$ac_delim
LN_S!$LN_S$ac_delim
SET_MAKE!$SET_MAKE$ac_delim
TTF_OPT!$TTF_OPT$ac_delim
TEXMF!$TEXMF$ac_delim
CPP!$CPP$ac_delim
GREP!$GREP$ac_delim
EGREP!$EGREP$ac_delim
LIBOBJS!$LIBOBJS$ac_delim
LTLIBOBJS!$LTLIBOBJS$ac_delim
_ACEOF

  if test `sed -n "s/.*$ac_delim\$/X/p" conf$$subs.sed | grep -c X` = 58; then
    break
  elif $ac_last_try; then
    { { echo "$as_me:$LINENO: error: could not make $CONFIG_STATUS" >&5
echo "$as_me: error: could not make $CONFIG_STATUS" >&2;}
   { (exit 1); exit 1; }; }
  else
    ac_delim="$ac_delim!$ac_delim _$ac_delim!! "
  fi
done

ac_eof=`sed -n '/^CEOF[0-9]*$/s/CEOF/0/p' conf$$subs.sed`
if test -n "$ac_eof"; then
  ac_eof=`echo "$ac_eof" | sort -nru | sed 1q`
  ac_eof=`expr $ac_eof + 1`
fi

cat >>$CONFIG_STATUS <<_ACEOF
cat >"\$tmp/subs-1.sed" <<\CEOF$ac_eof
/@[a-zA-Z_][a-zA-Z_0-9]*@/!b end
_ACEOF
sed '
s/[,\\&]/\\&/g; s/@/@|#_!!_#|/g
s/^/s,@/; s/!/@,|#_!!_#|/
:n
t n
s/'"$ac_delim"'$/,g/; t
s/$/\\/; p
N; s/^.*\n//; s/[,\\&]/\\&/g; s/@/@|#_!!_#|/g; b n
' >>$CONFIG_STATUS <conf$$subs.sed
rm -f conf$$subs.sed
cat >>$CONFIG_STATUS <<_ACEOF
:end
s/|#_!!_#|//g
CEOF$ac_eof
_ACEOF


# VPATH may cause trouble with some makes, so we remove $(srcdir),
# ${srcdir} and @srcdir@ from VPATH if srcdir is ".", strip leading and
# trailing colons and then remove the whole line if VPATH becomes empty
# (actually we leave an empty line to preserve line numbers).
if test "x$srcdir" = x.; then
  ac_vpsub='/^[	 ]*VPATH[	 ]*=/{
s/:*\$(srcdir):*/:/
s/:*\${srcdir}:*/:/
s/:*@srcdir@:*/:/
s/^\([^=]*=[	 ]*\):*/\1/
s/:*$//
s/^[^=]*=[	 ]*$//
}'
fi

cat >>$CONFIG_STATUS <<\_ACEOF
fi # test -n "$CONFIG_FILES"


for ac_tag in  :F $CONFIG_FILES  :H $CONFIG_HEADERS
do
  case $ac_tag in
  :[FHLC]) ac_mode=$ac_tag; continue;;
  esac
  case $ac_mode$ac_tag in
  :[FHL]*:*);;
  :L* | :C*:*) { { echo "$as_me:$LINENO: error: Invalid tag $ac_tag." >&5
echo "$as_me: error: Invalid tag $ac_tag." >&2;}
   { (exit 1); exit 1; }; };;
  :[FH]-) ac_tag=-:-;;
  :[FH]*) ac_tag=$ac_tag:$ac_tag.in;;
  esac
  ac_save_IFS=$IFS
  IFS=:
  set x $ac_tag
  IFS=$ac_save_IFS
  shift
  ac_file=$1
  shift

  case $ac_mode in
  :L) ac_source=$1;;
  :[FH])
    ac_file_inputs=
    for ac_f
    do
      case $ac_f in
      -) ac_f="$tmp/stdin";;
      *) # Look for the file first in the build tree, then in the source tree
	 # (if the path is not absolute).  The absolute path cannot be DOS-style,
	 # because $ac_f cannot contain `:'.
	 test -f "$ac_f" ||
	   case $ac_f in
	   [\\/$]*) false;;
	   *) test -f "$srcdir/$ac_f" && ac_f="$srcdir/$ac_f";;
	   esac ||
	   { { echo "$as_me:$LINENO: error: cannot find input file: $ac_f" >&5
echo "$as_me: error: cannot find input file: $ac_f" >&2;}
   { (exit 1); exit 1; }; };;
      esac
      ac_file_inputs="$ac_file_inputs $ac_f"
    done

    # Let's still pretend it is `configure' which instantiates (i.e., don't
    # use $as_me), people would be surprised to read:
    #    /* config.h.  Generated by config.status.  */
    configure_input="Generated from "`IFS=:
	  echo $* | sed 's|^[^:]*/||;s|:[^:]*/|, |g'`" by configure."
    if test x"$ac_file" != x-; then
      configure_input="$ac_file.  $configure_input"
      { echo "$as_me:$LINENO: creating $ac_file" >&5
echo "$as_me: creating $ac_file" >&6;}
    fi

    case $ac_tag in
    *:-:* | *:-) cat >"$tmp/stdin";;
    esac
    ;;
  esac

  ac_dir=`$as_dirname -- "$ac_file" ||
$as_expr X"$ac_file" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$ac_file" : 'X\(//\)[^/]' \| \
	 X"$ac_file" : 'X\(//\)$' \| \
	 X"$ac_file" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$ac_file" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  { as_dir="$ac_dir"
  case $as_dir in #(
  -*) as_dir=./$as_dir;;
  esac
  test -d "$as_dir" || { $as_mkdir_p && mkdir -p "$as_dir"; } || {
    as_dirs=
    while :; do
      case $as_dir in #(
      *\'*) as_qdir=`echo "$as_dir" | sed "s/'/'\\\\\\\\''/g"`;; #(
      *) as_qdir=$as_dir;;
      esac
      as_dirs="'$as_qdir' $as_dirs"
      as_dir=`$as_dirname -- "$as_dir" ||
$as_expr X"$as_dir" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$as_dir" : 'X\(//\)[^/]' \| \
	 X"$as_dir" : 'X\(//\)$' \| \
	 X"$as_dir" : 'X\(/\)' \| . 2>/dev/null ||
echo X"$as_dir" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
      test -d "$as_dir" && break
    done
    test -z "$as_dirs" || eval "mkdir $as_dirs"
  } || test -d "$as_dir" || { { echo "$as_me:$LINENO: error: cannot create directory $as_dir" >&5
echo "$as_me: error: cannot create directory $as_dir" >&2;}
   { (exit 1); exit 1; }; }; }
  ac_builddir=.

case "$ac_dir" in
.) ac_dir_suffix= ac_top_builddir_sub=. ac_top_build_prefix= ;;
*)
  ac_dir_suffix=/`echo "$ac_dir" | sed 's,^\.[\\/],,'`
  # A ".." for each directory in $ac_dir_suffix.
  ac_top_builddir_sub=`echo "$ac_dir_suffix" | sed 's,/[^\\/]*,/..,g;s,/,,'`
  case $ac_top_builddir_sub in
  "") ac_top_builddir_sub=. ac_top_build_prefix= ;;
  *)  ac_top_build_prefix=$ac_top_builddir_sub/ ;;
  esac ;;
esac
ac_abs_top_builddir=$ac_pwd
ac_abs_builddir=$ac_pwd$ac_dir_suffix
# for backward compatibility:
ac_top_builddir=$ac_top_build_prefix

case $srcdir in
  .)  # We are building in place.
    ac_srcdir=.
    ac_top_srcdir=$ac_top_builddir_sub
    ac_abs_top_srcdir=$ac_pwd ;;
  [\\/]* | ?:[\\/]* )  # Absolute name.
    ac_srcdir=$srcdir$ac_dir_suffix;
    ac_top_srcdir=$srcdir
    ac_abs_top_srcdir=$srcdir ;;
  *) # Relative name.
    ac_srcdir=$ac_top_build_prefix$srcdir$ac_dir_suffix
    ac_top_srcdir=$ac_top_build_prefix$srcdir
    ac_abs_top_srcdir=$ac_pwd/$srcdir ;;
esac
ac_abs_srcdir=$ac_abs_top_srcdir$ac_dir_suffix


  case $ac_mode in
  :F)
  #
  # CONFIG_FILE
  #

  case $INSTALL in
  [\\/$]* | ?:[\\/]* ) ac_INSTALL=$INSTALL ;;
  *) ac_INSTALL=$ac_top_build_prefix$INSTALL ;;
  esac
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF
# If the template does not know about datarootdir, expand it.
# FIXME: This hack should be removed a few years after 2.60.
ac_datarootdir_hack=; ac_datarootdir_seen=

case `sed -n '/datarootdir/ {
  p
  q
}
/@datadir@/p
/@docdir@/p
/@infodir@/p
/@localedir@/p
/@mandir@/p
' $ac_file_inputs` in
*datarootdir*) ac_datarootdir_seen=yes;;
*@datadir@*|*@docdir@*|*@infodir@*|*@localedir@*|*@mandir@*)
  { echo "$as_me:$LINENO: WARNING: $ac_file_inputs seems to ignore the --datarootdir setting" >&5
echo "$as_me: WARNING: $ac_file_inputs seems to ignore the --datarootdir setting" >&2;}
_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF
  ac_datarootdir_hack='
  s&@datadir@&$datadir&g
  s&@docdir@&$docdir&g
  s&@infodir@&$infodir&g
  s&@localedir@&$localedir&g
  s&@mandir@&$mandir&g
    s&\\\${datarootdir}&$datarootdir&g' ;;
esac
_ACEOF

# Neutralize VPATH when `$srcdir' = `.'.
# Shell code in configure.ac might set extrasub.
# FIXME: do we really want to maintain this feature?
cat >>$CONFIG_STATUS <<_ACEOF
  sed "$ac_vpsub
$extrasub
_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF
:t
/@[a-zA-Z_][a-zA-Z_0-9]*@/!b
s&@configure_input@&$configure_input&;t t
s&@top_builddir@&$ac_top_builddir_sub&;t t
s&@srcdir@&$ac_srcdir&;t t
s&@abs_srcdir@&$ac_abs_srcdir&;t t
s&@top_srcdir@&$ac_top_srcdir&;t t
s&@abs_top_srcdir@&$ac_abs_top_srcdir&;t t
s&@builddir@&$ac_builddir&;t t
s&@abs_builddir@&$ac_abs_builddir&;t t
s&@abs_top_builddir@&$ac_abs_top_builddir&;t t
s&@INSTALL@&$ac_INSTALL&;t t
$ac_datarootdir_hack
" $ac_file_inputs | sed -f "$tmp/subs-1.sed" >$tmp/out

test -z "$ac_datarootdir_hack$ac_datarootdir_seen" &&
  { ac_out=`sed -n '/\${datarootdir}/p' "$tmp/out"`; test -n "$ac_out"; } &&
  { ac_out=`sed -n '/^[	 ]*datarootdir[	 ]*:*=/p' "$tmp/out"`; test -z "$ac_out"; } &&
  { echo "$as_me:$LINENO: WARNING: $ac_file contains a reference to the variable \`datarootdir'
which seems to be undefined.  Please make sure it is defined." >&5
echo "$as_me: WARNING: $ac_file contains a reference to the variable \`datarootdir'
which seems to be undefined.  Please make sure it is defined." >&2;}

  rm -f "$tmp/stdin"
  case $ac_file in
  -) cat "$tmp/out"; rm -f "$tmp/out";;
  *) rm -f "$ac_file"; mv "$tmp/out" $ac_file;;
  esac
 ;;
  :H)
  #
  # CONFIG_HEADER
  #
_ACEOF

# Transform confdefs.h into a sed script `conftest.defines', that
# substitutes the proper values into config.h.in to produce config.h.
rm -f conftest.defines conftest.tail
# First, append a space to every undef/define line, to ease matching.
echo 's/$/ /' >conftest.defines
# Then, protect against being on the right side of a sed subst, or in
# an unquoted here document, in config.status.  If some macros were
# called several times there might be several #defines for the same
# symbol, which is useless.  But do not sort them, since the last
# AC_DEFINE must be honored.
ac_word_re=[_$as_cr_Letters][_$as_cr_alnum]*
# These sed commands are passed to sed as "A NAME B PARAMS C VALUE D", where
# NAME is the cpp macro being defined, VALUE is the value it is being given.
# PARAMS is the parameter list in the macro definition--in most cases, it's
# just an empty string.
ac_dA='s,^\\([	 #]*\\)[^	 ]*\\([	 ]*'
ac_dB='\\)[	 (].*,\\1define\\2'
ac_dC=' '
ac_dD=' ,'

uniq confdefs.h |
  sed -n '
	t rset
	:rset
	s/^[	 ]*#[	 ]*define[	 ][	 ]*//
	t ok
	d
	:ok
	s/[\\&,]/\\&/g
	s/^\('"$ac_word_re"'\)\(([^()]*)\)[	 ]*\(.*\)/ '"$ac_dA"'\1'"$ac_dB"'\2'"${ac_dC}"'\3'"$ac_dD"'/p
	s/^\('"$ac_word_re"'\)[	 ]*\(.*\)/'"$ac_dA"'\1'"$ac_dB$ac_dC"'\2'"$ac_dD"'/p
  ' >>conftest.defines

# Remove the space that was appended to ease matching.
# Then replace #undef with comments.  This is necessary, for
# example, in the case of _POSIX_SOURCE, which is predefined and required
# on some systems where configure will not decide to define it.
# (The regexp can be short, since the line contains either #define or #undef.)
echo 's/ $//
s,^[	 #]*u.*,/* & */,' >>conftest.defines

# Break up conftest.defines:
ac_max_sed_lines=50

# First sed command is:	 sed -f defines.sed $ac_file_inputs >"$tmp/out1"
# Second one is:	 sed -f defines.sed "$tmp/out1" >"$tmp/out2"
# Third one will be:	 sed -f defines.sed "$tmp/out2" >"$tmp/out1"
# et cetera.
ac_in='$ac_file_inputs'
ac_out='"$tmp/out1"'
ac_nxt='"$tmp/out2"'

while :
do
  # Write a here document:
    cat >>$CONFIG_STATUS <<_ACEOF
    # First, check the format of the line:
    cat >"\$tmp/defines.sed" <<\\CEOF
/^[	 ]*#[	 ]*undef[	 ][	 ]*$ac_word_re[	 ]*\$/b def
/^[	 ]*#[	 ]*define[	 ][	 ]*$ac_word_re[(	 ]/b def
b
:def
_ACEOF
  sed ${ac_max_sed_lines}q conftest.defines >>$CONFIG_STATUS
  echo 'CEOF
    sed -f "$tmp/defines.sed"' "$ac_in >$ac_out" >>$CONFIG_STATUS
  ac_in=$ac_out; ac_out=$ac_nxt; ac_nxt=$ac_in
  sed 1,${ac_max_sed_lines}d conftest.defines >conftest.tail
  grep . conftest.tail >/dev/null || break
  rm -f conftest.defines
  mv conftest.tail conftest.defines
done
rm -f conftest.defines conftest.tail

echo "ac_result=$ac_in" >>$CONFIG_STATUS
cat >>$CONFIG_STATUS <<\_ACEOF
  if test x"$ac_file" != x-; then
    echo "/* $configure_input  */" >"$tmp/config.h"
    cat "$ac_result" >>"$tmp/config.h"
    if diff $ac_file "$tmp/config.h" >/dev/null 2>&1; then
      { echo "$as_me:$LINENO: $ac_file is unchanged" >&5
echo "$as_me: $ac_file is unchanged" >&6;}
    else
      rm -f $ac_file
      mv "$tmp/config.h" $ac_file
    fi
  else
    echo "/* $configure_input  */"
    cat "$ac_result"
  fi
  rm -f "$tmp/out12"
 ;;


  esac

done # for ac_tag


{ (exit 0); exit 0; }
_ACEOF
chmod +x $CONFIG_STATUS
ac_clean_files=$ac_clean_files_save


# configure is writing to config.log, and then calls config.status.
# config.status does its own redirection, appending to config.log.
# Unfortunately, on DOS this fails, as config.log is still kept open
# by configure, so config.status won't be able to write to it; its
# output is simply discarded.  So we exec the FD to /dev/null,
# effectively closing config.log, so it can be properly (re)opened and
# appended to by config.status.  When coming back to configure, we
# need to make the FD available again.
if test "$no_create" != yes; then
  ac_cs_success=:
  ac_config_status_args=
  test "$silent" = yes &&
    ac_config_status_args="$ac_config_status_args --quiet"
  exec 5>/dev/null
  $SHELL $CONFIG_STATUS $ac_config_status_args || ac_cs_success=false
  exec 5>>config.log
  # Use ||, not &&, to avoid exiting from the if with $? = 1, which
  # would make configure fail if this is the last instruction.
  $ac_cs_success || { (exit 1); exit 1; }
fi



==> dvipdfm/doc/dvipdfm.tex <==
% $Header$
% \special{ pdf: pagesize width 8.5truein height 11.0truein}
\special{  pdf:  docview <</PageMode /UseOutlines>>}%
\catcode`\ =11\def\space{ }\catcode`\ =10
% Page layout
\tolerance=2000
\magnification\magstephalf
\advance\hoffset by 0.5truein
\advance\voffset by 0.5truein
\advance\hsize by -1.0truein
\advance\vsize by -1.0truein
\def\makefootline{\baselineskip=40pt\line{\the\footline}}
%
%  Some helpful symbols
\def\rtm{{\font\r=cmss10 at 4pt
\font\c=cmsy5
\setbox0\hbox{\c\char13}\skip0\wd0\box0\setbox0\hbox{\r R}\advance\skip0 by
\wd0\kern-0.5\skip0\box0}}
\def\tm{{\font\r=cmss10 at 4pt \hbox{\r TM}}}%
%
% Verbatim mode borrowed from manmac macros
%
\outer\def\begindisplay{\obeylines\startdisplay}
{\obeylines\gdef\startdisplay#1
  {\catcode`\^^M=5$$#1\halign\bgroup\indent##\hfil&&\qquad##\hfil\cr}}
\outer\def\enddisplay{\crcr\egroup$$}
\chardef\other=12
\def\ttverbatim{\begingroup \catcode`\\=\other \catcode`\{=\other
 \catcode`\}=\other \catcode`\$=\other \catcode `\&=\other
 \catcode`\#=\other \catcode`\%=\other \catcode `\~=\other
 \catcode`\_=\other \catcode`\^=\other
  \obeyspaces \obeylines \tt}
{\obeyspaces\gdef {\ }}
\outer\def\begintt{$$\let\par=\endgraf\ttverbatim \parskip=0pt
 \catcode`\|=0 \rightskip=-5pc \ttfinish}
{\catcode`\|=0 |catcode`|\=\other
 |obeylines % end of line is now active
 |gdef|ttfinish#1^^M#2\endtt{#1|vbox{#2}|endgroup$$}}
\catcode`\|=\active
{\obeylines\gdef|{\ttverbatim\spaceskip=\ttglue\let^^M=\ \let|=\endgroup}}
\newskip\ttglue
\ttglue=0.5em plus 0.25em minus 0.15em
%
%
% Some color definitions
% 
\def\begincolor#1{\special{pdf:bc #1}}%
\def\endcolor{\special{pdf:ec}}%
\def\colored#1#2{%
  \begincolor{#1}#2\endcolor}
\def\red{[0.8 0.5 0]}%
\def\green{[0 1 0]}%
\def\blue{[0 0.4 0.8]}%
\def\yellow{[0.8 0.9 0.1]}%
\def\linkcolor{[0.5 0.0 0.7]}%
%
% Small help for images
\def\reserve#1#2#3{\setbox0\hbox{}\wd0=#1
                   \ht0=#2\special{#3}\box0}
\def\nreserve#1#2#3{\setbox0\hbox{}\wd0=#1
                   \ht0=#2{#3}\box0}
%
% Some font definitions
%
\font\maintitlefont=cmti12 at 20.74pt
\font\headingfont=cmss12 at 14.4pt
\font\subheadingfont=cmss12 at 12pt
%
%
% Miscellaneous token lists
%
\newtoks\title\newtoks\author\newtoks\version
\newtoks\date
%
% Bibliography counters
\newcount\biblioitems\biblioitems=0
\def\bibitem{\medskip\advance\biblioitems by 1\item{[\the\biblioitems]}}
%
% Counters for section levels
%
\newcount\sectioncount\newcount\ssectioncount\newcount\sssectioncount
\sectioncount0\ssectioncount0\sssectioncount0
%
\newskip\indentlevel\indentlevel=\parindent
\newskip\secskip\secskip=24pt plus 1pt minus 2pt
\newskip\subsecskip\subsecskip=16pt plus 1pt minus 2pt
\def\beginlist{\par\nobreak\advance\leftskip by \indentlevel\advance\rightskip by
\indentlevel\medskip\nobreak}
\def\endlist{\par\advance\leftskip by -\indentlevel\advance\rightskip by
-\indentlevel\medskip}
%
%
\def\settitle{%
  {\maintitlefont\colored{\blue}{\the\title}}%
  \special {pdf:  docinfo << /Title (\expandafter\the\title) >>}}
%
\def\setauthor{%
  {\headingfont\colored{\blue}{\the\author}}%
  \special {pdf:  docinfo << /Author (\the\author) >>}}%
%
\def\setversion{%
  {\subheadingfont{\the\version}}%
}%
\def\setdate{%
  {\subheadingfont{\the\date}}%
}%
\def\setlink#1{\colored{\linkcolor}{#1}}%
%  
\def\setheading#1{%
  {\headingfont\colored{\blue}{#1}}\raise\baselineskip
  \hbox{\special{pdf: outline 1 << /Title (#1) /Dest [
@thispage /FitH @ypos ]  >> }}}%
%
\def\setsubheading#1{%
  {\subheadingfont\colored{\blue}{#1}}\raise\baselineskip
  \hbox{\special{pdf: outline 2 << /Title (#1) /Dest [
@thispage /FitH @ypos ]  >> }}}%
%
% \def\link#1#2{\setbox0\hbox{\setlink{#1}}%
%    \leavevmode\special{pdf: ann width \the\wd0\space height \the\ht0\space depth \the\dp0
%      << /Type /Annot /Subtype /Link /Border [ 0 0 0 ] /A << /S /GoTo
%      /D (#2) >> >>}\box0\relax}%
\def\link#1#2{%
  \leavevmode\special{pdf: bann 
    << /Type /Annot /Subtype /Link /Border [ 0 0 0 ] /A << /S /GoTo /D (#2)
>>
>>}\setlink{#1}\special{pdf: eann}\relax}
%
\def\dest#1{\hbox{\raise14pt\hbox{\special{pdf:dest (#1) [ @thispage /FitH
@ypos ]}}}}%
%
\def\maketitle{\noindent\settitle\hfill\setauthor\par
          \hrule height 1.0pt\medskip
          \noindent\setversion\hfill\setdate\vskip0.3in}%
%
\def\section#1{\advance\sectioncount by 1\ssectioncount0
\vskip-\lastskip\vskip\secskip\goodbreak
\noindent\setheading{\the\sectioncount. #1}\medskip\nobreak}%
\def\subsection#1{\vskip-\lastskip\advance\ssectioncount by 1%
\vskip\subsecskip\noindent
\setsubheading{\the\sectioncount.\the\ssectioncount\
          #1}\par\nobreak\smallskip}%
%
\def\display#1{\medskip\line{\quad #1\hfil}\medskip}
\def\example{\medskip\noindent{\it Example:\quad}\nobreak}
\def\note{\medskip\noindent{\it Note:\quad\nobreak}}
\def\syntax{\medskip\noindent{\it Syntax:\quad}\nobreak}
\def\description{\medskip\noindent{\it Description:\quad}\nobreak}
%
\def\newpage{\vfill\eject}
%
\def\dvipdfm{{\tt dvipdfm}}%
%
\title{Dvipdfm User's Manual}
\author{Mark A. Wicks}
\version{Version 0.12.4b}
\date{September 19, 1999}
\maketitle
\section{Introduction}
This package is a DVI (\TeX) to PDF conversion utility,
having the following features:

\beginlist
\item{$\bullet$} {\it Support for outline entries (also called bookmarks), named destinations,
and \link{annotations}{Annotate} (including hyperlinks, forms and widgets).}  Nearly
every Acrobat Distiller pdfmark is approximated.

\item{$\bullet$} {\it Support for ``standard'' DVI specials such
as Hyper\TeX\ (HTML), TPIC, color specials, |PSfile|, and other PostScript specials.}

\item{$\bullet$} {\it Native support for inclusion of
\link{MetaPost}{postscript} output and
inclusion of arbitrary \link{PostScript}{postscript} files with help from an external program.}

\item{$\bullet$} {\it Support for thumbnails with a little help from GhostScript to
generate the thumbnails.}

\item{$\bullet$} {\it Support for arbitrary, nested linear transformations
of typeset material.}  Any material on the page, including
\TeX\ text, may be \link{scaled and rotated}{textxform}.

\item{$\bullet$} {\it Ability to include the first page of a \link{PDF file}{pdfimage} as
an encapsulated object along with its embedded resources such as fonts.}
Included PDF images may be cropped by supplying a bounding box.
Note:  Currently, this doesn't work if the contents stream
has multiple segments. 

\item{$\bullet$} {\it Ability to include \link{JPEG}{jpegimage} and
PNG bitmapped images as encapsulated objects.}

\item{$\bullet$} {\it An internal color stack.} A color stack allows you to change the current color, pushing the
current color onto a stack.  At any time, the original color
can be popped from the stack.  This is useful, for example, in
headlines, that may have a different color from the current text.
The headline macro can restore the current color without knowing
what it is.

\item{$\bullet$} {\it Support for partial font embedding and Flate compression
to reduce file size}

\item{$\bullet$} {\it Support for font reencoding to work around encodings
that aren't fully supported by the Acrobat suite of products.}

\item{$\bullet$} {\it Balanced page and destination trees.} Balancing
these trees improves reader access speed 
on very large documents.

\endlist

The electronic version of the document exercises
some of the hypertext features and serves as
a sample input file for |dvipdfm|.
It assumes the reader has some familiarity with the basic features
of the Portable Document Format.  The PDF specification
is distributed by Adobe Systems\link{[1]}{pdfmanual}.
An excellent source for information about PDF documents
in general is \link{[2]}{pdfprimer}.  Information about
using \TeX\ to construct PDF documents (mainly using Distiller) is the
AcroTeX home page\link{[3]}{acrotex}.

Currently, the widely accepted method to generate PDF file from \TeX\
is to use Adobe's Acrobat Distiller on a PostScript
file produced by {\tt dvips}.
The hyperlink features are accessed by using \TeX\ |special| primitives
to embed pdfmarks in the PostScript produced by |dvips|.
H\`an Th\'e Th\`an's PDF\TeX\ project is an alternative method
of generating PDF from \TeX\ source.
Although quite good and fairly mature, the PDF\TeX\ project
modified \TeX\ itself to add primitives that support the PDF features.
I prefer to work with \TeX\ unmodified, as released by Donald Knuth
(call me a purist).
There is an existing DVI to PDF driver called
|dvipdf| written by Sergey Lesenko.  At present, it's not widely
available, so I haven't used it.  I wrote |dvipdfm|
mainly as an exercise to get at the features
of PDF I was trying to use.  This |dvipdfm| project demonstrates that many features
of PDF can be accessed by using a DVI driver.
The PDF features are activated in the driver via
\TeX\ |special| primitives.

Even though Distiller is the best method of generating PDF (and
probably will remain so for some time) I have several reasons for
seeking alternatives to Distiller.
First, Distiller isn't available for my principle operating
system---Linux.

My second objection is philosophical.
\TeX\ is a programming language.
A DVI file is a page description consisting of very
simple program instructions that have no branching or
decision instructions.
Similarly PostScript is a complete programming language,
while PDF is a page description language consisting
of simple program instructions
without any branching or decision capabilities.
\TeX\ is like PostScript (without the graphics)
while DVI is like PDF (without the graphics or the hyperlinks).
Creating PDF from DVI using Distiller requires converting a page description to a program,
and converting that program back to a page description.
To continue this analogy,
Pdfmarks are PostScript ``escapes'' and are meant for the Distiller.
\TeX\ |\special| primitives are \TeX\ ``escapes'' and are meant for the DVI driver.
It seems natural to go directly from DVI to PDF, where \TeX\ replaces
PostScript, the DVI driver replaces Distiller,
and \TeX\ |\special| primitives replace the pdfmarks.

Unfortunately, until graphics software
begins to produce PDF content streams or encapsulated
PDF objects, PostScript will remain the easiest
way to include graphics in \TeX\ documents.
I would hope that in the future, graphics programs
will begin to produce PDF content streams or PDF objects that
may be included using a DVI to PDF translator.  Either
of these may be easily embedded using \dvipdfm\ or a similar driver.

\section{Command Line Options}
\link{Table~1}{commandline} lists the options
that are available on the command line.
\par\noindent
Note: Several flags may be specified at once:
\example
\begintt
dvipdfm -ecz 9 test.dvi
\endtt

\topinsert
{\dest{commandline}}
\centerline{\colored{\blue}{\subheadingfont Table~1---Command line options
recognized by |dvipdfm|}}
\bigskip\nobreak
\centerline{\vbox{\halign{{\tt #}\hskip
1em\strut&\vtop{\leftskip0pt\rightskip0pt\hsize=3.5in\noindent #}\cr
\omit\hfil\it Option\hfil&\omit\hfil \it Description \hfil\cr
\noalign{\smallskip\begincolor\red\hrule\endcolor\smallskip}
-c&{\it Disable color specials}  Specifying this option
forces all color commands to be ignored.  This is useful for printing a color document
on a black and white printer.\cr
\noalign{\smallskip}
-e&{\it Disable partial font embedding.}  This may be useful
for forms which need complete fonts, or if you run accross a PFB
file that \dvipdfm\ cannot correctly parse.\cr
\noalign{\smallskip}
-f&{\it Set font map file name}.  See
the \link{Font Mapping}{fontmap} section for additional information.\cr
\noalign{\smallskip}
-m {\it number}&{\it Specify an additional magnification for
the document}.\cr
\noalign{\smallskip}
-o {\it filename}&{\it Set the output PDF file name}.\cr
\noalign{\smallskip}
-p {\it papersize}&{\it Specify the output papersize.}
Valid paper sizes are |letter|, |legal|, |ledger|, |tabloid|,
|a4|, or |a3|.  The default is |letter|.  Arbitrary paper
sizes can be specified via \TeX\ special commands,
which is the recommended method.\cr
\noalign{\smallskip}
-l&{\it Landscape the document.}  This is only
meaningful for paper sizes specified on the command line.\cr
\noalign{\smallskip}
-s {\it page\_ranges}&{\it Select a subset of pages from the DVI file.}
The {\it page\_ranges} specifier is a set of comma-separated page
ranges---e.g., |dvipdfm -s 10-12,10-20|.  If the first
page in a range is empty (e.g., |dvipdfm -s -10|), it represents
the beginning of the document.  If
the last page in a range is empty (e.g., |dvipdfm -s 10-|), it selects the end of the document.\cr
\noalign{\smallskip}
-t&{\it Embed thumbnail images.} The thumbnails must be generated by a
separate program. Details are discussed \link{later}{thumbnails} in this document\cr
\noalign{\smallskip}
-d&{\it Delete thumbnail images after embedding.}\cr
\noalign{\smallskip}
-x {\it number}&{\it Specify the horizontal offset
for the document.}  The default is 1.0in.\cr
\noalign{\smallskip}
-y {\it number}&{\it Specify the vertical offset
for the document.}  The default is 1.0in.\cr
\noalign{\smallskip}
-z {\it number}&{\it Specify the compression level.}
Valid compression levels range from 0 to 9, with 0 indicating
no compression.  A compression level of 9 is the default.\cr
\noalign{\smallskip}
-v&{\it Be verbose.}  Among other things, dvipdfm
will display complete file names as various files are opened.\cr
\noalign{\smallskip}
-vv&{\it Be more verbose.}\cr}}}
\endinsert

\section{General Concepts and Syntax for TeX Specials}
Each \TeX\ |\special|
represents a separate command to the \dvipdfm\ 
driver.  Each |special| must begin with ``|pdf:|''
to identify that ||special|| as a command for the \dvipdfm\ driver.
A |\special| beginning with any other characters is ignored
by the driver.  Leading spaces are ignored.  The characters ``|pdf:|''
are immediately followed by a \dvipdfm\ command.  These commands
are documented in \hbox{Sections~3--6}.

\subsection{PDF Object Syntax and Variable Expansion}
With one exception, the syntax used for PDF objects
within each |\special| specials follows
the PDF specification.
The one exception is variable expansion.
In the syntax specifications that follow, {\it PDF\_Object}
means that an arbitary PDF object is expected.  Similarly
{\it PDF\_Array} indicates that a PDF array is expected, {\it PDF\_Dict}
inciates that a PDF dictionary is expected, etc.
See the \link{reference manual}{pdfmanual}\
for a complete list of PDF object types.

The single extension implemented in this driver
allows a symbol name of the
form |@|{\it name} whereever any PDF object is expected.
The {\it name} may contain any characters allowed
in a PDF name.
A user-defined symbol beginning with |@| expands to an indirect
reference to the user-defined PDF object.  This feature replaces
the |{|{\it name}|}| syntax used with pdfmarks.
In addition to the user-defined names, some names
are defined by the driver.
The driver defined variables are for
referencing objects such as the current page, future pages,
or the current location on the current page.
The driver defined variables appear in \link{Table~2}{drivervariables}.
\topinsert
{\dest{drivervariables}}
\centerline{\colored{\blue}{\subheadingfont Table~2---List of driver
defined variables}}
\bigskip\nobreak
\centerline{\vbox{\halign{{\tt #}\hskip
1em&\vtop{\leftskip0pt\rightskip0pt\hsize=3.0in\noindent #}\cr
\omit\hfil\it Variable\hfil&\omit\hfil \it Description \hfil\cr
\noalign{\smallskip\begincolor\red\hrule\endcolor\smallskip}
@catalog&A reference to the document's catalog.\cr
\noalign{\smallskip}
@names&A reference to the document's /Names dictionary.\cr
\noalign{\smallskip}
@pages&A reference to the root of the document's /Pages tree.\cr
\noalign{\smallskip}
@resources&A reference to the current page resource dictionary.\cr
\noalign{\smallskip}
@thispage&A reference to the current page.\cr
\noalign{\smallskip}
@page{\it n}&A reference to page {\it n}.\cr
\noalign{\smallskip}
@nextpage&A reference to the page following |@thispage|.\cr
\noalign{\smallskip}
@prevpage&A reference to the page preceding |@thispage|.\cr
\noalign{\smallskip}
@ypos&A {\it number} representing the current vertical position in units of PDF points.\cr
\noalign{\smallskip}
@xpos&A {\it number} representing the current horizontal position in units of PDF points.\cr
}}}
\endinsert

In the syntax specifications that follow, several
standard conventions are followed.  Terminal
characters that appear in the command 
are typeset in the |\tt| font, e.g., |object|.
Nonterminal symbols are typeset in italics.
Optional parameters are surrounded by brackets, e.g.,
[{\it optional\_argument}].  An item followed
by~``{*}'' represents an item that may appear
zero or more times.  An item followed by~``{+}''
represents a required item that may appear multiple times.

\subsection{Dimensions and transformations}
Interaction with the |dvipdfm| driver consists
of short commands with a few arguments delimited by white space.
Typically the arguments are PDF objects.
Two exceptions are dimension specifications and transformations.

In the \TeX\ style, a dimension specification consists of one of the keywords
|width|, |height|, or |depth| followed by a dimension
consisting of a numerical value, followed by a unit for the dimension.  The
unit will typically be |pt| (which represents a \TeX\ point, not a
PDf point) but |mm|, |cm| and |in| are also allowed.
If the document is magnified, the ``true'' dimensions |truept|,
|truemm|, |truecm|, and |truein| may be used.  The notation
{\it dimension\/} in a syntax description means a dimension is expected.

A transformation consists of one of the keywords |scale|, |xscale|,
|yscale|, or |rotate| followed by a numerical value.  In the
case of |rotate| the value is the rotation angle in degrees.
The notation
{\it transformation} means a transformation is expected.
In the case of included images originating from
PDF/PostScript files, a clipping or bounding box may be specified
as part of the ``transformation.''  The bounding
box specification consists of the keyword |bbox|
followed by four numerical values, which are 
the standard PostScript |llx|, |lly|, |urx|, and |ury|
coordinates of the bounding box.

\section{Document Construction Commands}
All commands are executed via \TeX\ |\special| primitives
prefixed with the characters ``|pdf:|''.
\example
\begintt
\special{ pdf: out 1 << /Title (Introduction)
                        /Dest [ 1 0 R /FitH 234 ] >>
\endtt

\dest{Annotate}
\subsection{Annotate}
\hbox to 0pt{\hskip-1.0in\special{pdf: ann width 3.0in height 36pt << /Type /Annot /Subtype /Text
/Contents (This is a /Text Annotation that looks like a sticky note.) >>}\hss}
\syntax
{\tt annotate} [{\tt @}{\it name}] {\it dimension}+ {\it PDF\_dictionary}
\description
The |annotate| (|annot| or |ann|) command defines an annotation.
Annotations are typically used for
notes, hyperlinks, forms, or widgets.
The parameter {\it name} is an optional alphanumeric identifier
and {\it PDF\_dictionary} is a valid PDF dictionary after variable expansion.
If {\tt @}{\it name} is specified, it may be used in
other PDF objects to refer to this annotation.
One or more {\it dimension} parameters are required
and each consists of the keyword
{\tt height}, {\tt width}, or {\tt depth} followed
by an appropriate length, specified as per \TeX\null.
The |width| must be nonzero and either the |height| or |depth|
must be nonzero.
Each length is a number followed by a unit, such as {\tt pt},
{\tt in}, or {\tt cm}.  Since these values
would typically be entered by \TeX, a {\tt pt}
is a \TeX\ point, not a PDF point.

\example The annotation in this subsection
was typeset with
\begintt
\special{pdf: ann width 3.0in height 36pt
     << /Type /Annot /Subtype /Text
        /Contents (This is a /Text Annotation 
        that looks like a sticky note.) >>}
\endtt

\subsection{Begin Annotation}
\syntax
{\tt beginann} {\it PDF\_dictionary}
\description
The |beginann| (|bann| or |bannot|) command begins a breakable annotation.
Dvipdfm tries to determine the boundaries of the annotation automatically.
Such an annotation may be broken over several lines (or even several pages).
Unlike |annot|, the annotation may be not be referred to by name later,
since there may be more than once instances of the annotation.
The |beginann| command needs not dimension because |dvipdfm|
computes the correct bounding box on the fly.

Note:  Link breaking is easily fooled at page breaks.  If you have problems
with the header or footer wanting to become part of the link, you can
insert a |nolink| command at the beginning of the footer and a |link|
command at the end of the footer.

\subsection{End Annotation}
\syntax
{\tt endann}
\description
The |endann| (|eann| or |eannot|) terminates a breakable annotation.

\subsection{Link}
{\tt link}
\description
The |link| command instructs the link breaking algorithm to resume its
operation after a |nolink| command.

\subsection{Nolink}
{\tt nolink}
\description
The |nolink| command instructs the link breaking algorithm to suspend
it operation.  This is only required if there is material inserted
on the page in the {\it middle} of a link.  For example, when a link
is broken at the end of a page, the header and footer are inserted
in the middle of the link, but are not part of the link.  Material
that is inserted between a |nolink| and |link| will not become
part of the link.  The |nolink| and |link| escapes are not necessary
with the standard LaTeX header and footer lines, but may become necessary
if these are changed.

\subsection{Dest}
\syntax
{\tt dest} {\it PDF\_String} {\it PDF\_Dest}
\description
The |dest| command defines a named destination.
The {\it PDF\_String} is a PDF string naming
the destination.  This string may be used in the destination
fields of annotations and outline entries to refer to
this destination.  {\it PDF\_Dest} is a PDF
destination object (typically an array).
\example
\begintt
\special{pdf: dest (listofreferences) [ @thispage /FitH @ypos ]}
\endtt

\subsection{Docinfo}
\syntax
{\tt docinfo} {\it PDF\_dictionary}
\description
The |docinfo| command adds the keys in the specified dictionary to the
document's |/Info| dictionary.  All keys are optional, but may include
the keys |/Author|, |/Title|, |/Keywords|, |/Subject|,
and |/Creator|.
\example
\begintt
\special{pdf: docinfo << /Author (Mark A. Wicks)
                         /Title (This Document) >>}
\endtt

\subsection{Docview}
\syntax
{\tt docview} {\it PDF\_dictionary}
\description
The |docview| command adds the keys in the specified dictionary to the
document's |/Catalog| dictionary.  All keys are optional, but may include
the keys |/PageMode|,
|/URI|, |/OpenAction|, |/AA|
and |/ViewerPreferences|.  See the PDF Reference Manual
for documentation of these keys and additional keys.
\example
\begintt
\special{pdf: docview << /PageMode /UseThumbs >> }
\endtt


\subsection{Object}
\syntax
{\tt object} [@{\it name}] {\it PDF\_Object}
\description
The |object| (also |obj|) command creates a
PDF object.  The parameter {\it PDF\_Object} is any valid PDF object.  The
parameter {\it name} may be used to provide an indirect reference
to this object within other
objects. It will be expanded anywhere within
a {\tt special} where a PDF object is
expected. Typically {\it object} is an array
or dictionary.  It may be an empty array or
dictionary that can be constructed dynamically via
the {\tt put} command.
\example
\begintt
\special{pdf: object @mydict << /Firstpage @thispage >>}
\endtt

\subsection{Out}
\syntax
{\tt out} {\it number} {\it PDF\_dictionary}

\description
The |out| (also |outline|) command adds an outline (also called a ``bookmark'') entry
to the document.
The parameter {\it level\/} is an integer representing the
level of the outline entry (beginning with 1) and
{\it  PDF\_dictionary\/} must contain
the two keys {\tt /Title} and either {\tt /Dest} or {\tt /A}.
It may also contain the {\tt /AA} key.  These keys are documented
in the PDF Reference Manual.
\example
\begintt
out 1 << /Title (Section 1) /Dest [ @thispage /FitH @ypos ] >>
\endtt
which may be followed by
\begintt
out 2 << /Title (Section 1.1) /Dest [ @thispage /FitH @ypos ] >>
\endtt
\note
You may not skip levels.  A level~2 outline entry
must follow a level~1 outline
entry.  A level~3 outline entry must follow a level~2 outline
and cannot immediately follow a level 1 outline entry.

\subsection{Pagesize}
\syntax
{\tt pagesize} {\it dimension}+
\description
The |pagesize| command specifies the document's physical
paper size.  The |pagesize| command must be specified on
the first page and must precede the first annotation
or background color specification on the page.
In other words, it should occur as close to the
beginning of the document as possible.
\example
\begintt
pagesize width 11.0truein height 8.5truein
\endtt

\subsection{Put}
\syntax
\beginlist
{\tt put} @{\it name} {\it PDF\_Object}+
\endlist
or 
\beginlist
{\tt put} @{\it name} {\it PDF\_Dictionary}
\endlist
\description
The |put| command modifies an existing PDF object created with |obj|,
or one of the following internally defined objects: |@catalog|,
|@names|, |@pages|, |@thispage|, or |@resources|.
The first form is used when @{\it name} is an array.  The second
form is used when @{\tt name} is a dictionary.  More than
one object may be added to an array at once.
All keys in {\it PDF\_Dictionary}
are added to the dictionary represented by @{\it name}.
\example
\begintt
\special{pdf: put @mydict << /Nextpage @thispage >>}
\endtt

\subsection{Thread}
\syntax
{\tt thread} {\tt @}{\it name} {\it dimension}+ [ {\it PDF\_dictionary} ]

\description
The |thread| (or |art|) command adds a bead to an article.
An article is a collection of boxed regions in the document that should be
read consecutively.
Each bead using the same {\it name} belongs to the same article.
The {\it name} parameter is required.  The {\it dimension} parameter
defined the rectangular area belonging to the bead in
the same manner as for |annot|.
The optional PDF dictionary 
should supplied on one of the beads.  Its keys are
similar to the |/Info| dictionary accessed via the |docinfo| command
and would typically include the |/Title| and |/Author| keys.
Keys in the dictionary may be overwritten by subsequent {\tt thread} commands.
\example
\begintt
\special {pdf: thread @somearticle << /Title (Some title)
                                       /Author (Me) >>}
\endtt

\subsection{Close}
\syntax
{\tt close} @{\it name}
\description
The |close| writes the named PDF object created with |obj| to the PDF file.
No further |put| commands may be executed for this object.
The object may continue to be referenced using @{\it name}
indefinitely.  If the object is never closed, it will
be closed when |dvipdfm| finishes processing the document.

\section{Form XObjects}
The PDF specification allows an object to be stored once
and displayed at multiple locations throughout the document.
The following commands give access to this facility.

\subsection{Beginxobj}
\syntax
{\tt beginxobj} @{\it name} {\it dimension}+
\description
The |beginxobj| (or |bxobj|) command begins the definition of
a Form XObject.  All material typeset between the
|beginxobj| and |endxobj| commands will be captured
into the XObject.  The material can be displayed later
at an arbitrary location with the |usexobj| command.
The {\it name} may be used to refer to the object later,
either via the |usexobj| command or as an indirect
reference to the XObject if {\it name} is
used within the context of a {\it PDF\_Object}..
The required {\it dimension} identifies the extent
(i.e., bounding box) of the area to be captured.
It is specified in the same way as for |annot|.

The material will not display during the object definition.
In other words, if you are typsetting with \TeX\ you
should place the XObject in a box of dimension 0 so
you don't leave a white space hole where the object was
defined.
\example
\begintt
bxobj @myform width 2.0in height 24pt
\endtt

\subsection{Endxobj}
\syntax
{\tt endxobj}
\description
The |endxobj| (or |exobj|) command ends the previous
|beginxobj| definition.  Note that XObject definitions
may not be nested.  XObjects can be {\it used} within
other XObjects, however.
\example
\begintt
exobj
\endtt

\subsection{Usexobj}
\syntax
{\tt usexobj} @{\it name}
\description
The |usexobj| (or |uxobj|) command displays the 
form XObject previously defined and
associated with {\it name}.
\example
\begintt
uxobj @myform
\endtt

\section{Text Transformation Commands}
The commands in this section deal with transformation
of arbitrary material, which may include
material typeset by \TeX.  These
may also be used on included graphics images
if the commands in Section~8 won't do the job.

\subsection{BeginTransform}
\syntax
{\tt begintransform} {\it transformation}+

\description
The |begintransform| (|btrans| or |bt|) applies
the specified transformation to all subsequent text.
The scaling is applied first, followed by the rotation.
The reference point of a box following
the |\special| remains fixed.  Such transformations
may be nested to perform rotations within rotated text, for exmaple.

\example
\begintt
\special{pdf: bt rotate 90 xscale 2.0 }
\endtt

\subsection{BeginTransform}
\syntax
{\tt endtransform}
\description
The |endtransform| (|etrans| or |et|) concludes
the action of the immediately preceding |begintransform|
command.  All transformations must be closed
on the same page.  The driver will close
any pending unclosed transformations at the
end of the page and issue a warning message.
All material to be transformed
should probably be enclosed in a single box
to prevent any break.
\example
\begintt
\special{pdf: et}
\endtt


\section{Color Commands}
The commands in this section deal with manipulation of the color
stack.

\subsection{Setcolor}
\syntax
{\tt setcolor} {\it PDF\_Number$\vert$\it PDF\_Array}
\description
The |setcolor| (|scolor| or |sc|) command uses its
argument to set the default color for future marking operators.
The current color is replaced and may be retrieved
only by a subsequent |setcolor| command.  The argument
may be a single number, which is interpreted as a grayscale
value; a three element array, which is interpreted as an RGB
color space coordinate; or a four element array, which
is interpreted as a CMYK color space coordinate.
\example
\begintt
\special{ pdf: sc [ 1 0 0 ] }
\endtt

\subsection{Begincolor}
\syntax
{\tt begincolor} {\it PDF\_Number$\vert$\it PDF\_Array}
\description
The |begincolor| (|bcolor| or |bc|) command uses its
argument to set the default color for future marking operators.
The current color is pushed on the color stack.  The argument
may be a single number, which is interpreted as a grayscale
value; a three element array, which is interpreted as an RGB
color space coordinate; or a four element array, which
is interpreted as a CMYK color space coordinate.
\example
\begintt
\special{ pdf: bc [ 1 0 0 ] }
\endtt

\subsection{Endcolor}
\syntax
{\tt endcolor}
\description
The |endcolor| (|ecolor| or |ec|)
changes the default color to
match the color on the top
of the stack.  It removes
the color from the stack.
\example
\begintt
\special{ pdf: ec }
\endtt

\subsection{Bgcolor}
\syntax
{\tt bgcolor} {\it PDF\_Number$\vert$\it PDF\_Array}
\description
The |bgcolor| (|bbc| or |bgc|) command uses the value
of its argument to set the default color for the page
background.  The interpretation
fo the argument is the same as for the |begincolor| command.
The stack is not involved here.  There is no way
to go back to the previous background color.
\example
\begintt
\special{ pdf: bc [ 1 0 0 ] }
\endtt

\section{Image Commands}
The commands in this section deal with embedding
graphics into your PDF document.  The present
driver supports PDF, PNG, and JPEG graphics inclusion.

\subsection{Epdf}
\syntax
{\tt epdf} [|@|{\it name}] [{\it dimension}$\vert${\it transformation}]*  {\it PDF\_String}

\description
The {\tt epdf} command ``encapsulates'' the first page of a PDF
file named by {\it PDF\_String}
into a PDF XObject.  The resulting XObject is drawn
with the lower left corner at the current location of the page.
The optional @{\it name} parameter may be used
to reference this object within other objects.  If a
{\it dimension} is supplied, the object will be scaled to fit
that dimension.  A {\it transformation} consists of one of the keywords
|scale|, |xscale|, |yscale|, or |rotate|
followed by a number representing
the scaling factor or rotation angle in degrees.  Both {\it transformation} and {\it dimension}
parameters can be supplied as long as they are not logically
inconsistent.

Note: The object is stored as an XObject and can be redisplayed later by using the
|usexobj| function and specifying {\it name}.

\example
\begintt
\special{pdf:epdf yscale 0.50 width 4.0in
                              rotate 45 (circuit.pdf)}
\endtt

\subsection{Image}
\syntax
{\tt image} [@{\it name}] [{\it dimension} $\vert$ {\it transformation}]*  {\it PDF\_String}

\description
The {\tt image} command ``encapsulates'' an image
taken from the file named by {\it PDF\_String}.
This command functions just like |epdf|.  Value
image types may be PDF, JPEG, or PNG images.
This special will eventually replace the |epdf| special.

Note: The object is stored as an XObject and can be redisplayed later by using the
|usexobj| function and specifying {\it name}.

\section{Raw Page Marking Commands}
The commands in this section deal with embedding
raw PDF graphics operators into your PDF document.

\subsection{Bop}
\syntax
{\tt bop} {\it stream}
\description
The |bop| command specifies a marking
stream to be generated at the top of each page.
The parameter {\it stream} is any sequence
of marking operators and is added to the page's content stream.  
The stream is applied {\it to all pages} regardless
of where it appears in the document.
\example  The two horizontal lines appearing
at the top of each page in this document
were set with
\begintt
\special {pdf: bop  q 0 w 0.8 0.5 0 RG
               54 740 m 504 740 l 504 740.25 l 54 740.25 l b
               36 760 m 504 760 l 504 760.25 l 36 760.25 l b Q }
\endtt
\special {pdf: bop  q 0 w 0.8 0.5 0 RG
                           54 740 m 504 740 l 504 740.25 l 54 740.25 l b  
                           36 760 m 504 760 l 504 760.25 l 36 760.25 l b Q }

\subsection{Content}
\syntax
{\tt content} {\it stream}
\description
The |content| command specifies a marking
stream to be added to the current page at
the current location.  While it
is possible to change the color
state, etc., with this command, it is
not advised.  Use the color management
commands to change colors.


\subsection{Eop}
\syntax
\beginlist
{\tt eop} {\it stream}
\endlist
\description
The {\tt eop} specifies a marking stream to be generated at the end
of each page. The parameter {\it stream} is any sequence
of marking operators and is added to the page's content stream.  
The stream is applied {\it to all pages} regardless
of where it appears in the document.

\section{Graphics Examples}

The examples in this section illustrate some of the transformation
and image inclusion capabilities of \dvipdfm.

\dest{textxform}
\subsection{Text Transformation}
Tables with slanted entries are possible as shown
in \link{Table~3}{rotatedtable}.  This table was achieved using
various ``|bt rotate 35|'' commands.

The following line of text was done with nested
combinations of ``|bt rotate 10|'' and ``|bt rotate -10|''.

\def\up#1{\special{pdf:bt rotate 10}\hbox{#1}}
\def\down#1{\special{pdf:bt rotate -10}\hbox{#1}}
You \down{can} nest \down{the} \up{text}
trans\up{form}ation \up{capa}\down{bili}ties \down{to}
achieve \down{effects} \down{like}
{this}.
\special{pdf:et}\special{pdf:et}\special{pdf:et}\special{pdf:et}
\special{pdf:et}\special{pdf:et}\special{pdf:et}\special{pdf:et}
\special{pdf:et}
\vskip 0.5in


\def\rvr{\colored{\red}{\vrule}}\def\entry#1{\special{pdf:bt rotate 35}%
{\vbox to 0pt{\vss\hbox{\quad\colored{\blue}{#1}\quad}\vskip 1pt\colored{\red}{\hrule}}\special{pdf:et}}}
\topinsert
\dest{rotatedtable}
\bigskip
\centerline{\colored{\blue}{\subheadingfont Table 3---Example of rotated
text set in Computer Modern Roman}}
\bigskip
\centerline{\vbox to 0.45in{\vss\offinterlineskip\halign{#&#&#&#&#&#\cr
\entry{1994}&
\entry{1995}&
\entry{1996}&
\entry{1997}&
\entry{1998}&
\entry{1999}\cr
\noalign{\colored{\red}{\hrule}}
\strut\rvr&\rvr&\rvr&\rvr&\rvr&\rvr\crcr}}}
\bigskip
\endinsert

\dest{imageinclude}
\subsection{Image Inclusion}
 
The image in \link{Figure~1}{jpegimage} was included from a JPEG file.
The image shown in \link{Figure~2}{rotatedimage} comes from the same file,
but is loaded at a 50\% scale and a 45$^\circ$ rotation.

\topinsert
\dest{jpegimage}
\bigskip
\centerline{\reserve{1.50in}{2.05in}{pdf: image (mwicks.jpeg)}}
\medskip
\centerline{\subheadingfont
\begincolor{\blue}Figure~1---A JPEG image of the author.\endcolor}
\bigskip
\endinsert

\topinsert
\dest{rotatedimage}
\bigskip
\centerline{\reserve{0.75in}{1.25in}{pdf: image rotate 45 scale 0.50 (mwicks.jpeg)}}
\medskip
\centerline{\subheadingfont
\begincolor{\blue}Figure~2---Image of the author scaled by 0.5 and rotated
by 45$^\circ$.%
\endcolor}
\bigskip
\endinsert

By default, JPEG files are included
at a resolution of 100dpi so if you know the pixel size
of the image, you know how much space to reserve.
Any \TeX\ magnification is applied to the image
in addition to any scaling defined in the |\special|.
For example, this document sets |\magnification=\magstephalf|,
so the images are actually scaled by 1.095.  The first
image in this section has a printed width of 1.643in
even though 1.50in was specified in the |\special|.

Several command line utilities exist that read
the pixel dimensions of a JPEG file.  For PDF files,
you can |grep| on |/MediaBox| to get an indication
of the image size.  The |/MediaBox| dimensions are
in PDF points.

The image in \link{Figure~3}{pdfimage} was produced by embedding a PDF file
using |epdf|.

\topinsert
\dest{pdfimage}
\centerline{\reserve{2.41in}{2.6in}{pdf: epdf width 2.41in (transistor.pdf)}}
\medskip\centerline{\subheadingfont
\begincolor{\blue}Figure~3---An embedded PDF object.
\endcolor}
\endinsert
Notice that any resources required for the object
are also embedded.  In this case, the Times Roman font
resource was embedded along with the content stream.

\dest{thumbnails}\section{Thumbnails}
Thumbnails can be inserted automatically by |dvipdfm|
using the |-t| command line option.  However, |dvipdfm|
is unable to generate the thumbnails by itself.  This
must be done by some other program such as GhostScript.
The typical two-pass process to include thumbnails would be
\item{1.}
Run |dvipdfm| without the |-t| option (probably
using command line options optimized for speed and not space)
\item{2.}
Run GhostScript to generate the thumbnail images of
each page.
\item{3.}
Run |dvipdfm| with the |-t| or |-dt| option.

The |dvipdfm| distribution includes a sample
shell script called |dvipdft| which is a wrapper
for |dvipdfm| that generates thumbnails.

|Dvipdfm| searches for the thumbnail images
in the directory specified by the TMP or TEMP
environment variables, or in the current directory.
The thumbnails must have the same base name as the PDF output
file with an extension indicating the number of the page.
For example, to create a thumbnailed document named |foo.pdf|
you would need to generate thumbnail images in files named
|foo.1|, |foo.2|, etc.

\dest{fontmap}\section{Font Mapping}
\TeX\ font names can be
mapped into arbitrary physical (PostScript) font names via
the map file named |t1fonts.map|.  The file is
similar to the |psfonts.map| file used by |dvips|
and other drivers.  Each line in the
file consists of one to three fields delimited
by white space, followed by options that apply to that font.
The complete list of recognized options
appears in \link{Table~4}{options}.

Sample map file lines are\nobreak
\begintt
cmr10 ot1 -r
ptmro8r 8r Times-Roman -s 0.167
pncbo8r 8r pncb8a -s 0.167
\endtt

The first field of each line
is the \TeX\ font name.  The second
field, which is optional, is the encoding name (|.enc| will
be appended to this name, if necessary
to locate an encoding file).  The
encoding files have the same format
as those used for |dvips|.
The third optional field is {\it either} the PostScript font
name (if one of the standard PostScript fonts) {\it or}
the file name of a Type~1 binary font file (PFB file).
The {}.pfb extension is assumed by the program.
three fields. If the encoding field is unspecified,
|dvipdfm| used the default encoding supplied with
the Type~1 font.  If the name field is unspecified,
|dvipdfm| looks for a Type~1 binary font file
having the same name as the \TeX\ font name.
If there is {\it no} line in the map file,
the behavior is as if a line was specified
without the second or third field.
The keywords |default| or |none| are
recognized in the encoding field so that
a third field may be specified while still
having default behavior in the second field.

Currently, three options may be specified for each font
as shown in \link{Table~4}{options}.
\topinsert
{\dest{options}}
\centerline{\colored{\blue}{\subheadingfont Table~4---Font options
recognized by |dvipdfm| in the font map file}}
\bigskip\nobreak
\centerline{\vbox{\halign{{\tt #}\hskip
1em\strut&\vtop{\leftskip0pt\rightskip0pt\hsize=3.5in\noindent #}\cr
\omit\hfil\it Option\hfil&\omit\hfil \it Description \hfil\cr
\noalign{\smallskip\begincolor\red\hrule\endcolor\smallskip}
-r&{\it Remap the font to eliminate control characters.}  This
option attempts to work around bugs in Acrobat reader that seem
to be triggered by characters that are encoded in certain positions.
Unfortunately, standard \TeX encodings normally use these positions.\cr
\noalign{\smallskip}
-e {\it number}&{\it Extend the font horizontally, multiplying the natural
width of the font by the specified number.}  This is useful
for generating new fonts by widening existing fonts.\cr
\noalign{\smallskip}
-s {\it number}&{\it Slant the font using the specified number}.
This option is useful for building a slanted fonts from a font
for which there is no slanted font.\cr}}}
\endinsert

\section{Configuration file}
{\dest{configuration}}Dvipdfm reads default command line options, such
as paper size, from a configuration
file contained in the |dvipdfm| directory of the TeX tree.
The format of this file is similar to the |dvips| file configuration
file format.  Each line consists of a single command line switch
followed by any arguments.  See the configuration file supplied
with the |dvipdfm| distribution for examples.

\section{Including PostScript graphics images}
{\dest{postscript}}Dvipdfm provides support for illustrations
contained in external PostScript files. 
It recognizes two distinct kinds of PostScript files---those
created by MetaPost and everything else.

MetaPost
files output only a subset of PostScript and
are interpreted {\it natively} by |dvipdfm|
with its own internal minimal PostScript interpreter.
Also, MetaPost output files contain \TeX\ font information in their header
comments, so that they can be easily integrated with \TeX\ by DVI
drivers. Dvipdfm recognizes this font information and uses the \TeX\
fonts defined in the MetaPost header.


All other PostScript files require an external
program to convert the image to PDF format before
|dvipdfm| can include the image.
The freely available GhostScript is capabable of performing this conversion
for most images.

The user must specify the command line required
to invoke an external program to perform this conversion.
The command line required to invoke the conversion
program is specified using the |-D| command
line (or configuration file) option.  The string passed to the |-D| command
line option is a C-style string that is parsed by |dvipdfm|.  Within the string,
expansions are performed as described in \link{Table~5}{expansion}.
For example, to use GhostScript, one might use the
command line

\bigskip

{\tt -D "cat \%i \vrule\ gs -q -sDEVICE=pdfwrite -sOutputFile=\%o - -c quit" }


\topinsert
{\dest{expansion}}
\centerline{\colored{\blue}{\subheadingfont Table~5---Expansions
performed in the -D string.}}
\bigskip\nobreak
\centerline{\vbox{\halign{{\hfil\tt #\hfil}\hskip
1em\strut&\vtop{\leftskip0pt\rightskip0pt\hsize=3.5in\noindent #}\cr
\omit\hfil\it Variable\hfil&\omit\hfil \it Description \hfil\cr
\noalign{\smallskip\begincolor\red\hrule\endcolor\smallskip}
\%i&{\it Expanded to the full path of the EPS file to be included}\cr
\noalign{\smallskip}
\%o&{\it Expanded to the full path name of the PDF file to be
generated}.  The command line must be able to create a file
with the name supplied by dvipdfm.\cr
\noalign{\smallskip}
\%b&{\it Expanded to the  ``basename'' of the EPS file that is being included.}
The ``basename'' is the full path of the EPS file with the 
last ``.'' and any trailing name extension removed.\cr
}}}
\endinsert

\section{Compatibility with other DVI drivers}
Compatibility with other DVI drivers is achieved
by support for the following ``standard'' special calls.
Many legacy DVI files can be processed by |dvipdfm|,
so long as they use fairly standard special commands.
For example, |dvipdfm| can process DVI files generated
that use the
|\color|, |\rotatebox|, and |\includegraphics| macros
from the standard La\TeX\ Graphics bundle even if |dvips| was the target DVI driver,
e.g.,

\begintt
\usepackage[dvips]{graphics}
\usepackage[dvips]{color}
\endtt

Specifically, |dvipdfm| understands the following standard special commands:

\beginlist
\item{$\bullet$} The TPIC specials.

\item{$\bullet$} The HyperTeX (HTML) hyperlink specials.

\item{$\bullet$} The ``color'' specials supported by |dvips| and
other drivers.

\item{$\bullet$} The ``PSfile'' and ``plotfile'' specials for PS/EPS file inclusion
supported by |dvips| and other drivers.  Dvipdfm uses a user-specified
external program to convert the PostScript file to PDF format
before including it.

\item{$\bullet$} The raw PostScript ``ps:'' special supported by |dvips| and
other drivers.  Only a few PostScript operators are supported;
|dvipdfm| does not include a complete PostScript interpreter.
Complex PostScript code, such as that embedded by the PSTricks
package, is not supported.
\endlist

\section{LaTeX Support and Ebb}
Support for the La\TeX\ graphics bundle and |hyperref|
are available.  A driver file named |dvipdfm.def|
is distributed with the standard La\TeX
graphics bundle.  The latest version
of the |dvipdfm.def| file is supplied
with the |dvipdfm| distribution.
The file required for |hyperref|
support is called |hdvipdfm.def|.  

To facilitate La\TeX\ support, I distribute a companion program
called |ebb|, which extracts bounding boxes from graphics files.  If
you want to include JPEG, PNG, or PDF files in your document, you can run
|ebb| on the JPEG, PNG, or PDF file to create the |.bb| files.
The bounding box file will be similarly named with an extension of |.bb|.
For DOS 8+3 compatibility, an original file name extension 
of |.jpg|, |.png|, or |.pdf| is removed before creating the name of
the |.bb| file.  An extension of |.jpeg| is also recognized and similarly removed.

\newpage
\section{References}
\tolerance=1000\hbadness=1000
\bibitem\dest{pdfmanual}{\it Portable Document
Format Reference Manual}, Version 1.2, Adobe Systems Incorporated, 1996.
Available at the following URL:  {\tt http://www.adobe.com}. 

\bibitem\dest{pdfprimer}Thomas Merz,
{\it Web Publishing with Acrobat/PDF},
Springer-Verlag, 1997, ISBN 3-540-63762-1.  Chapter~6 of this book is available
at the URL:  |http://http://www.ifconnection.de/~tm|.

\bibitem\dest{acrotex}D. P. Story, {\it AcroTeX},  The AcroTeX home page
is located at the URL:  |http://www.math.uakron.edu/~dpstory/acrotex.html|.

\bye


==> dvipdfm/dvipdfm.1 <==
.de EX
.sp
.in +5
.nf
.ft CW
..
.de EE
.in -5
.ft R
.sp
.fi
..
.TH dvipdfm 1 5/28/2001
.SH NAME
dvipdfm \- Produce PDF files directly from DVI files

.SH SYNOPSIS
.B dvipdfm
.RI [ options ]
.IR file [.dvi]

.SH DESCRIPTION
The program
.B dvipdfm
generates a
.SM PDF
file from a
.SM DVI
file.
.SM DVI
files are the output format
produced by TeX.
Output from 
.B groff
can be converted to
.SM DVI
format
using
.BR grodvi .

The program
.B dvipdfm
recognizes several commonly used
.BR \especial
commands, which are extensions to the
.SM DVI
format.
Specifically, it understands
color specials, papersize specials,
tpic specials (which allow it to be used with
.BR pic ),
hypertex specials, and some PostScript
specials.  These extensions allow documents
to contain color, figures, and hyperlinks.
The program tries to mimic
the behavior of
.B dvips
so that many
macro packages produced for use with 
.B dvips
will work with 
.B dvipdfm.
Dvipdfm understands its own specific
.B \especial
commands to allow access to PDF features
such as annotations and bookmarks.
For more details, consult the 
.I "Dvipdfm User's Manual,"
which is distributed with
.B dvipdfm.

.SH OPTIONS

.TP 5
.B \-\^c
Ignore color
.BR \especials .
The
.B \-\^c
toggles a flag that disables color
.B \especial
processing.
Unless changed in the configuration file,
that flag is off, and color
.BR \especial "s"
are interpreted normally.
The
.B \-\^c
option may be used to produce a black and white document
from a document containing color TeX
.B \especial
commands.

.TP 5
.B \-\^d
Remove thumbnail images after including them.
(See the
.B \-\^t
option for more information.)

.TP 5
.B \-\^e
Toggle partial font embedding flag.  If partial
font embedding is off, embedded fonts are
.I fully
embedded.
The default, if not changed in the configuration file,
is to embed only those glyphs actually used in the document.

.TP 5
.B \-\^f map_file
Set the name of the font map file to 
.IR map_file .
The format of the font map file
is documented in the 
.IR "Dvipdfm User's Manual" .

.TP 5
.B \-\^l
Select landscape mode.  In other words, exchange the 
.I x
and
.I y
dimensions of the paper.

.TP 5
.B \-\^m " mag"
Magnify the input document by
.IR mag .

.TP 5
.B \-\^o " name"
Generate PDF output file having the name
.IR name .
By default, the name of the output
file is
.IR file .pdf.

.TP 5
.B \-\^p " paper"
Select the papersize by name (e.g.,
.BR letter ", " legal ", " ledger ", " tabloid ", " a3 ", " a4 ", or " a5
)

.TP 5
.B \-\^r " size"
Set resolution of bitmapped fonts to
.B size
dots per inch.  Bitmapped fonts are generated
by the Kpathsea library, which uses MetaFont.  Bitmapped
fonts are included as type 3 fonts in the PDF output file.

.TP 5
.B \-\^s " page_specifications"
Select the pages of the
.SM DVI
file to be converted.
The
.I page_specifications
consists of a comma separated list of
.I page_ranges:

.EX
.IR "page_specifications := page_specification" "[," page_specifications "]"
.EE

where

.EX
.IR "page_specification := single_page" | page_range

.IR "page_range := " [ first_page ]\^\-\^[ last_page ]
.EE

An empty
.I first_page
is implied to be the first page of the
.SM DVI
file.
An empty
.I last_page
is treated as the last page of the
.SM DVI
file.

Examples:
.RS
.TP 5
.B "\-\^s 1,3,5"
includes pages 1, 3, and 5;
.TP 5
.B "\-\^s \-"
includes all pages;
.TP 5
.B "\-\^s \-,\-"
includes two copies of all pages in the
.SM DVI
file;
and
.TP 5
.B "\-\^s 1\-10"
includes the first ten pages of the
.SM DVI
file.
.RE
.TP 5
.B \-\^t
Search for thumbnail images of each page
in the directory named by the
.B TMP
environment variable.
The thumbnail images must be named in a specific format.
They must have the same base name
as the
.SM DVI
file and they must have the page number as the extension
to the file name.  Dvipdfm does not
generate the thumbnails itself, but it is distributed with a wrapper
program named 
.B dvipdft 
that does so.

.TP 5
.B \-\^v 
Increase verbosity.
Results of the 
.B \-\^v
option are cumulative (e.g., 
.B \-\^vv
) increases the verbosity by two increments.

.TP 5
.B \-\^x x_offset
Set the left margin to 
.IR x_offset .
The default left margin is
.BR 1.0in .
The dimension may be specified in any units understood by TeX (e.g.,
.BR bpt ", " pt ", " in ", " cm
)

.TP 5
.B \-\^y y_offset
Set the top margin to 
.IR y_offset .
The default top margin is
.BR 1.0in .
The dimension may be specified in any units understood by TeX (e.g.,
.BR bpt ", " pt ", " in ", " cm
)

.TP 5
.B \-\^z compression_level
Set the compression level to 
.IR compression_level .
Compressions levels range from 0 (no compression) to
9 (maximum compression) and correspond to the values understood by zlib.

.SH ENVIRONMENT

.B Dvipdfm 
uses the
.B kpathsea
library for locating the files that it opens.  Hence,
the environment variables documented in the
.I Kpathsea library
documentation influence
.B dvipdfm.

Dvipdfm also reads the following environment variables:

.TP 5
TMP
The directory to search for thumbnail images of each page.

.SH FILES
The precise location of the following files is determined by the
.I Kpathsea library
configuration.  The location may be determined by using kpsewhich, e.g.,
.nf
.B kpsewhich \-progname=dvipdfm \-format='other text files' config
.fi

.TP 5
.I config
Startup options

.TP 5
.I t1fonts.map
The default font map file (this name may be changed in the config file).

.TP 5
.I *.tfm
TeX font metrics

.TP 5
.I *.vf
TeX virtual font files

.TP 5
.I *.pfb
PostScript Type 1 font files

.TP 5
.I 
texmf.cnf
The Kpathsea library configuration file.
The location of this file may be found by typing
.nf
.B kpsewhich texmf.cnf
.fi


.SH "SEE ALSO"
.BR tex "(1), " dvips "(1), " groff "(1), " grodvi "(1), " pic "(1), "
and the
.I "Kpathsea library"
info documentation.

.SH AUTHOR
Mark A. Wicks <mwicks@kettering.edu>



==> dvipdfm/dvipdft <==
#!/bin/sh
TMP=${TMP:-/tmp}
# Process command line args
# This script isn't very smart.  It assumes
# the last thing is the file name and ignores
# everything else.

usage() {
  echo No file name specified.
  exit 1
}

# Must have at least one argumen (the DVI filename)
if [ $# -eq 0 ]
then
  usage
fi

# Loop over all arguments except the last one
USERARGS=$@
ARGS=
PDFFILENAME=
while [ $# -ne 1 ]
do
   ARGS="$ARGS $1"
   if [ "$1" = "-o" ]
   then
      PDFFILENAME=`echo $2 | sed -e's/\.pdf//g'`
      ARGS="$ARGS $2"
      shift
   fi
   shift
done
FILENAME=$1
if [ -z "$PDFFILENAME" ] 
then
  PDFFILENAME=$FILENAME
fi

# Run dvipdfm with the fastest options for the first pass
if dvipdfm $ARGS -e -z0 $FILENAME
then
   if gs -r10 -dNOPAUSE -dBATCH -sDEVICE=png256 -sOutputFile=$TMP/$PDFFILENAME.%d $PDFFILENAME.pdf
   then
#  Run dvipdfm with the users specified options for the last pass
      echo dvipdfm -dt $USERARGS;
      dvipdfm -dt $USERARGS;
   fi   
fi   



==> dvipdfm/mkinstalldirs <==
#! /bin/sh
# mkinstalldirs --- make directory hierarchy
# Author: Noah Friedman <friedman@prep.ai.mit.edu>
# Created: 1993-05-16
# Public domain

# $Id: mkinstalldirs,v 1.13 1999/01/05 03:18:55 bje Exp $

errstatus=0

for file
do
   set fnord `echo ":$file" | sed -ne 's/^:\//#/;s/^://;s/\// /g;s/^#/\//;p'`
   shift

   pathcomp=
   for d
   do
     pathcomp="$pathcomp$d"
     case "$pathcomp" in
       -* ) pathcomp=./$pathcomp ;;
     esac

     if test ! -d "$pathcomp"; then
        echo "mkdir $pathcomp"

        mkdir "$pathcomp" || lasterr=$?

        if test ! -d "$pathcomp"; then
  	  errstatus=$lasterr
        fi
     fi

     pathcomp="$pathcomp/"
   done
done

exit $errstatus

# mkinstalldirs ends here

